Numerical Study of Eigenvector Deflation to Accelerate the WaveHoltz Method

We present a numerical study of eigenvector deflation as a means of accelerating the WaveHoltz method for solving the Helmholtz equation. For energy-conserving (Dirichlet or Neumann) boundary conditions the WaveHoltz fixed-point iteration converges slowly at high frequency, requiring approximately $\mathcal{O}(\omega^{2d})$ iterations in $d$ dimensions. We show that deflating the eigenvectors whose eigenvalues lie nearest the driving frequency substantially reduces iteration counts, and we examine two ways of incorporating the eigenvectors: direct eigenvector deflation (DEVD), in which the forcing and iterate are projected against the deflation set, and augmented-Krylov eigenvector deflation (AUKED) using deflated conjugate gradient (DCG), augmented GMRES (AGMRES), and augmented (recycled) BICGSTAB (ABICGSTAB). The required eigenpairs can be computed efficiently with the EigenWave approach, and we demonstrate, in two dimensions, that when the number of deflation vectors grows quadratically with $\omega$ the asymptotic convergence rate remains essentially constant. Because the eigenvectors on structured grids are naturally represented as matrices, we further apply SVD-based compression to reduce their storage. Numerical experiments on single curvilinear grids discretized with summation-by-parts operators, and on overset grids illustrate the robustness and efficiency of the approach, with the deflated solver breaking even against the undeflated solver after as few as two right-hand sides, when accounting for the cost of precomputing the eigenvectors.

==> tex/convergenceSpeed.tex <==
%!TEX root = ../deflation.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Convergence speed of deflated WaveHoltz method\label{sec:waveholtz_deflation}} \deaa{Remove this section?}

To accelerate the convergence of the WaveHoltz method for energy conserving problems with trapped wave structures, we apply the DCG algorithm with eigenvectors or prolonged eigenvectors as the deflation matrix.
Here, we formally analyze the relation between the number of  eigenvectors in the deflation space and the convergence speed. 
For simplicity, we consider a homogeneous velocity field with $c(\xb)=1$. We first present the analysis results in Sec. \ref{sec:analysis-result}, followed by details of the analysis  in Sec. \ref{sec:analysis-procedure}. 


\subsection{Relation between the number of eigenvectors and computational costs\label{sec:analysis-result}}
Assume a homogeneous velocity field $c(\xb)=1$, which allows us to utilize the Weyl's principle \cite{weyl1912asymptotische} to formally estimate the relation between the dimension of the eigenvector deflation space and the number of iterations needed for convergence of DCG. In this section, we present our main results.

\textbf{Relation between number of eigenvectors and number of iterations for convergence.} Assume $W$ comprising eigenvectors corresponding to the $\Na$ smallest eigenvalues of the discrete WaveHoltz operator $A=I-S_h$. With  sufficiently high frequency $\omega$,  sufficiently small mesh size $h$ and time step size $\Dt$, the DCG algorithm solving $A\ub=(I-S_h)\ub=\bbb$ converges with $$N^{\textrm{DCG}}_{\textrm{iter}}\approx\frac{C_{\textrm{iter}}}{\Na}$$  iterations, where $C_{\textrm{iter}}$ represents a constant.

\textbf{Computational cost of the DCG in Alg. \ref{alg:DCG} and Eig-DCG in Alg. \ref{alg:eig-DCG} with the eigenvector deflation.}  When eigenvector deflation is applied, the deflation matrix $W\in\mathbb{R}^{N_{\textrm{DOF}}\times \Na}$ is a dense matrix, and $W^TAW\in\mathbb{R}^{\Na\times \Na}$ is a diagonal matrix leading to $O(\Na)$ computational cost of applying $(W^TAW)^{-1}$. Additionally, the matrix $W^TA\in\mathbb{R}^{N_{\textrm{DOF}}\times \Na}$ is dense and can be pre-computed. 
Utilizing these facts, computational cost of each step in the DCG algorithm is  estimated and summarized in Tab. \ref{tab:dcg-cost}.
\begin{table}[htbp]
  \centering
 \medskip
    \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|}
    \hline
	& Vector Operations  & Apply A  & Apply $W^TA$  & Apply $(W^TAW)^{-1}$ & Apply $W$  \\ \hline
 Line in Alg. \ref{alg:DCG} & $14-19, 22$ & $13$ & $20$ & $21$ & $22$ \\ \hline
 Cost &	$O(N_{\textrm{DOF}})$ & $N_tO(N_{\textrm{DOF}})$ & $KO(N_{\textrm{DOF}})$ & $O(\Na)$ & $KO(N_{\textrm{DOF}})$ \\
 	\hline
 \end{tabular}
      \caption{Computational cost of each steps in the DCG method Alg. \ref{alg:DCG} with the eigenvector deflation.\label{tab:dcg-cost}}
\end{table}

DCG converges with approximately $C_{\textrm{iter}}/\Na$ iterations. 
Consequently, the total cost of solving the WaveHoltz system $A\xb=(I-S_h)\xb=\bbb$ with DCG can be estimated as follows:
\begin{align}
\textrm{Cost}_{\textrm{DCG}} &\approx N^{\textrm{DCG}}_{\textrm{iter}}\times
\Big( \textrm{Vector Operations (line 14-19, 22)} + \textrm{Apply A (line 13)}\notag\\
&\quad\quad+\textrm{Apply $W^TA$ (line 20)} + \textrm{Solve $W^TAW$ (line 21)}+\textrm{Apply $W$ (line 22)}\Big)\notag\\
&= \frac{C_{\textrm{iter}}}{\Na}\times
\big(  O(N_\textrm{DOF})+N_t O(N_\textrm{DOF})+\Na O(\textrm{DOF})+O(\Na)\big)\notag\\
&=C_{\textrm{iter}}O(N_\textrm{DOF})\left(\frac{C_tN_t+C^{\textrm{DCG}}_{\textrm{vec}}}{\Na}+C_W+C_{W^TA}\right).\label{eq:cost19}
\end{align}
where $C_t, C^{\textrm{DCG}}_{\textrm{vec}},C_W$ and $C_{W^TA}$ 
 are constants. As a result, we would expect a sub-linear acceleration as we increase the number of eigenvectors $\Na$. 

Similarly, the cost of Eig-DCG with $\Na$-eigenvectors as the deflation amtrix can be estimated as:
\begin{align}
\textrm{Cost}_{\textrm{Eig-DCG}} &\approx N^{\textrm{Eig-DCG}}_{\textrm{iter}}\times
\Big( \textrm{Vector Operations (line 14-20)} + \textrm{Apply A (line 13)}\Big)\notag\\
&= \frac{C_{\textrm{iter}}}{\Na}\times
\big(  O(N_\textrm{DOF})+N_t O(N_\textrm{DOF})\big)\notag\\
&=C_{\textrm{iter}}O(N_\textrm{DOF})\left(\frac{C_tN_t+C^{\textrm{Eig-DCG}}_{\textrm{vec}}}{\Na}\right).\label{eq:cost19}
\end{align}
where $C_t, C^{\textrm{DCG}}_{\textrm{vec}},C_W$ and $C_{W^TA}$ 
 are constants. 
 

Without deflation, the computational cost of solving the WaveHoltz system with CG is approximately
\begin{align}
\textrm{Cost}_{\textrm{CG}} &\approx N^{\textrm{CG}}_{\textrm{iter}}\times
\left( \textrm{Vector Operations} + \textrm{Apply A }\right)\notag\\
&= N^{\textrm{CG}}_{\textrm{iter}} O(N_{\textrm{DOF}})(C_tN_t+C^{\textrm{CG}}_{\textrm{vec}}).
\end{align}
Therefore, the relative computational cost of the DCG method (Alg. \ref{alg:DCG}) and Eig-DCG method (Alg. \ref{alg:DCG}) with respect to the CG method are approximately
\begin{subequations}
\begin{align}
\textrm{Relative Cost of DCG}&=\frac{\textrm{Cost}_{\textrm{DCG}}}{\textrm{Cost}_{\textrm{CG}}} \approx 
    \frac{C_{\textrm{iter}}}{N_{\textrm{iter}}^{\textrm{CG}}}\left(\frac{\frac{1}{\Na}\left(C_tN_t+C^{\textrm{DCG}}_{\textrm{vec}}\right)+\left(C_W+C_{W^TA}\right)}{C_tN_t+C^{\textrm{CG}}_{\textrm{vec}}}\right),\\
  \textrm{Relative Cost of Eig-DCG}&=  \frac{\textrm{Cost}_{\textrm{DCG}}}{\textrm{Cost}_{\textrm{CG}}} \approx 
    \frac{C_{\textrm{iter}}}{N_{\textrm{iter}}^{\textrm{CG}}}\left(\frac{\frac{1}{\Na}\left(C_tN_t+C^{\textrm{Eig-DCG}}_{\textrm{vec}}\right)}{C_tN_t+C^{\textrm{CG}}_{\textrm{vec}}}\right).
\end{align}
\end{subequations}
In comparison with CG, DCG has overheads for applying $W$, $W^TA$ and $(W^TAW)^{-1}$ in each iteration, but it converges with fewer total iterations. Overall, with a proper chosen $\Na$, DCG achieves acceleration over CG. 



When prolonged eigenvectors are leveraged, the matrix $W^TAW$ is not diagonal anymore, potentially increasing the cost of applying $(W^TAW)^{-1}$ to $O(\Na^2)$. If eigenvectors on the fine mesh are well approximated by the prolonged eigenvectors from the coarse mesh, the estimated computational cost of solving the WaveHoltz system with DCG becomes
\begin{equation}
C_{\textrm{iter}}O(N_\textrm{DOF})\left(\frac{C_tN_t+C^{\textrm{DCG}}_{\textrm{vec}}}{\Na}+C'_W+C'_{W^TA}\right)+C'_{W^TAW} O(\Na)\label{eq:prolong_cost}
\end{equation}
where
$C'_W,C'_{W^TA},C'_{W^TAW}$ are constants. In practice, the number of eigenvectors in the deflation space, $\Na$, is much smaller than the total number of degrees of freedom $N_{\textrm{DOF}}$, and the $O(\Na)$ term in the computational cost \eqref{eq:prolong_cost} is almost negligible. We still expect a sub-linear acceleration, as we increase the number of eigenvectors $\Na$. 

%Since the cost of  applying the WaveHoltz operator is dominant, enlarging the number of prolonged eigenvectors $\Na$ initially results in computational saving. However, there may be no computational saving or even more computational costs when $\Na$ becomes too large.     

In our numerical tests, we observe that using a moderate number of eigenvectors or prolonged eigenvectors as the deflation matrix, we are able to gain almost linear acceleration over CG.%computational saving compared to CG. 

% \

==> tex/convergence_analysis.tex <==
%!TEX root = ../deflation.tex
\subsection{Convergence analysis\label{sec:analysis-procedure}}
We formally analyze the convergence speed of DCG using  eigenvector deflation by exploiting the eigen-structure of the WaveHoltz operator. 
Recall that an eigenvalue of the continuous WaveHoltz operator is in the form of $1-\beta(\lambda_j;\omega)$, where $-\lambda_j^2$ is an eigenvalue of the Laplacian operator.
In our analysis, we first convert the filtering transfer function $\beta(\lambda;\omega)$ to a scaled filtering transfer function $\wtbeta(\frac{\lambda}{\omega})$. Then, we utilize the property of the scaled transfer function $\wtbeta(\frac{\lambda}{\omega})$ and Weyl's asymptotic for the eigenvalues of the Laplacian operator \cite{weyl1912asymptotische,strauss2007partial} to estimate the condition number of the WaveHoltz operator. Finally, leveraging the convergence theory of the DCG algorithm in Theorem \ref{thm:dcg}, we estimate the relation between the number of eigenvectors and the number of iterations for convergence. 

In this section, we derive the scaled filtering transfer function and present its properties in Sec. \ref{sec:scaled-transfer} and then complete the analysis  in Sec. \ref{sec:analysis-condition-number}


\subsubsection{Scaled filtering transfer function\label{sec:scaled-transfer}}
As proved in \cite{garcia2022extensions}, the eigenvalues of the continuous WaveHoltz operator are given by $1-\beta(\lambda;\omega)$, where $\lambda$ is the square root of an eigenvalue of the negative Laplacian operator. To simplify the analysis, we prove that the filtering transfer function $\beta(\lambda;\omega)$ equals to a scaled transfer function $\wtbeta(\frac{\lambda}{\omega})$:
\begin{align}
\beta(\lambda;\omega) &= \frac{\omega}{\pi}\int_{0}^{\frac{2\pi}{\omega}}\left(\cos(\omega t)-\frac{1}{4}\right)\cos(\lambda t) dt\notag\\
&\stackrel{\tau= \omega t}{=}\frac{1}{\pi}\int_{0}^{2\pi} (\cos(\tau)-\frac{1}{4})\cos(\frac{\lambda}{\omega}\tau)d\tau,
\end{align}
Let $\theta = \frac{\lambda}{\omega}$. We have
\begin{align}
\beta(\lambda;\omega) &= \frac{1}{\pi}\int_{0}^{2\pi} \left(\cos(\tau)-\frac{1}{4}\right)\cos(\theta\tau)d\tau\notag\\
&=\frac{1}{2\pi}\int_{0}^{2\pi}\left(\;\cos((1+\theta)\tau)+\cos((1-\theta)\tau)-\frac{1}{2}\cos(\theta\tau)\;\right)d\tau\notag\\
&=\wtbeta(\theta).
\end{align}
When $\theta\neq 0,1$, we obtain
\begin{align}
    \wtbeta(\theta)&=\frac{1}{2\pi}\left(\frac{1}{1+\theta}\sin( (1+\theta)\tau)+\frac{1}{1-\theta}\sin((1-\theta)\tau)-\frac{1}{2\theta}\sin(\theta\tau)\right)\Big|_{\tau=0}^{\tau=2\pi}\notag\\
    &=\frac{\sin(2\pi\theta)}{2\pi}\left(\frac{1}{\theta+1}+\frac{1}{\theta-1}-\frac{1}{2\theta}\right).    
\end{align}
One can also show that $\wtbeta(0)=\lim_{\theta\rightarrow 0+}\wtbeta(\theta)=-\frac{1}{2}$ and $\wtbeta(1)=\lim_{\theta\rightarrow1}\wtbeta(\theta)=1$. In summary,
\begin{align}
    \wtbeta(\theta) = \begin{cases}
                      -0.5, \quad&\theta=0,\\
                      1,\quad &\theta = 1,\\
                      \frac{\sin(2\pi\theta)}{2\pi}\left(\frac{1}{\theta+1}+\frac{1}{\theta-1}-\frac{1}{2\theta}\right),\quad &\text{otherwise}.
                      \end{cases} 
\end{align}
We can easily prove that $\wtbeta(\theta)=0$ when $\theta=\frac{2k+1}{2}$, $k\in\mathbb{N}$.
The shape of the scaled transfer function $\wtbeta$ is demonstrated in Fig. \ref{fig:wtbeta}. Basic properties of $\wtbeta(\theta)$ are summarized in the theorem below. 
\begin{thm}\label{thm:beta-property}
The scaled transfer function $\wtbeta(\theta)$ satisfies the following properties.
\begin{enumerate}
\item $\wtbeta(\theta)$ is monotonically increasing on $[0,1]$ and monotonically decreasing on $[1,\frac{3}{2}]$.
\item When $\theta\geq \frac{3}{2}$, $|\wtbeta(\theta)|\leq\frac{31}{30\pi}<\frac{1}{3}$.
\item When $\theta\geq 0$, $-\frac{1}{2}\leq\wtbeta(\theta)\leq 1$.
\end{enumerate}
\end{thm}

\begin{proof}
By computing the derivative of $\wtbeta(\theta)$, we can prove that $\wtbeta(\theta)$ is monotonically increasing when $\theta\in(0,1)$ and monotonically decreasing when $\theta\in(1,\frac{3}{2}$].
Further leveraging $\wtbeta(0)=-\frac{1}{2}$, $\wtbeta(1)=1$ and $\wtbeta(\frac{3}{2})=0$, we can show that $-\frac{1}{2}\leq \wtbeta(\theta)\leq 1$ when $\theta\in[0,\frac{3}{2}]$

Now, we only need to show that when $\theta\geq\frac{3}{2}$, we have $|\wtbeta(\theta)|\leq\frac{31}{30\pi}<\frac{1}{3}$. 
Let 
$$\gamma(\theta)=\frac{1}{2\pi}\left(\frac{1}{\theta+1}+\frac{1}{\theta-1}-\frac{1}{2\theta}\right)
=\frac{3\theta^2+1}{4\pi(\theta^2-1)\theta},
$$ then 
\begin{equation}
\wtbeta(\theta)=\sin(2\pi\theta)\gamma(\theta)\quad\text{and}\quad
    \frac{d\gamma}{d\theta}=-\frac{3\theta^4+6\theta^2-1}{4\pi(\theta^2-1)^2\theta^2}
    =-\frac{3(\theta^2+1)^2-4}{4\pi(\theta^2-1)^2\theta^2}.
\end{equation}
When $\theta\geq \frac{3}{2}$, we can verify that $ \frac{d\gamma}{d\theta}<0$
and $\gamma(\theta)>0$. Therefore, $\gamma(\theta)$ is a positive function monotonically decreasing on $[\frac{3}{2},\infty)$. Hence, $$\max_{\theta\geq\frac{3}{2}}|\gamma(\theta)|=\max_{\theta\geq\frac{3}{2}}\gamma(\theta)=\gamma(\frac{3}{2})=\frac{31\pi}{30}.$$
Utilizing these facts, we get when $\theta\geq\frac{3}{2}$, 
$$|\wtbeta(\theta)|=|\sin(\theta)\gamma(\theta)|\leq |\gamma(\theta)|\leq\gamma(\frac{3}{2})=\frac{31}{30\pi}<\frac{1}{3}.$$
\end{proof}

Recall that the eigenvalue of the continuous WaveHoltz operator $I-S$ is $\beta(\lambda;\omega)=\wtbeta(\lambda/\omega)$, where $-\lambda^2$ is an eigenvalue of the Laplacian operator. Utilizing the local monotonicity and boundedness of $\wtbeta$ in Theorem \ref{thm:beta-property}, the smallest eigenvalues of the continuous WaveHoltz operator are corresponding to $\theta=\frac{\lambda}{\omega}$ closest to $1$, or in other words, $\lambda$ closest to $\omega$.


\begin{rem}
Lemma 2.1 of \cite{appelo2020waveholtz} demonstrates an analysis of $\beta(\lambda;\omega)$ similar to Theorem \ref{thm:beta-property}. 
The details of these two analysis are different. Furthermore, Theorem \ref{thm:beta-property} results in a slightly sharper upper bound for the case when $\theta=\lambda/\omega>\frac{3}{2}$.
\end{rem}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[htb]
\begin{center}
\includegraphics[width=0.46\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/beta_tilde.eps}
\caption{The scaled filter transfer function $\wtbeta(\theta)$.\label{fig:wtbeta}}
\end{center}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Condition number of the deflated WaveHoltz operator\label{sec:analysis-condition-number}}
With energy conserving boundary conditions, the WaveHoltz method yields an SPD linear system. To estimate the condition number of the deflated WaveHoltz operator, we need to find an upper bound for its largest eigenvalue and a lower bound for its smallest eigenvalue. 

Recall that the eigenvalue of the continuous WaveHoltz operator $I-S$ is $1-\beta(\lambda;\omega)=1-\wtbeta(\theta)$, where $-\lambda^2$ is an eigenvalue of the Laplacian operator. According to the monotonicity and the boundedness of $\wtbeta$ discussed in Theorem \ref{thm:beta-property}, the largest eigenvalue of the continuous WaveHoltz operator is not greater than $1-(-0.5)=1.5$ and the smallest eigenvalues of it are corresponding to $\theta=\frac{\lambda}{\omega}$ closest to $1$. 
To estimate the desired condition number, we analyze the local behavior of $\wtbeta$ around $\theta=1$ and utilize Weyl's principle to find $\lambda$'s closest to $\omega$.

\begin{thm}\label{thm:weiyl}(Weyl's principle\cite{weyl1912asymptotische,strauss2007partial})
With $d=2,3$, the $n$-th eigenvalue of the $d$-dimensional problem  
$-\Delta u=\lambda_n^2 u$ in the domain $D$ with the Dirichlet boundary conditions $u|_{\partial D}=0$ satisfies
\begin{equation}
    \lim_{n\rightarrow \infty}\frac{\lambda^2_n}{n^{\frac{2}{d}}} = \frac{C_d}{V^{\frac{2}{d}}}=G_d,
    \quad 
    C_d=\begin{cases}
    4\pi, \; \text{if}\;d=2,\\
    (6\pi)^{\frac{2}{3}},\;\text{if}\;d=3,
    \end{cases}
\end{equation}
where $V$ is the volume of $D$.
\end{thm}

\textbf{Assumption.} For simplicity, we make the following assumptions.
\begin{enumerate}
    \item We assume that the eigenvalue of the WaveHoltz operator, which is closest to the frequency $\omega$, corresponds to the $j$-th eigenvalue of the Laplacian operator $\Delta$, $-\lambda_j^2$. In other words, 
    $$\lambda_j=\arg\min_\lambda|\lambda-\omega|$$ 
    subject to $-\lambda^2$ being an eigenvalue of the Laplacian operator.
    %\item We assume $M\in\mathbb{N}$ satisfying $|\lambda_{j+M+1}-\lambda_{j-M-1}|/\omega<1$.
    \item We assume that $\omega$ is sufficiently large so that Weyl's principle gives us a reasonable approximation to $\lambda_k$ for $j-M-1\leq k\leq j+M+1$:
    \begin{equation}
        \lambda_{k}\approx C_d/V^{\frac{1}{d}}k^{\frac{1}{d}}=k^\frac{1}{d}/{G_d}.
    \end{equation}
    \vspace{-0.25in}
    \item Mesh size $h$ and time step size $\Delta t$ are sufficiently small so that eigenvalues of the continuous Laplacian operators, $-\lambda^2_{k}$ with $j-M-1\leq k\leq j+M+1$, 
    are well approximated by the eigenvalues of the discrete Laplacian operator $-\lambda_{h,k}^2$.
    \item We assume $K=2M+3$, and $W$ consists of eigenvectors corresponding to $\lambda_{h,k}$, where $j-M-1\leq k\leq j+M+1$.
\end{enumerate}
Assumption $2$ guarantees the applicability of Weyl's principle. 
When Assumption $3$ and $4$ hold, we can utilize Theorem \ref{lem:kappa} to estimate an upper bound for the condition number of the deflated discrete WaveHoltz operator $P^T(I-S_h)P$ as follows:
\begin{align}
    \kappa_{P^T(I-S_h)P}&=\frac{1-\lambda_{\textrm{min}}^{S_h}}{1-\beta_h(\lambda_{h,j_{K+1}};\omega)}
    \leq \frac{1-\lambda_{\textrm{min}}^{S_h}}{1-\beta_h(\lambda_{h,j+M+1};\omega)}
        \approx \frac{1-\lambda_{\min}^{S}}{1-\beta_(\lambda_{j+M+1};\omega)}\notag\\
       & \leq\frac{1.5}{1-\beta(\lambda_{j+M+1};\omega)}=\frac{1.5}{1-\wtbeta(\theta_{j+M+1})}=R(\theta_{j+M+1}),\quad\theta_{j+M+1}=\frac{\lambda_{j+M+1}}{\omega},\label{eq:R-definition}
\end{align}
where $\lambda_{\textrm{min}}^S$ and $\lambda_{\textrm{min}}^{S_h}$ are the smallest eigenvalues of $S$ and $S_h$ respectively, and $-\lambda^2_{h,j_{K+1}}$ is the eigenvalue of the discrete Laplacian operator which is the $K+1$-th closest to $-\omega^2$. The ratio $$R(\theta_{j+M+1})=\frac{3}{2}/(1-\wtbeta(\theta_{j+M+1}))$$ provides an estimated upper bound for the desired condition number, in other words,
$$ \kappa_{P^TAP}\lesssim R(\theta_{j+M+1}).$$

\textbf{Estimate $R(\theta_{j+M+1})$.}
We first estimate the value of $j$ and the value of $\theta_{j+M+1}$, then perform a Taylor expansion of $\wtbeta$ around $\theta=1$ to estimate $R(\theta_{j+M+1})$.

\textbf{Step 1a: estimate $j$.} Utilizing the fact that $\lambda_j\approx j^{\frac{1}{d}}/G_d$ is the closest $\lambda$ to $\omega$, we obtain 
\begin{equation}
    j \approx \textrm{Int}(G_d^d\omega^d),
\end{equation}
where $\textrm{Int}(G_d^d\omega^d)$ is the closest integer to $G_d^d\omega^d$.

\textbf{Step 1b: estimate}
\begin{align}
\Delta\theta_{j+M+1}= \frac{\lambda_{j+M+1}}{\omega}-1.
\end{align}
With the estimation of $j$, we have
\begin{align}
|\Delta\theta_{j+M+1}|=&\left|\frac{\lambda_{j+ M+1}}{\omega}-1\right|
\approx\left|\frac{\frac{1}{G_d}\left(\textrm{Int}(G_d^d\omega^d)+M+1 \right)^\frac{1}{d}}{\omega}-1\right|
\notag\\
\geq& \frac{ (G_d^d\omega^d+M)^{\frac{1}{d}}}{G_d\omega}-1
= \left(1+\frac{M}{G_d^d\omega^d}\right)^{\frac{1}{d}}-1.
\end{align}
Using L'Hopitol rule, we have
\begin{align}
\lim_{\omega\rightarrow\infty} \frac{ \left(1+\frac{M}{G_d^d\omega^d}\right)^{\frac{1}{d}}-1}{\frac{1}{G_d^d\omega^d}}=\frac{M}{d}.
\end{align}
Then, for sufficiently large frequency $\omega$, 
\begin{equation}
   |\Delta \theta_{j+M+1}|\gtrsim\frac{M}{d}\frac{1}{(1+\epsilon)G_d^d\omega^d}, 
   \label{eq:jump}
\end{equation} 
where $\epsilon>0$ is an arbitrary positive number.

\textbf{Step 2a: Taylor expansion of $\wtbeta$.} 
Let $\Delta\theta = \theta-1$, then 
 Taylor expansion gives us
\begin{align}
\widetilde{\beta}(\theta)
&= \frac{2\pi\Delta\theta-\frac{4\pi^3}{3}\Delta\theta^3+O(\Delta\theta^5)}{2\pi}\left(\frac{1}{\theta-1}+\frac{1}{\theta+1}-\frac{1}{2\theta}\right)\notag\\
&=\left(\Delta\theta-\frac{2\pi^2}{3}\Delta\theta^3+O(\Delta\theta^5)\right)
\left(\frac{1}{\Delta\theta}+\frac{1}{2+\Delta\theta}-\frac{1}{2+2\Delta\theta}\right)
\notag\\
&= 1-\frac{2\pi^2}{3}\Delta\theta^2+O(\Delta\theta^4)+\left(\Delta\theta+O(\Delta\theta^3)\right)\left(\frac{1}{2(1+\frac{1}{2}\Delta\theta)}-\frac{1}{2(1+\Delta\theta)}\right)\notag\\
&= 1-\frac{2\pi^2}{3}\Delta\theta^2+
\frac{\Delta\theta}{2}\left( -\frac{1}{2}\Delta\theta+\Delta\theta\right)+O(\Delta\theta^3)\notag\\
&=1+\left(\frac{1}{4}-\frac{2\pi^2}{3}\right)\Delta\theta^2 + O(\Delta\theta^3).
\end{align}
As a result,
\begin{equation}
R(\theta)=\frac{\frac{3}{2}}{1-\widetilde{\beta}(\theta)}\approx \frac{\frac{3}{2}}{(\frac{2\pi^2}{3}-\frac{1}{4})\Delta\theta^2}.
\label{eq:R_fun}
\end{equation}
\textbf{Step 2b: estimate $R(\theta_{j+M+1})$.} Substitute \eqref{eq:jump} into \eqref{eq:R_fun}, we obtain
\begin{equation}
    R(\theta_{j+M+1})\approx \frac{1.5}{(\frac{2\pi^2}{3}-\frac{1}{4})\Delta\theta_{j+M+1}^2}\gtrsim \frac{1.5(1+\epsilon)^2G_d^{2d}\omega^{2d}}{(\frac{2\pi^2}{3}-\frac{1}{4})}\frac{d^2}{M^2}.\label{eq:R-estimate}
\end{equation}

\textbf{Estimate the number of iterations for convergence.} According to Theorem \ref{thm:dcg}, to reach an error $||\xb_{N_\varepsilon}-\xb||\approx\varepsilon$, we have
\begin{align}
    &2\left(\frac{\sqrt{\kappa_{P^T(I-S_h)P}}-1}{\sqrt{\kappa_{P^T(I-S_h)P}}+1}\right)^{N_\varepsilon}=2\left(1-\frac{2}{\sqrt{\kappa_{P^T(I-S_h)P}}+1}\right)^{N_\varepsilon}\approx \varepsilon,\\
    &N_\varepsilon \approx \ln\left(\frac{\varepsilon}{2}\right)/\ln\left(1-\frac{2}{\sqrt{\kappa_{P^T(I-S_h)P}}+1}\right)
    \leq \left|ln\left(\frac{\varepsilon}{4}\right)\right|(\sqrt{\kappa_{P^T(I-S_h)P}}+1), \; \text{if}\; \kappa> 1.\label{eq:N-eps}
\end{align}
The last inequality is obtained by taking the Taylor expansion of $\ln\left(1-\eta\right)$ around $\eta=0$ and utilizing the fact that $\kappa_{P^TAP}\geq 1$ is inside the convergence domain of the expansion.
Leveraging \eqref{eq:R-definition}, \eqref{eq:R-estimate} and \eqref{eq:N-eps}, we obtain
$N_{\varepsilon}\leq O(\sqrt{\kappa_{P^T(I-S_h)P}})\lesssim O(\frac{1}{M})=O(\frac{1}{K})$. 


==> tex/main.tex <==
% %!TEX root = ../deflation.tex
% \section{WaveHoltz method for the Helmholtz equation\label{sec:waveholtz}}
% We use the WaveHoltz method \cite{appelo2020waveholtz} to solve the Helmholtz equation 
% \begin{align}
% \omega^2 u + \nabla \cdot (c(\bx)^2 \nabla u) = f(x), \ \  \bx \in \Omega, \label{eq:helmholtz}
% \end{align}
% with the energy conserving homogenuous Dirichlet boundary condition
% \begin{align}
% u(\bx) = 0, \ \ \bx \in \Gamma=\partial \Omega.
% \end{align}
% Here, frequency $\omega$ is not a resonance.
% WaveHoltz method is an iterative solver built on a time-domain solver for the wave equation 
% \begin{subequations}
% \begin{align}
%     &\hat{u}_{tt}=\nabla \cdot (c(\bx)^2 \nabla \hat{u})-f(\bx)\cos(\omega t),\\
%     &\hat{u}(\bx,t)=0,\ \ \bx\in \partial\Omega,\\
%     &\hat{u}(\bx,0)=\nu(\bx),\\
%     &\hat{u}_t(\bx,0)=0.
% \end{align}
% \label{eq:wave}
% \end{subequations}
% A filtering operator acting on the initial condition of the wave equation $\nu(\bx)$ is introduced as
% \begin{align}
%     \Pi \nu(\bx) = \frac{2}{T}\int_{0}^{T}(\cos(\omega t)-\frac{1}{4})\hat{u}(\bx,t) dt,
% \end{align}
% where $\hat{u}(\bx,t)$ is the time-domain solution determined by the initial condition $\nu(x)$. Operator $\Pi$ filters the time-domain solution 
%  over one period.
% As shown in \cite{appelo2020waveholtz}, the solution to the Helmholtz equation \eqref{eq:helmholtz} $u$ is a fixed point of the filtering operator $\Pi$ and the corresponding time-domain solution is $\hat{u}(\bx,t)=u(\bx)\cos(\omega t)$. In other words, the Helmholtz equation is equivalent to the fixed point problem
% \begin{equation}
%     \Pi u = u.
% \end{equation}
% This fixed point problem can be further rewritten as an equivalent linear problem 
% \begin{align}
%     (I-S)u = \Pi 0,\label{eq:I_minus_S}
% \end{align}
% where the linear operator $S$ is defined as $Su = \Pi u -\Pi 0$. 
% After discretization, the resulting linear system can be solved by a Krylov subspace method. Moreover, with homogeneous Dirichlet boundary conditions, this linear system is proved to be  symmetric positive definite (SPD) \cite{appelo2020waveholtz}. As a result, conjugate gradient (CG) method can be applied to solve it.

% \input ./tex/discretization.tex


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Convergence theory of WaveHoltz method}

% Here we summarize the convergence theory for the continuous WaveHoltz algorithm, see~\cite{appelo2020waveholtz} for more details.
% The WaveHoltz algorithm can be analyzed using the eigenfunctions of,
% \bse
% \ba
% \ea
% \ese

% The convergence speed of the WaveHoltz method can be analyzed by utilizing the eigenmodes of the Laplacian operator $-\nabla\cdot(c(x)^2\nabla)$.
% With the homogeneous Dirichlet boundary conditions, the operator $-\nabla\cdot(c(x)^2\nabla)$ has a point spectrum with positive eigenvalues $\lambda_j^2$ and corresponding eigen-functions $\phi_j$. These eigen-functions form a basis of $L^2(\Omega)$. Then, any function $\nu(x)\in L^2(\Omega)$ can be expanded as $\nu=\sum_{j=0}^\infty\hat{\nu}_j\phi_j$. 

% Following \cite{appelo2020waveholtz,garcia2022extensions}, the linear operator $S: L^2(\Omega)\rightarrow L^2(\Omega)$ operator can be written as:  
% \begin{align}
%     S:\sum_{j=0}^\infty \hat{\nu}_j\phi_j\rightarrow \sum_{j=0}^\infty\beta(\lambda_j;\omega)\hat{\nu}_j \phi_j,
% \end{align}
% where 
% \begin{align}
%     \beta(\lambda;\omega) = \frac{2}{T}\int_{0}^{T}(\cos(\omega t)-\frac{1}{4})\cos(\lambda t)dt,
%     \label{eq:beta_fun}
% \end{align}
% and the eigenvalues of $S$ are $\beta(\lambda_j;\omega)$.
% As shown in \cite{appelo2020waveholtz,garcia2022extensions}, $-0.5\leq\beta(\lambda;\omega)\leq 1$ and the spectral ratio of $S$ scales as $$\rho_S \sim 1-O(\delta^2)<1,$$ where $\delta =\min_{\lambda_j}\frac{\lambda_j-\omega}{\omega}$. As a result, the largest eigenvalue of $I-S$ is bounded $0<\lambda^{I-S}_{\max}\leq 1.5$, and the smallest eigenvalue scales as $\lambda^{I-S}_{\min} \sim O(\delta^2)$. Thus, the condition number of $I-S$ scales as $O(\delta^2)$, and Weyl proved $\delta\sim O(\omega^d)$ \cite{weyl1912asymptotische}. As a result, the condition number of $I-S$ scales as $O(\omega^{2d})$, which implies that CG method  needs  $O(\omega^d)$ iterations for convergence. 

% %As presented in \cite{saad2000deflated}, the convergence 
% %If one can introduce a deflation space to remove the eigenvalues of $S$ which are close to $1$, the CG iterative solver can be accelerated.
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% \subsection{Eigenvalues of discrete WaveHoltz operator\label{sec:waveholtz-eig}}
% The eigenvalues of the discrete WaveHoltz operator $S_h$ can be obtained based on the eigenvalues of the discrete Laplacian operator $L_h$. Suppose $\{-\lambda_{h,j}^2\}_{j=1}^{N}$ are the eigenvalues of $L_h$ and $\{\wb_j\}_{j=1}^{N}$ are the corresponding eigenvectors. 
% One can verify that $\wb_j^h$ is also an eigenvector of the discrete WaveHoltz operator $I-S_h$:
% \begin{equation}
%     (I-S_h)\wb_j = (1-\beta_h(\lambda_j;\omega))\wb_j, \label{eq:waveholtz_eigvectors}
% \end{equation} 
% where
% \begin{subequations}
% \begin{align}
%     &\beta_h(\lambda_j;\omega) = \frac{2\Dt}{T}\sum_{j=0}^{N_t}\eta_n\mu^n_j,\quad  \eta_n=\begin{cases}
%             \half,\quad n=0\;\text{or}\; n=N_t,\\
%             1,\quad\text{otherwise}, 
%            \end{cases}\\
%     &\mu_j^{n+1}=2\mu_j^n-\mu_j^{n-1}-\frac{\widetilde{\omega}^2}{\omega^2}\Dt^2 \mu_j^n\lambda_{j}^2,\quad 0\leq n\leq N_t-1,\\
%     &\mu_j^0 = 1, \quad \mu_j^{-1}=\mu^0+\frac{\widetilde{\omega}^2}{\omega^2}\frac{\Dt^2}{2}\lambda_{j}^2.
% \end{align}
% \end{subequations}





% %%%%%%%%%%%%%%%%%%% 
% \section{Deflated conjugate gradient (DCG) method\label{sec:dcg}} 
% With energy conserving boundary conditions, the WaveHoltz method for Helmholtz equation or time-harmonic Maxwell's equations results in an SPD linear system, allowing CG method to solve it. However, energy conserving boundary conditions lead to trapped wave structures, and the number of iterations for convergence needed by CG scales as $O(\omega^{d})$ in the worst case, where $d$ is the dimension of the problem. For 3D high frequency problem, many iterations may be required, resulting in a high computational cost, especially when solutions corresponding to many right-hand sides are desired.

% To accelerate the convergence of the WaveHoltz method for such cases, we apply the deflated conjugate gradient (DCG) method \cite{saad2000deflated} by adding (approximated) eigenvectors associated with the smallest eigenvalues to the Krylov subspace.
 
% In this section, we will first review the DCG algorithm and its convergence theory \cite{saad2000deflated} in Sec. \ref{sec:dcg_algorithm}, and then discuss how to choose the deflation space in Sec. \ref{sec:deflation} and Sec. \ref{sec:deflation-band}.  
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{DCG algorithm  and its convergence theory \label{sec:dcg_algorithm}}
% %Assume $A$ is a SPD linear system. %Particularly, we denote $A$ as $A_h$ if it is corresponding to a discrete operator derived from a finite difference approximation of a partial differential equation (PDE) with mesh size $h$.


% Consider an SPD linear system $A\xb=\bbb\in\mathbb{R}^N$. Given an initial guess $\xb_0$, in the $k$-th iteration, the CG method seeks the solution $\xb_k$ in the Krylov subspace 
% \begin{equation}
%     \xb_0+\mathcal{\Na}(\rb_0,\whiA,k)=\xb_0+\{\rb_0,\whiA\rb_0,\dots,\whiA^{k-1} \rb_0\},\quad \rb_0=\bbb-\whiA\xb_0,
% \end{equation}
% corresponding to the optimal error with respect to the $||\cdot||_A$ norm,  $||\yb||_A=\sqrt{\yb^T\whiA\yb}$. In other words,
% \begin{align*}
% \xb_k = \min_{\hat{\xb} \in \xb_0+\mathcal{\Na}(\rb_0,\whiA,k)}||\xb-\hat{\xb}||_A.
% \end{align*}
% The DCG method augments the Krylov subspace  with a deflation space, which is the column space of a deflation matrix $W\in\mathbb{R}^{N\times \Na}$. The DCG method initializes $\xb_0$ in the deflation space such that $$W^TA(\xb_0-\bbb)=W^T\rb_0=0$$ and performs a CG search in the subspace $A$-orthogonal to the deflation space. 
% This strategy results in the DCG algorithm \cite{saad2000deflated}, which is presented in Algorithm \ref{alg:DCG}.

% As discussed in \cite{saad2000deflated}, the DCG method can be seen as a preconditioned CG method with the preconditioner $PP^T$, where $P$ is the projector onto the $A$-orthogonal complement of the deflation space determined by $W$:
% \begin{equation}
%     P = I-W(W^TA W)^{-1}W^TA.
% \end{equation}
% Utilizing this point of view, the convergence speed of the DCG method is analyzed in \cite{saad2000deflated}. 
% \begin{thm}\label{thm:dcg}
% (Theorem 4.3 of \cite{saad2000deflated})
% Let $\kappa_{P^TAP}$ be the condition number of $P^TAP$. The approximated solution of $A\xb=\bbb$ generated by the $j$-th iteration of the DCG algorithm in Algorithm \ref{alg:DCG} satisfies
% \begin{equation}
%     ||\xb-\xb_j||_A\leq2\left(\frac{\sqrt{\kappa_{P^TAP}}-1}{\sqrt{\kappa_{P^TAP}}+1}\right)^j|| \xb-\xb_0||_A, \quad ||\yb||_A=\sqrt{\yb^TA\yb}.
% \end{equation} 
% \end{thm}


% %If eigenvectors corresponding to smallest eigenvalues of $\whiA$ are inside or well approximated by vectors in the deflation space $W$, the convergence of CG will be accelerated.
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{algorithm}
% \caption{DCG($\whiA,\bbb,W$): deflated conjugate gradient to solve $\whiA\xb=\bbb$ with the deflation matrix $W$.}\label{alg:DCG}
% \begin{algorithmic}[1]
% \State Input: $\whiA$, $\bbb$ and $W$.
% \State $\xb_{-1}=0$
% \State $\rb_{-1} = \bbb-\whiA \xb_{-1}$
% \State $\xb_0 =  \xb_{-1} + W (\matW^T \whiA \matW)^{-1} ( \matW^T \rb_{-1} )$
% \State $ \rb_0 = \bbb - \whiA \xb_0 $
% \State $\etab_0 = \matW^T \whiA \rb_0$
% \State $ {\bm \mu_0} = (\matW^T \whiA \matW)^{-1} \etab_0$
% \State $ \pb_0 = \rb_0 - \matW {\bm \mu_0}$
% \State $ r_2 = \rb^T \rb$
% \State $ r_0 = r_2$
% \State $k\ge 0$
% \While{$r_2/r_0 > {\rm (TOL)}^2$ }
%  \State  $\qb_k  = \whiA \pb_k$
%  \State  $\alpha_k \gets r_2/ (\pb_k^T \qb_k)$
%  \State  $\xb_{k+1} = \xb_k + \alpha_k \pb_k$
%  \State  $ \rb_{k+1} = \rb - \alpha_k \qb$
%  \State  $ \hat{r}_2 \gets r_2$
%  \State  $ r_2 \gets \rb_{k+1}^T \rb_{k+1}$
%   \State  $ \beta_{k+1} \gets  r_2/\hat{r}_2$
%  \State $\etab_{k+1} = \matW^T \whiA \rb_{k+1}$
%  \State $ {\bm \mu_{k+1}}= (\matW^T \whiA \matW)^{-1} \etab_{k+1}$
%   \State  $ \pb_{k+1} = \beta_{k+1} \pb_k+\rb_{k+1} - \matW \mu_{k+1}$
%   \State $k \gets k+1$
% \EndWhile
% \end{algorithmic}
% \end{algorithm}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{algorithm}
% \caption{Eig-DCG($\whiA,\bbb,W$): eigenvector deflated conjugate gradient to solve $\whiA\xb=\bbb$.}\label{alg:eig-DCG}
% \begin{algorithmic}[1]
% \State Input: $\whiA$, $\bbb$ and $W$.
% \State $\xb_{-1}=0$
% \State $\rb_{-1} = \bbb-\whiA \xb_{-1}$
% \State $\xb_0 =  \xb_{-1} + W (\matW^T \whiA \matW)^{-1} ( \matW^T \rb_{-1} )$
% \State $ \rb_0 = \bbb - \whiA \xb_0 $
% \State $\etab_0 = \matW^T \whiA \rb_0$
% \State $ {\bm \mu_0} = (\matW^T \whiA \matW)^{-1} \etab_0$
% \State $ \pb_0 = \rb_0 - \matW {\bm \mu_0}$
% \State $ r_2 = \rb^T \rb$
% \State $ r_0 = r_2$
% \State $k\ge 0$
% \While{$r_2/r_0 > {\rm (TOL)}^2$ }
%  \State  $\qb_k  = \whiA \pb_k$
%  \State  $\alpha_k \gets r_2/ (\pb_k^T \qb_k)$
%  \State  $\xb_{k+1} = \xb_k + \alpha_k \pb_k$
%  \State  $ \rb_{k+1} = \rb - \alpha_k \qb$
%  \State  $ \hat{r}_2 \gets r_2$
%  \State  $ r_2 \gets \rb_{k+1}^T \rb_{k+1}$
%   \State  $ \beta_{k+1} \gets  r_2/\hat{r}_2$
%   \State  $ \pb_{k+1} = \beta_{k+1} \pb_k+\rb_{k+1}$
%   \State $k \gets k+1$
% \EndWhile
% \end{algorithmic}
% \end{algorithm}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \begin{rem}
% The main modifications to the CG algorithm made by the deflation method are as follows.
% The line $3$ of Algorithm \ref{alg:DCG} constructs  an initial guess $\xb_0\in W$ such that  
% \begin{align*}
% W^T\rb_0 &= W^T(\bbb-\whiA\xb)=W^T\bbb - W^T\whiA\left(\xb_{-1}+AW(W^TAW)^{-1}W^T\rb_{-1}\right)\notag\\
%          &=W^T\bbb - W^T\whiA\xb_{-1}+W^TAW(W^TAW)^{-1}W^T\rb_{-1}= W^T\rb_{-1}-W^T\rb_{-1}=0.
% \end{align*}
% Line $5,6,20$ and $21$ of Algorithm \ref{alg:DCG} enforce the search direction $\pb_{k}$ to be $A$-orthogonal to the deflation space $W$.
% \end{rem}







% \subsection{Eigenvector and prolonged eigenvector deflation matrix \label{sec:deflation}}
% When eigenvectors are used as the deflation matrix, after initialization through the projection onto the deflation space which is a span of eigenvectors, the Krylov vectors generated by the CG algorithm is always $A$-orthogonal to each other \cite{saad2000deflated}. In other words, when eigenvectors are chosen as the deflation matrix, line 20-22 in Alg. \ref{alg:DCG} enforcing $A$-orthogonality after each iteration is not necessary. Dropping these unnecessary lines result in the simplified eigenvector deflated DCG (eig-DCG) algorithm in Alg. \ref{alg:eig-DCG}.


% However, the computational cost of directly computing eigenvectors sometimes could be unaffordable. Alternatively, we can approximate eigenvectors through prolongation from coarser meshes. Let $A_h$ represent a linear system originating from a spatial discretization using mesh size $h$. We can use prolonged eigenvectors obtained  through linear interpolation of eigenvectors from coarser meshes (e.g., eigenvectors $A_{2h},A_{4h}$). On one hand, these prolonged eigenvectors can be obtained with less computational cost. On the other hand, using prolonged eigenvectors breaks the $A$-orthogonality required by the simplified Algorithm in Alg. \ref{alg:eig-DCG}. As a result, we need to use the original DCG method in Alg. \ref{alg:DCG} which enforces $A$-orthogonality in every iteration, otherwise DCG may lose its robustness \cite{saad2000deflated}. 

% The condition number of the eigenvector-deflated system $P^TAP$ is discussed in Sec. 5 of \cite{saad2000deflated}, and we summarize it as a theorem here.
% \begin{thm}(Sec. 5 of \cite{saad2000deflated})\label{lem:kappa}
% Let the eigenvalues of $A$ be $0< \tilde{\lambda}_1\dots\leq\tilde{\lambda}_N$. If the columns of the deflation matrix 
% $$W=\left(\wb_1,\wb_2,\dots,\wb_K\right)$$ are  eigenvectors corresponding to $\tilde{\lambda}_1,\dots,\tilde{\lambda}_K$, then the condition number of  $P^TAP$
% is $\kappa_{P^TAP}=\frac{\tilde{\lambda}_N}{\tilde{\lambda}_{\Na+1}}$.
% \end{thm}
% The eigenvector deflation essentially reduces the condition number of the linear system from $\frac{\tilde{\lambda}_N}{\tilde{\lambda}_1}$ to $\frac{\tilde{\lambda}_N}{\tilde{\lambda}_{\Na+1}}$. When eigenvectors of the system $A_h$ are well approximated on a coarse mesh, using prolonged eigenvectors as the deflation matrix leads to a deflated system whose condition number is close to $\tilde{\lambda}_N/\tilde{\lambda}_{\Na+1}$.
% A key difference between the eigenvector and prolonged eigenvector deflation is as follows. When columns of $W$ are eigenvectors of $A_h$, one can easily verify that $W^TA_hW$ is a diagonal matrix whose $k$-th diagonal element is $\tilde{\lambda}_k$. Thus, the computational cost of applying $(W^TA_hW)^{-1}$ is $O(\Na)$.
% However, when prolonged eigenvectors are utilized, $W^TA_hW$ is not diagonal, potentially increasing the computational cost of applying $(W^TAW)^{-1}$ to $O(\Na^2)$.


% \begin{rem}
% As demonstrated in Appx. \ref{sec:A-orthogonality}, using exact eigenvector deflation eliminates the need to perform line $5,6,20$ and $21$ of Alg \ref{alg:DCG} to enforce $A$-orthogonality. However, in practice, we still execute these lines due to numerical considerations. Eigenvectors of $A$ are usually numerically computed. Without executing these lines of Alg. \ref{alg:DCG}, accumulations of numerical errors over iterations may lead to the loss of $A$-orthogonality. This loss further causes slower convergence.
% \end{rem}

% \begin{rem}
% As pointed out in \cite{kruvzik2018implementace}, besides (approximated) eigenvectors, there are alternative choices for the deflation matrix. For example, it can also be chosen as a prolongation matrix from a geometric or an algebraic multigrid method  \cite{dwarka2020scalable}, subdomain aggregation \cite{nicolaides1987deflation} and discrete Wavelet compression \cite{kruzik2017wavelet}. 
% \end{rem}

% \begin{rem}
% In an abstract formulation, authors of \cite{tang2010comparison} systematically analyze and compare the deflation method and the two-grid method \cite{mandel1993balancing}. They prove that, with careful design, a prolongation based deflation method can achieve almost the same convergence property as a two-grid method.
% \end{rem}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Same deflation for a narrow frequency band\label{sec:deflation-band}}
% As discussed in Sec. \ref{sec:waveholtz-eig}, the discrete WaveHoltz operator shares identical eigenvectors with the discrete Laplacian operator for any frequency $\omega$. The eigenvectors corresponding to the smallest eigenvalues of the WaveHoltz operators for frequencies in a sufficiently narrow frequency bands are almost identical. Therefore, a shared deflation matrix may be utilized for various frequencies in a narrow band.






% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \section{Convergence speed of deflated WaveHoltz method\label{sec:waveholtz_deflation}}%\pzc{To-do: \cite{kahl2017deflated} analyzed how error of eigenvector computations influence convergence, we can probably use their theories to analyze the mulitilevel deflation as well.}

% To accelerate the convergence of the WaveHoltz method for energy conserving problems with trapped wave structures, we apply the DCG algorithm with eigenvectors or prolonged eigenvectors as the deflation matrix.
% Here, we formally analyze the relation between the number of  eigenvectors in the deflation space and the convergence speed. 
% For simplicity, we consider a homogeneous velocity field with $c(\xb)=1$. We first present the analysis results in Sec. \ref{sec:analysis-result}, followed by details of the analysis  in Sec. \ref{sec:analysis-procedure}. 


% \subsection{Relation between the number of eigenvectors and computational costs\label{sec:analysis-result}}
% Assume a homogeneous velocity field $c(\xb)=1$, which allows us to utilize the Weyl's principle \cite{weyl1912asymptotische} to formally estimate the relation between the dimension of the eigenvector deflation space and the number of iterations needed for convergence of DCG. In this section, we present our main results.

% \textbf{Relation between number of eigenvectors and number of iterations for convergence.} Assume $W$ comprising eigenvectors corresponding to the $\Na$ smallest eigenvalues of the discrete WaveHoltz operator $A=I-S_h$. With  sufficiently high frequency $\omega$,  sufficiently small mesh size $h$ and time step size $\Dt$, the DCG algorithm solving $A\ub=(I-S_h)\ub=\bbb$ converges with $$N^{\textrm{DCG}}_{\textrm{iter}}\approx\frac{C_{\textrm{iter}}}{\Na}$$  iterations, where $C_{\textrm{iter}}$ represents a constant.

% \textbf{Computational cost of the DCG in Alg. \ref{alg:DCG} and Eig-DCG in Alg. \ref{alg:eig-DCG} with the eigenvector deflation.}  When eigenvector deflation is applied, the deflation matrix $W\in\mathbb{R}^{N_{\textrm{DOF}}\times \Na}$ is a dense matrix, and $W^TAW\in\mathbb{R}^{\Na\times \Na}$ is a diagonal matrix leading to $O(\Na)$ computational cost of applying $(W^TAW)^{-1}$. Additionally, the matrix $W^TA\in\mathbb{R}^{N_{\textrm{DOF}}\times \Na}$ is dense and can be pre-computed. 
% Utilizing these facts, computational cost of each step in the DCG algorithm is  estimated and summarized in Tab. \ref{tab:dcg-cost}.
% \begin{table}[htbp]
%   \centering
%  \medskip
%     \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|}
%     \hline
% 	& Vector Operations  & Apply A  & Apply $W^TA$  & Apply $(W^TAW)^{-1}$ & Apply $W$  \\ \hline
%  Line in Alg. \ref{alg:DCG} & $14-19, 22$ & $13$ & $20$ & $21$ & $22$ \\ \hline
%  Cost &	$O(N_{\textrm{DOF}})$ & $N_tO(N_{\textrm{DOF}})$ & $KO(N_{\textrm{DOF}})$ & $O(\Na)$ & $KO(N_{\textrm{DOF}})$ \\
%  	\hline
%  \end{tabular}
%       \caption{Computational cost of each steps in the DCG method Alg. \ref{alg:DCG} with the eigenvector deflation.\label{tab:dcg-cost}}
% \end{table}

% DCG converges with approximately $C_{\textrm{iter}}/\Na$ iterations. 
% Consequently, the total cost of solving the WaveHoltz system $A\xb=(I-S_h)\xb=\bbb$ with DCG can be estimated as follows:
% \begin{align}
% \textrm{Cost}_{\textrm{DCG}} &\approx N^{\textrm{DCG}}_{\textrm{iter}}\times
% \Big( \textrm{Vector Operations (line 14-19, 22)} + \textrm{Apply A (line 13)}\notag\\
% &\quad\quad+\textrm{Apply $W^TA$ (line 20)} + \textrm{Solve $W^TAW$ (line 21)}+\textrm{Apply $W$ (line 22)}\Big)\notag\\
% &= \frac{C_{\textrm{iter}}}{\Na}\times
% \big(  O(N_\textrm{DOF})+N_t O(N_\textrm{DOF})+\Na O(\textrm{DOF})+O(\Na)\big)\notag\\
% &=C_{\textrm{iter}}O(N_\textrm{DOF})\left(\frac{C_tN_t+C^{\textrm{DCG}}_{\textrm{vec}}}{\Na}+C_W+C_{W^TA}\right).\label{eq:cost19}
% \end{align}
% where $C_t, C^{\textrm{DCG}}_{\textrm{vec}},C_W$ and $C_{W^TA}$ 
%  are constants. As a result, we would expect a sub-linear acceleration as we increase the number of eigenvectors $\Na$. 

% Similarly, the cost of Eig-DCG with $\Na$-eigenvectors as the deflation amtrix can be estimated as:
% \begin{align}
% \textrm{Cost}_{\textrm{Eig-DCG}} &\approx N^{\textrm{Eig-DCG}}_{\textrm{iter}}\times
% \Big( \textrm{Vector Operations (line 14-20)} + \textrm{Apply A (line 13)}\Big)\notag\\
% &= \frac{C_{\textrm{iter}}}{\Na}\times
% \big(  O(N_\textrm{DOF})+N_t O(N_\textrm{DOF})\big)\notag\\
% &=C_{\textrm{iter}}O(N_\textrm{DOF})\left(\frac{C_tN_t+C^{\textrm{Eig-DCG}}_{\textrm{vec}}}{\Na}\right).\label{eq:cost19}
% \end{align}
% where $C_t, C^{\textrm{DCG}}_{\textrm{vec}},C_W$ and $C_{W^TA}$ 
%  are constants. 
 

% Without deflation, the computational cost of solving the WaveHoltz system with CG is approximately
% \begin{align}
% \textrm{Cost}_{\textrm{CG}} &\approx N^{\textrm{CG}}_{\textrm{iter}}\times
% \left( \textrm{Vector Operations} + \textrm{Apply A }\right)\notag\\
% &= N^{\textrm{CG}}_{\textrm{iter}} O(N_{\textrm{DOF}})(C_tN_t+C^{\textrm{CG}}_{\textrm{vec}}).
% \end{align}
% Therefore, the relative computational cost of the DCG method (Alg. \ref{alg:DCG}) and Eig-DCG method (Alg. \ref{alg:DCG}) with respect to the CG method are approximately
% \begin{subequations}
% \begin{align}
% \textrm{Relative Cost of DCG}&=\frac{\textrm{Cost}_{\textrm{DCG}}}{\textrm{Cost}_{\textrm{CG}}} \approx 
%     \frac{C_{\textrm{iter}}}{N_{\textrm{iter}}^{\textrm{CG}}}\left(\frac{\frac{1}{\Na}\left(C_tN_t+C^{\textrm{DCG}}_{\textrm{vec}}\right)+\left(C_W+C_{W^TA}\right)}{C_tN_t+C^{\textrm{CG}}_{\textrm{vec}}}\right),\\
%   \textrm{Relative Cost of Eig-DCG}&=  \frac{\textrm{Cost}_{\textrm{DCG}}}{\textrm{Cost}_{\textrm{CG}}} \approx 
%     \frac{C_{\textrm{iter}}}{N_{\textrm{iter}}^{\textrm{CG}}}\left(\frac{\frac{1}{\Na}\left(C_tN_t+C^{\textrm{Eig-DCG}}_{\textrm{vec}}\right)}{C_tN_t+C^{\textrm{CG}}_{\textrm{vec}}}\right).
% \end{align}
% \end{subequations}
% In comparison with CG, DCG has overheads for applying $W$, $W^TA$ and $(W^TAW)^{-1}$ in each iteration, but it converges with fewer total iterations. Overall, with a proper chosen $\Na$, DCG achieves acceleration over CG. 



% When prolonged eigenvectors are leveraged, the matrix $W^TAW$ is not diagonal anymore, potentially increasing the cost of applying $(W^TAW)^{-1}$ to $O(\Na^2)$. If eigenvectors on the fine mesh are well approximated by the prolonged eigenvectors from the coarse mesh, the estimated computational cost of solving the WaveHoltz system with DCG becomes
% \begin{equation}
% C_{\textrm{iter}}O(N_\textrm{DOF})\left(\frac{C_tN_t+C^{\textrm{DCG}}_{\textrm{vec}}}{\Na}+C'_W+C'_{W^TA}\right)+C'_{W^TAW} O(\Na)\label{eq:prolong_cost}
% \end{equation}
% where
% $C'_W,C'_{W^TA},C'_{W^TAW}$ are constants. In practice, the number of eigenvectors in the deflation space, $\Na$, is much smaller than the total number of degrees of freedom $N_{\textrm{DOF}}$, and the $O(\Na)$ term in the computational cost \eqref{eq:prolong_cost} is almost negligible. We still expect a sub-linear acceleration, as we increase the number of eigenvectors $\Na$. 

% %Since the cost of  applying the WaveHoltz operator is dominant, enlarging the number of prolonged eigenvectors $\Na$ initially results in computational saving. However, there may be no computational saving or even more computational costs when $\Na$ becomes too large.     

% In our numerical tests, we observe that using a moderate number of eigenvectors or prolonged eigenvectors as the deflation matrix, we are able to gain almost linear acceleration over CG.%computational saving compared to CG. 

% % \input tex/convergence_analysis.tex

% \section{Numerical experiments\label{sec:numerical}}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% To demonstrate the effectiveness of the proposed deflated  WaveHoltz method, we test it with a series of numerical examples. All the code is implemented in the {\tt Julia} programming language.

% For problems with known analytical forms of eigenvalues and eigenvectors, we directly use their analytical form. For problems without known analytical forms, we use the Lanczos algorithm implemented in the {\tt KrylovKit.jl} package \cite{krylovkit} to compute the smallest eigenvectors of the WaveHoltz operators. In the Lanczos algorithm, the dimension of the Krylov space is set as $N_{\Na}=\max(2K,4\textrm{-ceil}(\omega))$, where $\Na$ is the desired number of eigenvectors, and $\omega$ is the frequency of the underlying problem. 

% We define the relative number of iterations for convergence of DCG compared to CG
% as
% \begin{equation}
% \textrm{Iter}_{\textrm{rel}}=\textrm{Iter}_{\textrm{DCG}}/\textrm{Iter}_{\textrm{CG}},
% \end{equation}
% where $\textrm{Iter}_{\textrm{CG}}$ and $\textrm{Iter}_{\textrm{DCG}}$ are number of iterations for convergence needed by CG and DCG respectively. Similarly, we can define relative computational of DCG compared to CG.


% All the 2D tests are performed on an iMac machine with the Apple M1 chip, while all the 3D tests are conducted on the High Performance Community Computing Cluster (HPC3) of the Hong Kong University of Science and Technology (HKUST).

% \clearpage
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{2D homogeneous problem\label{sec:2d-h}}
% \deaa{Our first experiment for a case where the eigenvectors are known and thus can be easily found. A purpose of this experiment is to experimentally assess the various constants in cost estimate (\ref{eq:cost19})} 



% We first consider a 2D homogeneous problem in the computational domain $[0,1]^2$ with the velocity field $c^2(x,y)=1$. A point source is located at $(x,y)=(0.1,0.1)$. For frequencies $\omega=25$ and $50$, we use a uniform mesh with $N=16\omega+1$ grid points in each direction. The relative tolerances in the stopping criteria for CG and DCG are set to $10^{-9}$.

% \textbf{Prolonged eigenvectors as the deflation matrix.} The eigenvectors and eigenvalues for the discrete Laplacian operator are known analytically for this homogeneous problem. Therefore, following Sec. \ref{sec:waveholtz-eig}, we analytically compute the eigenvalues and eigenvectors of the discrete WaveHoltz operator. We compare the performance of using eigenvectors and prolonged eigenvectors as the deflation matrix. As presented in Fig. \ref{fig:2d_coarse_deflation},  using eigenvectors and approximated eigenvectors prolonged from $1$ to $3$-level coarsened meshes as the deflation matrix has similar performance. As the number of eigenvectors $\Na$ increases, the number of iterations for conevergence needed by DCG initially scales as approximately $O(\Na^{-0.85})$, and eventually bottom out. Computational time of DCG scales approximately $O(\Na^{-0.82})$. Compared to CG, DCG achieves at most approximately  $8$ times acceleration for $\omega=25$ and approximately  $25$ times acceleration for $\omega=50$.


% %\textbf{Rectangle domain with different aspect ratios.} We consider a homogeneous rectangular domain $[0,1]\times[0,r]$ with frequency $\omega=150$ and PEC boundary conditions, where $0<r\leq 1$ is the aspect ratio. We use a uniform mesh with $601$ grid points along $x$-direction and $\lceil600r\rceil+1$ grid points alogn $y$-direction. Results are summarized in Fig. \ref{fig:2d_rectangle}.
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{figure}[htb] 
% \begin{center}
% \includegraphics[width=0.4\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/iter_2d_h1.eps}\hspace{0.2cm}
% \includegraphics[width=0.4\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/iter_2d_h2.eps}
% \includegraphics[width=0.4\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/time_2d_h1.eps}\hspace{0.2cm}
% \includegraphics[width=0.4\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/time_2d_h2.eps}
% \caption{Relative and absolute number of iterations for convergence and computational time of DCG compared to CG for the 2D homogeneous problem in Sec. \ref{sec:2d-h}. Top: relative number of iterations for convergence. Bottom: relative computational time. \label{fig:2d_coarse_deflation}}
% \end{center}
% \end{figure}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %\begin{figure}[htb]
% %\begin{center}
% %\includegraphics[width=0.4\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/iter_2d_h_rectangle.eps}
% %\includegraphics[width=0.4\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/iter_2d_h2.eps}
% %\caption{Relative number of iterations and computational time compared to CG for the 2D homogeneous problem in Sec. \ref{sec:2d-h}. \label{fig:2d_rectangle}}
% %\end{center}
% %\end{figure}

% \clearpage

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{2D inhomogeneous problem\label{sec:2d-ih}}
% We consider a 2D problem in the computational domain $[-1,1]^2$ with the velocity field 
% \begin{equation}
%     c^2(x,y) = 1.0-0.9\left( e^{-\left(\frac{x^2+(y-0.4)^2-0.4^2}{0.2^2} \right)^4}+e^{-\left(\frac{x^2+(y+0.4)^2-0.3^2}{0.2^2} \right)^4}\right).
% \end{equation}
% We consider frequencies $\omega=20,40,60$ and the source term
% \begin{equation}
%     f(x,y) = \frac{16\omega^2}{\pi}e^{-16\omega^2(x^2+y^2)}.
% \end{equation}
% We use a mesh with $N=8\omega$+1 grid points in each direction. The relative tolerances in the stopping criteria of CG and DCG are set as $10^{-10}$.
% The tolerance of the residual for Schur vectors in the Lanczos algorithm to generate eigenvectors is $10^{-12}$.
% The configuration of the velocity field and numerical solutions for frequencies $\omega=20,60$ are displayed in Fig. \ref{fig:reference-2d-ih}.

% \textbf{Performance with different dimensions of the deflation space.} In Fig. \ref{fig:convergence_2d_ih}, we present the performance of DCG with different dimensions of the deflation space. The relative number of iterations  for convergence and relative computational time compared to the CG method approximately scale  as $O(\Na^{-0.9})$. With $50$ to $200$ eigenvectors, DCG achieves approximately $2.23$ to $15.39$ times acceleration compared to CG. As shown in the right picture of Fig. \ref{fig:convergence_2d_ih}, the computational time of obtaining eigenvectors corresponding to smallest eigenvalues takes approximately $3.25$ to $4.93$ times of CG.  %Accounting for the computational time of obtaining eigenvectors, we gain computational saving if solutions for more than $5$ to $8$ different right-hand sides are desired.

% \textbf{Same deflation matrix for a  frequency band.} We utilize a uniform grid with $321$ grid points in each direction. Eigenvectors corresponding to the smallest $200$ eigenvalues of the WaveHoltz operator for the frequency $\omega=40$ serve as the deflation matrix for $\omega\in[37.5,42.5]$. The relative number of iterations for convergence and computational time of DCG compared to CG are displayed in Fig. \ref{fig:2d_windowed_deflation}. We observe that, for the frequency band $[37.5,42.5]$, DCG consistently converges with fewer iterations and smaller computational time than CG. Moreover, the closer the frequency to $\omega=40$, the greater the acceleration is achieved. 
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{figure}[htb]
% \begin{center}
% \includegraphics[width=0.32\textwidth,trim={1.5cm 0.15cm 2.5cm 0.25cm},clip]{figures/c_square_2d_ih.eps}
% \includegraphics[width=0.32\textwidth,trim={1.5cm 0.15cm 2.5cm 0.25cm},clip]{figures/sol_2d_ih_20.eps}
% %\includegraphics[width=0.40\textwidth,trim={1.5cm 0.15cm 2.5cm 0.25cm},clip]{figures/sol_2d_ih_40.eps}
% \includegraphics[width=0.32\textwidth,trim={1.5cm 0.15cm 2.5cm 0.25cm},clip]{figures/sol_2d_ih_60.eps}
% \caption{Configuration of the velocity field and  numerical solutions for the inhomogeneous 2D problem in Sec. \ref{sec:2d-ih}. \label{fig:reference-2d-ih}}
% \end{center}
% \end{figure}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{figure}[htb]
% \begin{center}
% \includegraphics[width=0.32\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/iter_2d_ih.eps}
% \includegraphics[width=0.32\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/time_2d_ih.eps}
% \includegraphics[width=0.32\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/eig_time_2d_ih.eps}
% \caption{Results for the 2D inhomogeneous 
%  problem in Sec. \ref{sec:2d-ih}. Left:  relative and absolute number of iterations with respect to the CG method. Middle: relative computational time with respect to the CG method. Right: relative  eigenvector computational time with respect to the CG method.\label{fig:convergence_2d_ih}}
% \end{center}
% \end{figure}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{figure}[htb]
% \begin{center}
% \includegraphics[width=0.4\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/iter_window_40.eps}
% \includegraphics[width=0.4\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/iter_window_40_zoomed_in.eps}
% \caption{Relative number of iterations and computational time of DCG compared to CG for the 2D inhomogeneous problem in Sec. \ref{sec:2d-ih}. \label{fig:2d_windowed_deflation}}
% \end{center}
% \end{figure}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{3D homogeneous cube \label{sec:convergence_test_3d}}
% We consider a 3D homogeneous problem with $c(x,y,z)=1$ and a point source term $\delta(x-0.1,y-0.1,z-0.1)$ in the computational domain $[0,1]^3$. We consider three different frequencies $\omega=20,\;25,\;30$. We partition the computation domain with a uniform mesh having $131$ grid points for $\omega = 20$, $181$ grid points for $\omega=25$ and $231$ grid points for $\omega=30$ in each direction. These number of grid points per direction is chosen based on the in the principle determining points per wave length to reach at least $2\%$ relative error. \pzc{cite Bill's paper here}. We set the relative tolerance in the stopping criteria of the CG and DCG solver as $10^{-9}$.

% \textbf{Performance with different dimensions of the deflation space.} For this homogeneous medium, the eigenvalues of the the discrete WaveHoltz operator can be analytically computed. Based on this fact, we estimate the condition number of the deflated operator by $\frac{1.5}{\hat{\lambda}_{\Na+1}}$, where $\hat{\lambda}_{\Na+1}$ is the $\Na+1$-th smallest eigenvalue of the discrete WaveHoltz operator. The estimated condition number is displayed in the bottom left plot of Fig. \ref{fig:convergence_test_3d}. We observe that the estimated condition number approximately scales as $O(\Na^{-2})$  for all frequencies, where $\Na$ is the number of eigenvectors in the deflation space. This observation matches our analysis.

% In the top and bottom right plots of Fig. \ref{fig:convergence_test_3d}, we present the number of iterations for convergence and relative computational time with respect to the CG method. For all frequencies, the number of iterations for convergence scales roughly as $O(\Na^{-0.9})$ before bottoming out. The relative computational time of DCG with respect to CG scales roughly as $O(\Na^{-0.9})$. In comparison with CG, when $\Na=300$, DCG achieves at most more than $10.46$ times acceleration for $\omega=20$,  $8.40$ times acceleration for $\omega=25$ and $10.01$ times acceleration for $\omega=30$. 

% \textbf{Prolonged eigenvectors as the deflation matrix.} In Fig. \ref{fig:convergence_test_3d_window}, we compare the number of iterations for convergence  and computational time using prolonged eigenvectors and analytical eigenvectors. We observe that, for frequencies $\omega=20,25,30$, employing prolonged eigenvectors from the $1$-level or $2$-level coarsened mesh, DCG converges with number of iterations comparable to using fine level eigenvectors. However, using prolonged eigenvectors requires enforcing $A$-orthogonality in each iteration. As a result, the speed-up gained by using prolonged eigenvectors is less compared to using the fine level eigenvectors. 


% In summary, prolonged eigenvectors as the deflation matrix performs well when the fine level eigenvectors are well approximated on the coarse mesh, otherwise it may suffer from significant efficiency decline.

% \begin{figure}[htb]
% \begin{center}
% \includegraphics[width=0.32\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/iter_3d_20.eps}
% \hspace{0.1cm}
% \includegraphics[width=0.32\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/iter_3d_25.eps}
% \hspace{0.1cm}
% \includegraphics[width=0.32\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/iter_3d_30.eps}
% \includegraphics[width=0.32\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/cond_3d.eps}
% \includegraphics[width=0.32\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/time_3d.eps}
% \caption{Results for the 3D  homogeneous cube in Sec. \ref{sec:convergence_test_3d}. Top: relative and absolute number of iterations. Bottom left: estimated conditional number of $W^TAW$. Bottom right: relative computational time with respect to the CG method.   \label{fig:convergence_test_3d}}
% \end{center}
%  \end{figure}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  \begin{figure}[htb]
% \begin{center}
% \includegraphics[width=0.32\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/iter_3d_ml_20.eps}
% \includegraphics[width=0.32\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/iter_3d_ml_25.eps}
% \includegraphics[width=0.32\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/iter_3d_ml_30.eps}
% \includegraphics[width=0.32\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/time_3d_ml_20.eps}
% \includegraphics[width=0.32\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/time_3d_ml_25.eps}
% \includegraphics[width=0.32\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/time_3d_ml_30.eps}
% \caption{Performance of DCG for 3D  homogeneous cube with deflation matrices comprising prolonged eigenvectors  in Sec. \ref{sec:convergence_test_3d}.  Top: relative and absolute number of iterations for convergence. Bottom: relative computational time compared to CG. \label{fig:convergence_test_3d_window}}
% \end{center}
%  \end{figure}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{3D homogeneous ball\label{sec:3d-ball}}
% We consider a 3D homogeneous problem   ball
% $\{(x,y,z):\sqrt{x^2+y^2+z^2}\leq0.5\}$ 
% with $c^2(\xb)=1$ and homogeneous boundary conditions. The source term is defined as
% \begin{equation}
%     f(x,y,z) = \frac{16\omega^2}{\pi}e^{-16\omega^2( (x-x_c)^2+(y-y_c)^2+(z-z_c)^2 )},
% \end{equation}
% where $\omega=25$ is the frequency of the underlying problem. The relative tolerances in the stopping criteria of CG and DCG are $10^{-9}$.

% To handle the curvilinear geometry, we utilize the second order embedded  boundary (EB) finite difference method in \cite{peng2023universal}. This EB method use interior boundary points leads to a SPD discrete Laplacian operator, so CG solver can still be applied. Moreover, it also avoids small cell stiffness, so a standard CFL condition can still be used in the time-domain simulation of the wave equation.
% In the EB method, we set computational domain as $[-0.55,0.55]^3$  and partition it by a uniform cartesian mesh with $220$ grid points in each direction. 

% To construct the deflation matrix, we use Lanczos method to compute $100$ eigenvectors  and obtain $123$ converged eigenvectors. The tolerance of the residual for Schur vectors in the Lanczos algorithm is set as $10^{-10}$. The deflation matrix consists of all converged eigenvectors.

% \textbf{Different source terms.} To test the performance of the proposed DCG methods for different source terms, we uniformly  pick $10$ different random center points for the source term $(x_c,y_c,z_c)$ inside the ball $\{\sqrt{x^2+y^2+z^2}\leq0.25\}$.

% Results are summarized in Tab. \ref{tab:3d-ball}. We observe that, on average, the DCG algorithm converges with approximately $18.90\%$ number of iterations and leads to approximately $3.60$ times acceleration compared to CG. 
% The computational time of constructing the deflation matrix is approximately $11.105$ times of the average time for one CG solve. As a result, we gain computational saving if the Helmholtz equation is solved for more than $16$ different source terms.   

% \textbf{Same deflation for a narrow frequency band.} We use the deflation matrix constructed for $\omega=25$ to solve problems with $\omega=24.5,24.6,\dots,30.5$ and the source term corresponding to $(x_c,y_c,z_c)=(0.1,0.1,0.1)$. As displayed in Fig. \ref{fig:3d_ball_windowed_deflation}, we observe that, for all frequencies, DCG converges with less number of iterations than CG and achieves approximately $4.00$ to $5.21$ times acceleration compared to CG. %Surprisingly, though the deflation matrix consists of eigenvectors for $\omega=40$, we achieve the largest acceleration at $\omega=40.3$. 
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{table}[htbp]
%   \centering
%  \medskip
%     \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|}
%     \hline
%    $\textrm{Iter}_\textrm{CG}$ & $\textrm{Iter}_\textrm{DCG}$ & ${T}_{\textrm{DCG}}/{{T}_{\textrm{CG}}}$ & ${T_{\textrm{Eig}}}/{{T}_{\textrm{CG}}}$ \\ \hline
%   $129.8$ & $20.1$ &  $0.278$ & 11.105 \\ \hline
%  \end{tabular}
%       \caption{Multiple source terms test for the 3D homogeneous ball in Sec. \ref{sec:3d-ball}. $\Na$: dimension of the deflation space. $\textrm{Iter}_\textrm{(D)CG}$: average number of iterations for (D)CG. $T_{\textrm{D}CG}$: average computational time for the (D)CG. $T_{Eig}$: computational time of obtaining eigenvectors needed by the deflation.  \label{tab:3d-ball}}
% \end{table}

% \begin{figure}[htb]
% \begin{center}
% \includegraphics[width=0.40\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/ball_25_various_frequencies.eps}
% \caption{The same deflation for various frequencies for the homogeneous ball in Sec. \ref{sec:3d-ball}. Relative number of iterations and computational time of DCG compared to CG are displayed. \label{fig:3d_ball_windowed_deflation}}
% \end{center}
% \end{figure}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{3D inhomogeneous problem\label{sec:3d-ih}}
% We consider a 3D inhomoeneous problem on the computational domain $[-0.5,0.5]^3$ with the velocity field 
% \begin{equation}
%     c^2(x,y,z) = 1.0-0.9e^{-\left( \frac{x^2+y^2+z^2-0.25^2}{0.25^2}\right)^4 }
% \end{equation}
% and the frequency $\omega=20$.
% We consider the source term \begin{equation}
%     f(x,y,z) = \frac{16\omega^2}{\pi}e^{-16\omega^2( (x-x_c)^2+(y-y_c)^2+(z-z_c)^2 )},
% \end{equation}
% where $\omega$ is the frequency of the underlying problem.
% We use a uniform grid with $181$ grid points in each direction. The relative tolearnces for the stopping criteria of CG and DCG are chosen as $10^{-9}$.

% To construct a deflation matrix, we use Lanczos method to compute $80$ smallest eigenvectors of the WaveHoltz operator on the original mesh and $1$-level coarsend mesh. The tolerance of the residual for Schur vectors is $10^{-11}$. With no coarsening and $1$-level coarsening, the Lanczos algorithm converges with $63$ and $61$ iterations and results in $84$ and $93$ converged eigenvectors, respectively. When eigenvectors are computed on the coarse mesh, we interpolate it to the original mesh with  linear interpolation.



% \textbf{Different source terms.} To test the performance of the proposed DCG method for different source terms, we uniformly  pick $10$ different random center points $(x_c,y_c,z_c)$ for the source term  inside the ball $\{\sqrt{x^2+y^2+z^2}\leq0.25\}$.

% Results are summarized in Tab. \ref{tab:3d-ih}. On average, deflation matrices comprising eigenvectors and prolonged eigenvectors lead to approximately $27.5\%$ and $29.5\%$ number of iterations for convergence and $3.61$ and $2.79$ times acceleration compared to CG, respectively. 
% The average computational time to obtain eigenvectors and prolonged eigenvectors are approximately $7.070$ and $0.595$ times of the average time for one CG solve. Accounting for the time of constructing the deflation matrix, we gain computational saving when solving more than $10$ source terms for the eigenvector deflation and $2$ source terms for the prolonged eigenvector deflation.  

% \textbf{Performance with different dimensions of the deflation space.} With $(x_c,y_c,z_c)=(-0.4,0.45,0.4)$, we test the performance of DCG with different dimensions of the deflation space $\Na$. The corresponding numerical solution is presented in Fig. \ref{fig:3d_ih_solution} 
% As shown in Fig. \ref{fig:3d_ih}, DCG method converges with less number of iterations and computational time compared to CG. The number of iterations and computational time for convergence approximately scale as $O(\Na^{-0.6})$. 

% \textbf{Same deflation for a narrow frequency band.} We use the converged $84$ eigenvectors and $93$ prolonged eigenvectors for $\omega=20$ as the deflation matrix for frequencies in the band $[19.4,20.6]$. As displayed in Tab. \ref{fig:3d_ih}, both eigenvector and prolonged eigenvector deflation is faster than CG. For all tested frequencies except for $\omega=20.6$, using the fine level eigenvectors as the deflation matrix achieves more acceleration than using prolonged eigenvectors. %when the frequency $\omega$ is close to $20$, this deflation matrix results in less number of iterations for convergence and smaller computational time.

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{table}[htbp]
%   \centering
%  \medskip
%     \begin{tabular}
%     {|l|c|c|c|c|c|c|c|c|c|c|c|}
%     \hline
% Eigenvector computation & $\Na$ & $\textrm{Iter}_\textrm{CG}$ & $\textrm{Iter}_\textrm{DCG}$ &  $\textrm{Iter}_\textrm{Eig}$ & ${T}_{\textrm{DCG}}/{{T}_{\textrm{CG}}}$ & ${T_{\textrm{Eig}}}/{{T}_{\textrm{CG}}}$ \\ \hline
%  No coarsening & $84$ &  $511.1$ & $140.6$ & $63$ & $0.277$ & $7.070$ \\ \hline
%  $1$-level coarsening & $93$ & $511.1$ & $151$ & $61$ & $0.358$ & $0.696$ \\ \hline
%  \end{tabular}
%       \caption{Multiple source terms test for the 3D inhomogeneous problem in Sec. \ref{sec:3d-ih}. $\textrm{Iter}_\textrm{(D)CG}$: average number of iterations for (D)CG. $T_{\textrm{D}CG}$: average computational time for the (D)CG. $T_{Eig}$: computational time of obtaining eigenvectors needed by the deflation.  \label{tab:3d-ih}}
% \end{table}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{table}[htbp]
%   \centering
%  \medskip
%     \begin{tabular}
%     {|l|c|c|c|c|c|c|c|c|c|c|c|}
%     \hline
%  $\omega$ & $19.4$ & $19.6$ & $19.8$ & $20.0$ & $20.2$ & $20.4$ & $20.6$\\ \hline
%  {$\textrm{Iter}_\textrm{DCG}/\textrm{Iter}_\textrm{CG}$, no coarsening} &  $0.458$&    $0.303$&    $0.289$&    $0.301$&    $0.335$&    $0.485$& $0.917$ \\ \hline
%  {$\textrm{Iter}_\textrm{DCG}/\textrm{Iter}_\textrm{CG}$}, $1$-level coarsening &  $0.861$&    $0.473$ &    $0.350$&    $0.321$ &    $0.248$ &    $0.301$    & $0.335$ \\ \hline
% {${T}_{\textrm{DCG}}/{{T}_{\textrm{CG}}}$, no coarsening} &  $0.459$&    $0.300$   & $0.271$   & $0.301$    &$0.329$    & $0.488$    & $0.952$ \\ \hline
%  {${T}_{\textrm{DCG}}/{{T}_{\textrm{CG}}}$, 1-level coarsening} &    $0.985$&    $0.607$&    $0.401$&    $0.423$&    $0.328$&    $0.377$&    $0.349$\\\hline 
%  \end{tabular}
%       \caption{Same deflation for frequencieis in a narrow band for the 3D inhomogeneous problem in Sec. \ref{sec:3d-ih}. $\textrm{Iter}_\textrm{(D)CG}$: average number of iterations for (D)CG. $T_{\textrm{(D)CG}}$: average computational time for the (D)CG.  \label{tab:3d-ih-window}}
% \end{table}

% %%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{figure}[htb]
% \begin{center}
% \includegraphics[width=0.32\textwidth,trim={0.3cm 0.3cm 0.3cm 0.4cm},clip]{figures/sliced_solution_x.eps}
% \includegraphics[width=0.32\textwidth,trim={0.3cm 0.05cm 0.3cm 0.4cm},clip]{figures/sliced_solution_y.eps}
% \includegraphics[width=0.32\textwidth,trim={0.3cm 0.05cm 0.3cm 0.4cm},clip]{figures/sliced_solution_z.eps}
% \caption{Slices of the numerical solution for 3D inhomogeneous problem in Sec. \ref{sec:3d-ih} with the source term corresponding to $(x_c,y_c,z_c)=(-0.4,0.45,0.4)$.  \label{fig:3d_ih_solution}}
% \end{center}
% \end{figure}
% %%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%
%  \begin{figure}[htb]
% \begin{center}
% \includegraphics[width=0.45\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/iter_3d_ih.eps}
% \hspace{0.1cm}
% \includegraphics[width=0.45\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/time_3d_ih.eps}
% %\includegraphics[width=0.32\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/cube_20_various_frequencies.eps}
% \caption{Results for 3D inhomogeneous problem in Sec. \ref{sec:3d-ih} with the source term corresponding to $(x_c,y_c,z_c)=(-0.4,0.45,0.4)$. Left: relative and absolute number of iterations for convergence for $\omega=20$. Right: relative computational time for $\omega=20$. \label{fig:3d_ih}}
% \end{center}
% \end{figure}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \section{Conclusions \label{sec:conclusion}}
% In this paper, we propose a deflated WaveHoltz method to solve Helmholtz problem with multiple right hand sides and energy conserving boundary conditions which yield trapped wave structures. 

% We formally show that using eigenvectors as the deflation matrix, the proposed deflated WaveHoltz method converges with a number of iterations approximately proportional to the  reciprocal  of number of eigenvectors, leading to a sub-linear saving of computational time. 

% Our numerical experiments demonstrate the effectiveness of the proposed method. The WaveHoltz method is effectively accelerated by leveraging a deflation matrix consisting of eigenvectors or approximated eigenvectors prolonged from a coarse mesh, which effectively resolves the wave structure. Additionally, we also show that the same deflation matrix can be applied for problems with various frequencies in a narrow band. 

% In the future, we plan to investigate using a deflation matrix based on reduced order models  for parametric problems \cite{cortes2018pod,panagiotopoulos2023accelerated}.

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \appendix
% \section{$A$-orthogonality with exact eigenvector deflation\label{sec:A-orthogonality}}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Here, we show that, when $W$ comprises exact eigenvectors of $\whiA_h$, there is no need to  impose $A$-orthogonality in DCG, as $A$-orthogonality is auntomatically guaranteed.

% Expand $\rb_0$ as a linear combintation of eigenvectors $\rb_0=\sum_{j=1}^N r_j\wb_j$.
% Since $W^T\rb_0=0$ we have $r_j=0$ with $j=1,\dots,\Na$. As a result 
% \begin{equation*}
% W^TA \rb_0 = \sum_{j={\Na+1}}^N W^T \lambda_j r_j\wb_j =0.
% \end{equation*}
% This guarantees ${\bm \mu_0}=0$ and $W^T \pb_0=0$. With mathematical induction one can show that ${\bm \mu_k}=0$ and $W^T\pb_{k}=W^T\rb_{k}=0$ for any $k$.



% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % \bibliographystyle{plain}
% % \bibliography{ref}





% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \clearpage
% %%%%%%%%%%%%%%%%%
% %\begin{comment}
% %%%%%%%%%%%%%%%%%
% \subsubsection{Accuracy needed for $(W^TAW)^{-1}$}
% We need to apply $(W^TAW)^{-1}$ when we construct $\xb_0$ or impose $A$-orthogonality with respect to the deflation space to the search directions $\pb_k$. Here we will discuss how we implement $(W^TAW)^{-1}$ operation in practice.

% When $W$ is formed eigenvectors of $A$, one can prove that $W^TAW$ is a diagonal matrix whose diagonal elements are the corresponding eigenvalues, and it is simple and computationally cheap to invert such a $W^TAW$.
% When the size of $W^TAW$, $\Na$ is much smaller than $N$, we can directly factorize it to compute $W^TAW)^{-1}$. 
% For a larger $W^TAW$, we can use a Krylov subspace iterative solver to invert it. The required accuracy for such solvers is numerically investigated in \cite{nabben2006comparison}, analyzed and further relaxed in \cite{kahl2017deflated}. The analysis in \cite{kahl2017deflated} suggests that given the sopping criterion for the DCG algorithm
% $||\rb_k||\leq \varepsilon \bbb$, 
% the required accuracy for the inner loop solving the linear system determined by $W^TAW$ is
% \begin{equation}
%     ||\rb_k^{\textrm{inner}}||\leq c\frac{\varepsilon}{||\rb_k||}||\bbb^{\textrm{inner}}|||,\quad 0\leq c<1.
% \end{equation}
% As the iteration continues, the residual in the DCG algorithm $||\rb_k||$ becomes smaller and the required accuracy for the inner loop solving $W^TAW$ can be adaptively enlarged.



% \subsection{Eigenvalues for different geometries} (\textcolor{blue}: we should remove this Section)
% The geometry of $\Omega$ affects the distribution and values of the eigenvalues of the $S$ operator. Here, we present the eigenvalues for a few different geometries.




% \subsubsection{The Unit Square in $d$-dimensions}
% The eigenvalues and eigenvectors of the three point discretization $[-1, 2, -1]$ of the Laplacian on $[0,1]$ with a grid size $h=1/(n+1)$ with Dirichlet boundary conditions are
% \begin{eqnarray}
%     \lambda_k &= 2 \left(1-\cos \left(\frac{k \pi}{n+1}\right) \right),\ \ k = 1\ldots,n \\
%     w_k[i] &= \sqrt{\frac{2}{n+1}} \sin\left(i\frac{k\pi}{n+1}\right),\ \  i = 1\ldots,n,\, k = 1\ldots,n. 
% \end{eqnarray}


% \begin{figure}[htb]
% \begin{center}
% \includegraphics[width=0.46\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/beta_eig_contour_2d}
% \includegraphics[width=0.5\textwidth]{figures/beta_eig_contour_3d}
% \caption{Number of eigenvectors needed to reach $\beta_\omega(\lambda)<\beta$. Left: 2D. Right: 3D. \label{fig:beta_omega_contour}}
% \end{center}
% \end{figure}


% \begin{figure}[htb]
% \begin{center}
% \includegraphics[width=0.5\textwidth]{figures/omega_ap_contour_2d}
% \caption{Number of eigenvectors needed to reach $\beta_\omega(\lambda)<0.95$. \label{fig:beta_omega_contour}}
% \end{center}
% \end{figure}

% \subsection{Multilevel DCG}
% Constructing eigenvector deflation matrix may be costly especially when a refined grid is used. To mitigate this computational cost, we can design a multilevel DCG method which first converts $\whiA\xb=\bbb$ to a problem on a coarse grid  and then performs the eigenvector deflation on the coarse grid where the eigenvectors can be more efficiently computed.  

% Multilevel DCG method can be designed following \cite{kruzik2017wavelet,kruvzik2018implementace}. Given a hierarchy of deflation matrix $W_l\in\mathbb{R}^{K_{l-1}\times K_l}$ with $l=1,\dots,L$ and $K_0=N$. Then the deflation matrix and the corresponding Galerkin matrix for the multilevel method are
% \begin{equation*}
% W = W_1W_2\dots W_L \quad\text{and}\quad W_L^T\dots W_2^T W_1^TAW_1W_2\dots W_L.
% \end{equation*}
% When solving $A\xb=\bbb$ we apply the DCG method with deflation matrix $W_1$, namely DCG($A,\bbb,W_1$). Inside DCG($A,\bbb,W_1$) we invert $W_1^TAW_1$ with a second DCG solver DCG($W_1^TAW_1,\cdot,W_2)$. We nest the DCG solve until we reach the last level $L$ and invert $W_L^TAW_L$ with a direct or Krylov solver.

% Particularly we will apply the following prolongation based deflation (PED) when inverting the WaveHoltz linear system. For $l=1,\dots,L-1$, we choose $W_l$ as a prolongation from a coarse grid with $h_l=2^lh$ to a fine grid with $h_{l-1}=2^{l-1}h$ and choose $W_L$ as eigenvectors of the Galerkin matrix $W_{L-1}^T\dots W_1^T A W_1\dots W_{L-1}^T$ on the most coarse level. The eigenvectors will be only computed on the most coarse grid and there is no need to impose the $A$-orthogonality in the DCG solve for $W_{L-1}^T\dots W_1^T A W_1\dots W_{L-1}^T$. 


% \begin{rem}
% The multilevel DCG described above may be combined with the aforementioned idea of approximating eigenvectors based on information provided by successive solves of multiple right hand side \cite{saad2000deflated,stathopoulos2010computing}, and this combination is left for future investigation.    
% \end{rem}

% \subsection{Prolongation based eigenvector deflation for the WaveHoltz matrix $\whiA_h$}
% Here we define a prolongation eigenvector deflation based a the linear prolongation, and we will find the eigenvectors for the most coarse Galerkin matrix $W_L^TW_{L-1}^T\dots W_1^T\whiA_h W_1W_2\dots W_L$. 

% For simplicity we consider $1D$ Helmholtz problem $c(x)\equiv1$.
% We first introduce the following grid. Assume $N$ be an even integer. Let $\Omega_h$ be a fine grid: $0=x_0\leq x_1 = h\leq \ldots\leq x_N=1$. Let $\Omega_{2h}$ be the coarse grid:
% $0=x^c_0\leq x^c_1 = 2h\leq \ldots\leq x^c_{N/2}=1$. 
% The fine grid  $\Omega_h$ and coarse grid $\Omega_{2h}$ with $N=8$ are illustrated in Fig. \ref{fig:fine-coarse-grid}. 
%  Let $L_h$ denote the matrix corresponding to the $[-1,2,-1]$ central difference discretization  of $\Delta$ with the mesh size $h=\frac{1}{N}$.

% We define the linear prolongation operator $I_{2h}^h$ which maps a grid function $\vb^{2h}$ on the coarse grid $\Omega_{2h}$ to a grid function  on the fine grid $\Omega_h$:
% \begin{subequations}
%     \begin{align}
%     &I_{2h}^h\vb^{2h}_{2j} = \vb^{2h}_j,\;0\leq j\leq\frac{N}{2},\\
%     &I_{2h}^h\vb^{2h}_{2j+1} =\half\left( \vb^{2h}_{j}+\vb^{2h}_{j+1}\right),\;0\leq j\leq\frac{N}{2}-1.
%     \end{align}
% \end{subequations}
% The full weighting restriction operator mapping a grid function $\vb^h$ on $\Omega_h$ to a grid function $\Omega_{2h}$ is defined as:
% \begin{equation}
% (I_{h}^{2h}\vb^h)_{j}=\frac{1}{4}(\vb^h_{j-1}+2\vb^h_{j}+\vb^h_{j+1}), \; 1\leq j\leq \frac{N}{2}-1.
% \end{equation}
% The full weighting restriction $I_{h}^{2h}$ and the linear prolongation $I_{2h}^h$ satisfy the variational relation: 
% \begin{equation}
%     I_{h}^{2h} = \frac{1}{2} (I_{2h}^h)^T.\label{eq:variational_property}
% \end{equation}
% Since in the DCG algorithm $W_l^T$ only appears in $(W^TAW)^{-1}W^T$ terms one can actually replace $W_l^T$ with the restriction operator $I_{2^{l-1}h}^{2^lh}$ when implementing the algorithm.

% In the $L$ level prolongation based eigenvector deflation we choose deflation matrices as
% \begin{equation}
% W_l = \begin{cases}
%        I_{2^lh}^{2^{l-1}h}, \quad &1\leq l\leq L-1,\\ 
%        \textrm{first $\Na$ eigenvectors of }W_{L-1}^T\dots W_1^T A W_1\dots W_{L-1}, \quad &l= L. 
%        \end{cases}
% \end{equation}
% With $\whiA_h$ equal to the WaveHoltz operator $I-S_h$, we will show that the eigenvectors for $W_{L-1}^T\dots W_1^T \whiA_h W_1\dots W_{L-1}$ are the eigenvectors of the discrete Laplacian operator on the most coarse grid, $L_{2^Lh}$. 

% \subsubsection{Eigenvectors of $W_{L-1}^T\dots W_1^T \whiA_h W_1\dots W_{L-1}$}
% We start with proving eigenvectors of $W_1^T\whiA_h W_1$ are the eigenvectors of the discrete Laplacian operator $L_{2h}$. With the variational property \eqref{eq:variational_property}, it is enough to find eigenvectors for $I^{2h}_{h}\whiA I_{2h}^h$. 

% The proof is based on the properties of the full weighting restriction and the linear prolongation \cite{briggs2000multigrid}. Let $\wb^h_k$ be an eigenvector of the discrete Laplacian operator $L_{h}$.
% \begin{lem}\label{lem:restriction_and_prolong_effect}
% Let $k'=N-k$. For $1\leq k < \frac{N}{2}$, following relations are satisfied:
% \begin{subequations}
% \label{eq:restri_prolong_equality}
% \begin{align}
%     I_{2h}^{h} \wb^{2h}_k &= c_k^{2h}\wb_k^h-s_k^{2h}\wb_{k'}^h,\label{eq:full_weight} \\
%     I_{h}^{2h}\wb^h_k &= c_k^{2h}\wb_k^{2h},\label{eq:prolong_k}\\
%     I_{h}^{2h}\wb^h_{k'} &= - s_k^{2h}\wb_k^{2h},\label{eq:prolong_kp}
% \end{align}
% \end{subequations}
% where $c_k^{2h}=\cos^2(\frac{k\pi}{2N})$ and $s_k^{2h}=\sin^2(\frac{k\pi}{2N})$.
% \end{lem}

% \begin{thm}
% Let $1\leq k< \frac{N}{2}$  and $L_{2h}\wb^{2h}_{k}=\sigma_k^2\wb^{2h}_{k}$. Then $\wb^{2h}_k$ is also an eigenvector of $I_{h}^{2h} \whiA_h I_{2h}^h$ with $\whiA_h$ being the WaveHoltz operator on $\Omega_h$ and 
% \begin{equation}
% I_{h}^{2h} \whiA_h I_{2h}^h\wb^{2h}_k =\left(\; 
% (c_k^{2h})^2(1-\beta_h(\sigma_k))+(s_k^{2h})^2(1-\beta_h(\sigma_{k'}))\;\right)\wb_k^{2h}.\label{eq:projected_waveholtz_eig}
% \end{equation}
% with $k'=N-k$.
% \end{thm}
% \begin{proof}
% Recall that eigenvectors of $L_h$ is also an eigenvector of $\whiA_h$ and satisfies \eqref{eq:waveholtz_eigvectors}. 
% Utilizing equation \eqref{eq:full_weight} and \eqref{eq:waveholtz_eigvectors} we get
% \begin{align}
% \whiA_h I_{2h}^h\wb^{2h}_k &= \whiA_hc_k^{2h}\wb_k^h-\whiA_hs_k^{2h}\wb_{k'}^h\notag\\
% &= (\;1-\beta(\sigma_k^h)\;)c_k^{2h}\wb_k^h-(\;1-\beta(\sigma_{k'}^h)\;)s_k^{2h}\wb_{k'}^h.
% \end{align}
% Then using \eqref{eq:prolong_k} and \eqref{eq:prolong_kp} we obtain
% \begin{align}
% I_{h}^{2h}\whiA_h I_{2h}^h\wb_{2h}^k &= (\;1-\beta(\sigma_k^h)\;)c_k^{2h}I_{h}^{2h}\wb_k^h-(\;1-\beta(\sigma_{k'}^h)\;)s_k^{2h}I_{h}^{2h}\wb_{k'}^h\notag\\
% &=  (\;1-\beta(\sigma_k^h)\;)(c_k^{2h})^2\wb_k^{2h}+
% (\;1-\beta(\sigma_{k'}^h)\;)(s_k^{2h})^2\wb_k^{2h}\notag\\
% &=\left(\; 
% (c_k^{2h})^2(1-\beta_h(\sigma_k))+(s_k^{2h})^2(1-\beta_h(\sigma_{k'}))\;\right)\wb_{k}^{2h}.
% \end{align}
% \end{proof}

% Now we move to the multilevel case. The computation is similar but more involved.
% \begin{thm}\label{thm:multilevel_eig}
% Let $1\leq k<\frac{N}{2^{l}}$. Then the $k$-th eigenvector of the discrete Laplacian operator $L_{2^{l}h}$, $\wb_{k}^{2^lh}$, is an eigenvector of 
% $I_{2^{l-1}h}^{2^lh}\dots I_{h}^{2h} \whiA_h I_{2h}^h\dots I_{2^lh}^{2^{l-1}h}$.
% \end{thm}
% \begin{proof}
% Repeatedly using \eqref{eq:restri_prolong_equality}, we get
% \begin{align*}
%    I_{2^{l-1}h}^{2^lh}\dots I_{h}^{2h} \whiA_h I_{2h}^h\dots I_{2^lh}^{2^{l-1}h}w_{k}^{2^lh} &=
%    I_{2^{l-1}h}^{2^lh}\dots I_{h}^{2h} \whiA_h I_{2h}^h\dots I_{2^{l-1}h}^{2^{l-2}h}
%    \left(C_k^{(l)}\wb_{k}^{2^{l-1}h}+C_{\frac{N}{2^{l-1}}-k}^{(l)}\wb^{2^{l-1}h}_{\frac{N}{2^{l-1}}-k}\right)\notag\\
%    &=I_{2^{l-1}h}^{2^lh}\dots I_{h}^{2h} \whiA_h
%   \left( \sum_{j=1}^{2^{l-1}} C_{\frac{(j-1)N}{2^{l-1}}+k}^{(1)}\wb_{\frac{(j-1)N}{2^{l-1}}+k}^h
%    +\sum_{j=1}^{2^{l-1}} C_{\frac{jN}{2^{l-1}}-k}^{(1)}\wb_{\frac{jN}{2^{l-1}}-k}^h\right)\notag\\
%    &=I_{2^{l-1}h}^{2^lh}\dots I_{h}^{2h}\left( \sum_{j=1}^{2^{l-1}} \widetilde{C}_{\frac{(j-1)N}{2^{l-1}}+k}^{(1)}\wb_{\frac{(j-1)N}{2^{l-1}}+k}^h
%    +\sum_{j=1}^{2^{l-1}} \widetilde{C}_{\frac{jN}{2^{l-1}}-k}^{(1)}\wb_{\frac{jN}{2^{l-1}}-k}^h\right)\notag\\
%    &=I_{2^{l-1}h}^{2^lh}\dots I_{2h}^{4h}\left( \sum_{j=1}^{2^{l-2}} \hat{C}_{\frac{(j-1)N}{2^{l-1}}+k}^{(2)}\wb_{\frac{(j-1)N}{2^{l-1}}+k}^{2h}
%    +\sum_{j=1}^{2^{l-2}} \hat{C}_{\frac{jN}{2^{l-1}}-k}^{(2)}\wb_{\frac{jN}{2^{l-1}}-k}^{2h}\right)\notag\\
%    &= \hat{C}^{(l)}\wb_{k}^{2^lh},
% \end{align*}
% where all the $\hat{C}$, $\widetilde{C}$ and $C$ are generic constants. 
% \end{proof}

% A direct result of the variational property \eqref{eq:variational_property} and Theorem \ref{thm:multilevel_eig} is that eigenvectors of $W_{L-1}^T\dots W_1^T A_h W_1\dots W_{L-1}$ with $W_l=I_{2^{l+1}h}^{2^lh}$ are the eigenvectors of the discrete Laplacian operator $L_{2^{L}h}$. 

% \subsubsection{Loss of Galerkin condition}
% We also want to point out that the WaveHoltz operator $\whiA_h$ does not satisfy the Galerkin condition, in other words 
% \begin{equation*}
%     \whiA_{2h}\neq I_{h}^{2h}\whiA_hI_{2h}^h.
% \end{equation*}
% With the time stepping in \eqref{eq:modified_time_stepping} and the quadrature in \eqref{eq:quadrature} one can show that $\whiA_{h}\wb = P_{N_t}(L_h)\wb$ where 
% $P_{N_t}(x)=\xi_0+\xi_1x+\dots+\xi_{N_t}x^{N_t}$ is a polynomial with $\xi_{N_t}\neq 0$.
% If CFL conditions for the coarse grid $\Omega_{2h}$ and the fine grid $\Omega_h$ are the same, the total number of time steps will be different and $A_{2h}$ will be a polynomial of $L_{2h}$ but with adifferent degree. We can also use the same total number of time steps on the coarse level to get a modified coarse level WaveHoltz operator $\widetilde{\whiA}_{2h}=P_{N_t}(L_2h)$. Based on the Galerkin condition $L_{2h}=I_{h}^{2h}L_hI_{2h}^h$ we have
% \begin{equation}
% (L_{2h})^{n_t} = (I_{h}^{2h}L_hI_{2h}^h)^{n_t}= I_{h}^{2h}L_h (I_{2h}^hI_{h}^{2h})L_h\dots L_h(I_{2h}^hI_{h}^{2h})L_h I_{h}^{2h} \neq I_h^{2h} (L_h)^{n_t} I_{2h}^h,\quad \textrm{if} n_t\geq 1.
% \end{equation}
%  As a result $\widetilde{\whiA}_{2h}\neq I_{h}^{2h}\whiA_hI_{2h}^h$.
% Without the Galerkin condition 
% $\left(I_{h}^{2h}\whiA_h I_{2h}^h\right)^{-1}$ can not be inverted by directly applying the WaveHoltz solver on the coarse grid.



% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{figure}
% \begin{center}
% \setlength{\unitlength}{0.8cm}
% \begin{picture}(8,3) 
% % Grid
% \thicklines
% \put(0,1){\line(1,0){8}}
% \put(0,2){\line(1,0){8}}
% % intervals on refined mesh
% \put(0,2){\line(0,1){0.25}}
% \put(1,2){\line(0,1){0.25}}
% \put(2,2){\line(0,1){0.25}}
% \put(3,2){\line(0,1){0.25}}
% \put(4,2){\line(0,1){0.25}}
% \put(5,2){\line(0,1){0.25}}
% \put(6,2){\line(0,1){0.25}}
% \put(7,2){\line(0,1){0.25}}
% \put(8,2){\line(0,1){0.25}}
% % intervalus on coarse mesh
% \put(0,1){\line(0,1){0.25}}
% \put(2,1){\line(0,1){0.25}}
% \put(4,1){\line(0,1){0.25}}
% \put(6,1){\line(0,1){0.25}}
% \put(8,1){\line(0,1){0.25}}
% % index for grid points on refined mesh
% \put(-0.1,2.3){$0$}
% \put(0.9,2.3){$1$} 
% \put(1.9,2.3){$2$} 
% \put(2.9,2.3){$3$} 
% \put(3.9,2.3){$4$} 
% \put(4.9,2.3){$5$} 
% \put(5.9,2.3){$6$} 
% \put(6.9,2.3){$7$} 
% \put(7.9,2.3){$8$} 
% % index for grid points on coarse mesh
% \put(-0.1,1.3){$0$}
% \put(1.9,1.3){$1$} 
% \put(3.9,1.3){$2$} 
% \put(5.9,1.3){$3$} 
% \put(7.9,1.3){$4$} 
% % text
% \put(-1,2){$\Omega_h$:}
% \put(-1,1){$\Omega_{2h}$:}
% \end{picture}
% \end{center}
% \caption{The fine grid $\omega_h$ and the coarse grid $\omega_{2h}$ with $N=8$.\label{fig:fine-coarse-grid}}
% \end{figure}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \section{Numerical verification}
% To verify the theory in Sec. \ref{sec:iter_vs_eig}, we
% consider two tests.

% In the first test we consider the problem
% \begin{align}
% \omega^2 u +\Delta u = \omega^2\delta(\bx-\bx_c), \quad\bx\in[0,1]^d,\bx_c=(0.5,\dots,0.5)^T, d=2,3.
% \end{align}
% We consider $\omega=40,80$ in 2D with and $\omega=20,40$ in 3D, In each direction we use $N=2^{\lceil\log_2(\lceil 4\omega\rceil)\rceil}-1$ in 2D and $N=2^{\lceil\log_2(\lceil 2\omega\rceil)\rceil}-1$ grid points in 3D. In the deflation step we not only use eigenvectors from the original grid but also use the eigenvectors interpolated from one level and two level coarsen grids.

% In Fig. \ref{fig:iter_vs_eig} we plot the number of iterations of the DCG method to reach the relative tolerance $10^{-7}$ as a function of the number of eigenvectors in the deflation space.
% According to our theory if the number of eigenvalues $\Na$ scales as $O(\omega^s)$, the number of iterations for the convergence $N_{\textrm{iter}}$ scales as $O(\omega^{d-s})$. Under the $\log$-scale we have
% \begin{equation}
%     \log_{10}(\Na)\propto\log_{10}(\omega) s \quad\text{and}\quad
%     \log_{10}(N_{\textrm{iter}})\propto \log_{10}(\omega)(d-s)=\log_{10}(\omega)d - \log_{10}(\Na),
% \end{equation}
% so $log_{10}(\Na)$-$\log_{10}(N_{\textrm{iter}})$ picture is a straight line with slope $-1$. 
% In Fig. \ref{fig:iter_vs_deflation_dim} $N_{\textrm{iter}}$-$\Na$ can indeed be qualitatively captured by straight lines with slope $-1$ under the $\log$-scale with both exact eigenvectors and eigenvectors interpolated from one or two level coarsened grid. 

% In the second test 

 

% \begin{figure}[htb]
% \begin{center}
% \includegraphics[width=0.46\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/2d_eig_vs_iter_eig_orig_40.eps}
% \includegraphics[width=0.46\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/2d_eig_vs_iter_eig_orig_80.eps}
% \includegraphics[width=0.46\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/3d_eig_vs_iter_eig_orig_20.eps}
% \includegraphics[width=0.46\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/3d_eig_vs_iter_eig_orig_40.eps}
% \caption{Number of iterations as a function of number of eigenvectors in the deflation space to reach relative error tolerance $10^{-7}$. \label{fig:iter_vs_eig}}
% \end{center}
% \end{figure}







% \subsection{Complexity}
% In this section we express the complexity with respect to estimated floating point operations and storage requirements. Throughout we assume that the discretization is done with a fixed number of points per wavelength. We give the complexity estimates both in terms of the frequency $\omega$ and the system size $N$. As will be seen some of the estimates are dimension dependent.   

% \begin{table}[htbp]
%   \centering
%  \medskip
%     \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|}
%     \hline
%  	Apply $A$ & $W^TA r$ & $(W^TAW)^{-1}$ & $O(N)$ operations & Total cost & Memory \\ \hline
%  	$N\times N_t$ & $k_\textrm{eig}\times N$ & $k_\textrm{eig}^2$ \textrm{or} $k_\textrm{eig}$ & $N$ & $k_\textrm{eig}\times N$ &
%  	 $k_\textrm{eig}\times N$ \\ \hline
%  	$\omega^d\times N_t$ & $\omega^{2d}$ & $\omega^{2d}$ or $\omega^d$ & $\omega^d$ &
%  	$\omega^{2d}$ & $\omega^{2d}$\\ 
%  	\hline
%  	 $N\times N_t$ & $N^2$ & $N^{2}$ or $N$ & $N$ & $N^2$ & $N^2$\\
%  	\hline
%  \end{tabular}
%       \caption{}
% \end{table}

% \begin{table}[htbp]
%   \centering
%  \medskip
%     \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|}
%     \hline
%  	Apply $A$ & $W^TA r$ & $(W^TAW)^{-1}$ & $O(N)$ operations & Total cost & Memory \\ \hline
%  	$N\times N_t$ & $k_\textrm{eig}\times N$ & $k_\textrm{eig}^2$ \textrm{or} $k_\textrm{eig}$ & $N$ & $k_\textrm{eig}\times N$ &
%  	 $k_\textrm{eig}\times N$ \\ \hline
%  	$\omega^d\times N_t$ & $\omega^{d+s}$ & $\omega^{2s}$ or $\omega^{s}$ & $\omega^d$ &
%  	$N_\textrm{iter}\omega^{d+s}$ & $\omega^{d+s}$\\ 
%  	\hline
%  	 $N\times N_t$ & $N^{1+s/d}$ & $N^{2s/d}$ or $N^{s/d}$ & $N$ & $N_\textrm{iter}\times N^{1+s/d}$ & $N^{1+s/d}$\\
%  	\hline\hline
%  	 	 $N\times N_t$ & $N$ & $1$  & $N$ & $N^2$ & $N$\\
%  	\hline
%  	 	 	 $N\times N_t$ & $N^{1+(d-1)/d}$ & $N^{2(d-1)/d}$ or $N^{(d-1)/d}$ & $N$ & $ N^2$ & $N^{1+(d-1)/d}$\\
%  	 	 	 \hline
%  \end{tabular}
%       \caption{}
% \end{table}


% \begin{table}[htbp]
% \scriptsize
% \begin{center}
% \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|}
%     \hline
%  	& Apply $A$ & $W^TA r$ & $(W^TAW)^{-1}$ & Form $AW$ & Form $W$ & Total cost & Memory    \\ 
%  	 	\hline
%  	DCG & $NN_t$ & $N^{2}$ & $N^2$ or $N$ & $N_tN^2$ & $N_\textrm{arpack}$ & $N_\textrm{RHS}( N_\textrm{iter}N+ N^{2})+N_t N^2+N_\textrm{arpack}$ & $N^2$
%  	 \\ \hline
%  	DCG & $N N_t$ & $N^{1+s/d}$ & $N^{2s/d}$ or $N^{s/d}$ & $N_tN^{1+s/d}$ & $N_\textrm{arpack}$ & $N_\textrm{RHS}( N^{1-s/d}N+ N^{1+s/d}) +N_t N^{1+s/d}+N_\textrm{arpack}$& $N^{1+s/d}$
%  	 \\ \hline
%  	 DCG & $\omega^d N_t$ & $\omega^{d+s}$ & $\omega^{2s}$ or $\omega^s$ & $N_t\omega^{d+s}$ & $N_\textrm{arpack}$ & $N_\textrm{RHS}( \omega^{2d-s}+ \omega^{d+s}) +N_t \omega^{d+s}+N_\textrm{arpack}$& $\omega^{d+s}$
%  	 \\ \hline
%    CG & $N N_t$ & NA & NA & NA & NA & $N_\textrm{RHS}N^2$ & $N$ \\ \hline
%    CG & $N N_t$ & NA & NA & NA & NA & $N_\textrm{RHS}\omega^{2d}$ & $N$ \\ \hline
%  \end{tabular}
%       \caption{}
%  \end{center}
% \end{table}
% \normalsize


% \begin{figure}[htb]
% \begin{center}
% \includegraphics[width=0.48\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/neigs_vs_cputime_40_2d}
% \includegraphics[width=0.48\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/neigs_vs_cputime_30_3d}
% \includegraphics[width=0.48\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/neigs_vs_iter_40_2d}
% \includegraphics[width=0.48\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/neigs_vs_iter_30_3d}
% \caption{CPU time and number of iterations for the KrylovKit (Krylov-Schur algorithm) to compute eigenvectors. Left: 2D. Right: 3D. \label{fig:eig_efficiency}}
% \end{center}
% \end{figure}


% \subsection{Rate of convergence with and without deflation}


% \begin{figure}[htb]
% \begin{center}
% \includegraphics[width=0.32\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/2d_iter_vs_defdim}
% \includegraphics[width=0.32\textwidth]{figures/3d_iter_vs_defdim}
% \includegraphics[width=0.32\textwidth]{figures/3d_iter_vs_defdim_2}
% \caption{Number of iterations for convergence for different dimensions of the deflation space. \label{fig:iter_vs_deflation_dim}}
% \end{center}
% \end{figure}


% \subsection{Compression of matrices}
% \subsubsection{Compression of $W$}
% \subsubsection{Compression of $W^T \whiA$}

% \clearpage


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Experiments in One Dimension}
% The eigenvalues and eigenvectors of the three point discretization $[-1, 2, -1]$ of the Laplacian on the unit square with a grid size $h=1/(n+1)$ with Dirichlet boundary conditions are
% \begin{eqnarray}
%     \lambda_k &= 2 \left(1-\cos \left(\frac{k \pi}{n+1}\right) \right),\ \ k = 1\ldots,n \\
%     v_k[i] &= \sqrt{\frac{2}{n+1}} \sin\left(i\frac{k\pi}{n+1}\right),\ \  i = 1\ldots,n,\, k = 1\ldots,n. 
% \end{eqnarray}

% To test how well the deflation works with eigenvectors computed on a coarse grid and then interpolated to a fine grid we consider the grids with $n=2^l-1$ interior points. In this experiment we only consider the case when the course and the fine level are one level apart. 

% In Fig. \ref{fig:conv_linear} and Fig. \ref{fig:conv_spline} we display the relative reduction in the Euclidean norm of each of the eigenvectors after one WaveHoltz iteration using $\omega = 30$. We also display the the square root of the WaveHoltz filter function 
% \begin{equation}
% \beta(\lambda;\omega) = \frac{\omega (3 \lambda^2+\omega^2) \sin \left(2 \pi \frac{\lambda}{\omega} \right)}{ (4 \pi (\lambda^3 - \lambda \omega^2)},
% \end{equation}
% and the relative reduction in the Euclidean norm of the error in the interpolated eigenvector with the part along the coarse eigenvector removed (deflated). To be precise, let $\mathcal{I}$ be the interpolation (prolongation) operator and $v^{\rm f}_k$ and $ v^{\rm c}_k$ be the $k$th eigenvectors on the fine and coarse grids. Then for each $\lambda_k$ on the coarse grid we display $ \| \Pi \delta_{\rm D} \| / \| \delta_{\rm D} \|$ where
% \[
% \delta_{\rm D} = v^{\rm f}_k -  \mathcal{I} v^{\rm c}_k. 
% \]  

% The two different figures display results using linear interpolation and spline interpolation.

% As can be seen in both cases the WaveHoltz iteration is highly efficient in reducing the size of the error contribution orthogonal to the deflation subspace (in this case a single vector...).

% It is also clear that the reduction is improved with increasing resolution but also on coarse meshes it is fairly good.

% \begin{figure}[htb]
% \begin{center}
% \includegraphics[width=1.0\textwidth,trim={8.0cm 2.5cm 6.0cm 2.3cm},clip]{figures/conv_in_norm1D_linear}
% \caption{Relative reduction in norm using deflation with interpolated eigenvectors. This figure is for linear interpolation. \label{fig:conv_linear}}
% \end{center}
%  \end{figure}

% \begin{figure}[htb]
% \begin{center}
% \includegraphics[width=1.0\textwidth,trim={8.0cm 2.5cm 6.0cm 2.3cm},clip]{figures/conv_in_norm1D_spline}
% \caption{Relative reduction in norm using deflation with interpolated eigenvectors. This figure is for spline interpolation. \label{fig:conv_spline}}
% \end{center}
%  \end{figure}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% \clearpage
% \subsection{Experiments in Two Dimensions}
% \subsubsection{The unit square}
% % This is computations using the file test2D_square.m
% The eigenvalues and eigenvectors of the five point discretization of the Laplacian on the unit square with a grid size $h=1/(n+1)$ with Dirichlet boundary conditions are found by tensor products from the one dimensional case. 
% %\begin{eqnarray}
% %    \lambda_k &= 2 \left(1-\cos \left(\frac{k \pi}{n+1}\right) \right),\ \ k = 1\ldots,n \\
%  %   v_k[i] &= \sqrt{\frac{2}{n+1}} \sin\left(i\frac{k\pi}{n+1}\right),\ \  i = 1\ldots,n,\, k = 1\ldots,n. 
% %\end{eqnarray}

% Let $n$ be odd, then we can prolongate these onto a grid with $n_{\rm f} = (n-1)/2+1$ points by injection and linear interpolation (i.e. averaging). 

% In Fig. \ref{fig:unit_square1} we display the number of iterations needed to reach a relative tolerance of $10^{-12}$ for $\omega = 10,11,\ldots,70$ using $n = \lceil 4 \omega \rceil -1$ and with the number of eigenvalues in the deflation space being $\lceil 0.005N \rceil $. The figure to the right also includes the number of iterations needed for the standard CG algorithm.

% We note that the computations only computed the eigenvectors by prolonging those from a coarser grid, the matrix $\matW^T \whiA$ was formed using the prolonged eigenvectors. We next consider the case when also $\matW^T \whiA$ is computed on a coarse grid.

% \begin{figure}[htb]
% \begin{center}
% \includegraphics[width=0.45\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/unit_square_iter2}
% \includegraphics[width=0.45\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/unit_square_iter1}
% \caption{Number of iterations needed to reach tolerance $10^{-12}$ for deflation using eigenvalues/eigenvectors computed on the grid (DCG) and using prolongated eigenvectors computed on a grid coarsened by a factor of 2 (DCG-prolonged). To the right results for CG is included for reference.  \label{fig:unit_square1}}
% \end{center}
%  \end{figure}


% \subsection{Experiments in Three Dimensions}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \clearpage

% \subsection{Experiments on the $d$-dimensional unit cube}
% In one dimension the eigenvalues and eigenvectors of the three-point center difference discretization $[-1,2,-1]$ of the Laplacian operator with a grid size $h=1/(n+1)$ with Dirichlet boundary conditions are
% \begin{subequations}
%     \begin{align}
%         &\lambda_k = 2\left(1-\cos(\frac{k\pi}{n+1})\right),\;k=1,\dots,n,\\
%         &\vb_k^n[i] =\sqrt{\frac{2}{n+1}}\sin\left(i\frac{k\pi}{n+1}\right),\;i=1,\dots,n,\;k=1,\dots,n. 
%     \end{align}
% \end{subequations}
% Let the matrix corresponding to this discretization be $L^{\textrm{(1d)}}_n$. Then $5$-point and $7$-point central difference of the  Laplacian operator for the unit square in 2D and unit cube in 3D can be written as
% \begin{equation}
% L^{\textrm{(2d)}}_n=L^{\textrm{(1d)}}_n\otimes I_{n}+I_{n}\otimes L^{\textrm{(1d)}}_n \quad\text{and}\quad
% L^{\textrm{(3d)}}_n=(L^{\textrm{(1d)}}_n\otimes I_{n})\otimes I_{n}+
% (I_{n}\otimes L^{\textrm{(1d)}}_n )\otimes I_{n}+
% I_{n}\otimes (I_{n}\otimes L^{\textrm{(1d)}}_n )
% \end{equation}
% respectively. 

% To test the deflation with eigenvectors computed on a coarse mesh and then prolonged to a fine grid, we consider $n=2^l-1$ interior points along one direction.

% Besides the original DCG algorithm, we also consider two modified version of it. We call the first modified version DCG-D. We invert the diagonal part of $W^TAW$, namely $\textrm{diag}(W^TAW)$, instead of $W^TAW$. With $A$ being SPD and $W$ being eigenvectors of $A$ $W^TAW$ is diagonal, however, when $W$ is constructed with prolonged eigenvectors $W^TAW$ is not exactly diagonal. In the second modified version of DCG we drop  $ {\bm \mu} \gets (\matW^T \whiA \matW)^{-1} (\matW^T \whiA \rb)$ in the inner loop of Algorithm \ref{alg:DCG}, and we call it DCG-OI.  

% We investigate the relation between number of iterations for the relative residual below $10^{-7}$ and the dimension of deflation space. We consider a problem with point source on the center of the computational domain $[0,1]^d$ with $d=1,2,3$.  In 1D the number of grid points is $n=2^{\lceil\log_2(\lceil16\omega\rceil)\rceil}-1$. In 2D we use 
% $n=2^{\lceil\log_2(\lceil4\omega\rceil)\rceil}-1$ grid points along one direction.

% \textcolor{blue}{Comment on the observations.}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{figure}[htb]
% \begin{center}
% \includegraphics[width=0.32\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/regular_geometry/1d_iter_eig1_orig.eps}
% \includegraphics[width=0.32\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/regular_geometry/1d_iter_eig1_diag.eps}
% \includegraphics[width=0.32\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/regular_geometry/1d_iter_eig1_no.eps}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \includegraphics[width=0.32\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/regular_geometry/1d_iter_eig75_orig.eps}
% \includegraphics[width=0.32\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/regular_geometry/1d_iter_eig75_diag.eps}
% \includegraphics[width=0.32\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/regular_geometry/1d_iter_eig75_no.eps}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \includegraphics[width=0.32\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/regular_geometry/1d_iter_eig5_orig.eps}
% \includegraphics[width=0.32\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/regular_geometry/1d_iter_eig5_diag.eps}
% \includegraphics[width=0.32\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/regular_geometry/1d_iter_eig5_no.eps}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \includegraphics[width=0.32\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/regular_geometry/1d_iter_eig25_orig.eps}
% \includegraphics[width=0.32\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/regular_geometry/1d_iter_eig25_diag.eps}
% \includegraphics[width=0.32\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/regular_geometry/1d_iter_eig25_no.eps}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \caption{Number of iterations as a function of frequency on 1D unit interval.\label{fig:iter_vs_omega_1d}}
% \end{center}
%  \end{figure}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{figure}[htb]
% \begin{center}
% \includegraphics[width=0.32\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/regular_geometry/2d_iter_eig2_orig.eps}
% \includegraphics[width=0.32\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/regular_geometry/2d_iter_eig2_diag.eps}
% \includegraphics[width=0.32\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/regular_geometry/2d_iter_eig2_no.eps}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \includegraphics[width=0.32\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/regular_geometry/2d_iter_eig15_orig.eps}
% \includegraphics[width=0.32\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/regular_geometry/2d_iter_eig15_diag.eps}
% \includegraphics[width=0.32\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/regular_geometry/2d_iter_eig15_no.eps}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \includegraphics[width=0.32\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/regular_geometry/2d_iter_eig1_orig.eps}
% \includegraphics[width=0.32\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/regular_geometry/2d_iter_eig1_diag.eps}
% \includegraphics[width=0.32\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/regular_geometry/2d_iter_eig1_no.eps}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \includegraphics[width=0.32\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/regular_geometry/2d_iter_eig05_orig.eps}
% \includegraphics[width=0.32\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/regular_geometry/2d_iter_eig05_diag.eps}
% \includegraphics[width=0.32\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/regular_geometry/2d_iter_eig05_no.eps}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \caption{Number of iterations as a function of frequency on 2D unit square.\label{fig:iter_vs_omega_1d}}
% \end{center}
%  \end{figure}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \newpage

% Line 17: 
% \begin{align}
% W^TAW=D+B=D+U\Sigma U^T
% =UDU^T+U\Sigma U^T
% = U(D+\Sigma)U^T\\
%  U(D+\Sigma)^{-1}U^T\\
% D^{-1}W^TAW=D^{-1}(D+U\Sigma U^T)
% = I + D^{-1} U\Sigma U^T
% \end{align}
% Von-Neumann series converges fast.
% %\end{comment}




==> tex/mainV1.tex <==
%!TEX root = ../deflation.tex
\section{WaveHoltz method for the Helmholtz equation\label{sec:waveholtz}}
We use the WaveHoltz method \cite{appelo2020waveholtz} to solve the Helmholtz equation 
\begin{align}
\omega^2 u + \nabla \cdot (c(\bx)^2 \nabla u) = f(x), \ \  \bx \in \Omega, \label{eq:helmholtz}
\end{align}
with the energy conserving homogenuous Dirichlet boundary condition
\begin{align}
u(\bx) = 0, \ \ \bx \in \Gamma=\partial \Omega.
\end{align}
Here, frequency $\omega$ is not a resonance.
WaveHoltz method is an iterative solver built on a time-domain solver for the wave equation 
\begin{subequations}
\begin{align}
    &\hat{u}_{tt}=\nabla \cdot (c(\bx)^2 \nabla \hat{u})-f(\bx)\cos(\omega t),\\
    &\hat{u}(\bx,t)=0,\ \ \bx\in \partial\Omega,\\
    &\hat{u}(\bx,0)=\nu(\bx),\\
    &\hat{u}_t(\bx,0)=0.
\end{align}
\label{eq:wave}
\end{subequations}
A filtering operator acting on the initial condition of the wave equation $\nu(\bx)$ is introduced as
\begin{align}
    \Pi \nu(\bx) = \frac{2}{T}\int_{0}^{T}(\cos(\omega t)-\frac{1}{4})\hat{u}(\bx,t) dt,
\end{align}
where $\hat{u}(\bx,t)$ is the time-domain solution determined by the initial condition $\nu(x)$. Operator $\Pi$ filters the time-domain solution 
 over one period.
As shown in \cite{appelo2020waveholtz}, the solution to the Helmholtz equation \eqref{eq:helmholtz} $u$ is a fixed point of the filtering operator $\Pi$ and the corresponding time-domain solution is $\hat{u}(\bx,t)=u(\bx)\cos(\omega t)$. In other words, the Helmholtz equation is equivalent to the fixed point problem
\begin{equation}
    \Pi u = u.
\end{equation}
This fixed point problem can be further rewritten as an equivalent linear problem 
\begin{align}
    (I-S)u = \Pi 0,\label{eq:I_minus_S}
\end{align}
where the linear operator $S$ is defined as $Su = \Pi u -\Pi 0$. 
After discretization, the resulting linear system can be solved by a Krylov subspace method. Moreover, with homogeneous Dirichlet boundary conditions, this linear system is proved to be  symmetric positive definite (SPD) \cite{appelo2020waveholtz}. As a result, conjugate gradient (CG) method can be applied to solve it.

\input ./tex/discretizationV1.tex


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Convergence theory of WaveHoltz method}
The convergence speed of the WaveHoltz method can be analyzed by utilizing the eigenmodes of the Laplacian operator $-\nabla\cdot(c(x)^2\nabla)$.
With the homogeneous Dirichlet boundary conditions, the operator $-\nabla\cdot(c(x)^2\nabla)$ has a point spectrum with positive eigenvalues $\lambda_j^2$ and corresponding eigen-functions $\phi_j$. These eigen-functions form a basis of $L^2(\Omega)$. Then, any function $\nu(x)\in L^2(\Omega)$ can be expanded as $\nu=\sum_{j=0}^\infty\hat{\nu}_j\phi_j$. 

Following \cite{appelo2020waveholtz,garcia2022extensions}, the linear operator $S: L^2(\Omega)\rightarrow L^2(\Omega)$ operator can be written as:  
\begin{align}
    S:\sum_{j=0}^\infty \hat{\nu}_j\phi_j\rightarrow \sum_{j=0}^\infty\beta(\lambda_j;\omega)\hat{\nu}_j \phi_j,
\end{align}
where 
\begin{align}
    \beta(\lambda;\omega) = \frac{2}{T}\int_{0}^{T}(\cos(\omega t)-\frac{1}{4})\cos(\lambda t)dt,
    \label{eq:beta_fun}
\end{align}
and the eigenvalues of $S$ are $\beta(\lambda_j;\omega)$.
As shown in \cite{appelo2020waveholtz,garcia2022extensions}, $-0.5\leq\beta(\lambda;\omega)\leq 1$ and the spectral ratio of $S$ scales as $$\rho_S \sim 1-O(\delta^2)<1,$$ where $\delta =\min_{\lambda_j}\frac{\lambda_j-\omega}{\omega}$. As a result, the largest eigenvalue of $I-S$ is bounded $0<\lambda^{I-S}_{\max}\leq 1.5$, and the smallest eigenvalue scales as $\lambda^{I-S}_{\min} \sim O(\delta^2)$. Thus, the condition number of $I-S$ scales as $O(\delta^2)$, and Weyl proved $\delta\sim O(\omega^d)$ \cite{weyl1912asymptotische}. As a result, the condition number of $I-S$ scales as $O(\omega^{2d})$, which implies that CG method  needs  $O(\omega^d)$ iterations for convergence. 

%As presented in \cite{saad2000deflated}, the convergence 
%If one can introduce a deflation space to remove the eigenvalues of $S$ which are close to $1$, the CG iterative solver can be accelerated.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsection{Eigenvalues of discrete WaveHoltz operator\label{sec:waveholtz-eig}}
The eigenvalues of the discrete WaveHoltz operator $S_h$ can be obtained based on the eigenvalues of the discrete Laplacian operator $L_h$. Suppose $\{-\lambda_{h,j}^2\}_{j=1}^{N}$ are the eigenvalues of $L_h$ and $\{\wb_j\}_{j=1}^{N}$ are the corresponding eigenvectors. 
One can verify that $\wb_j^h$ is also an eigenvector of the discrete WaveHoltz operator $I-S_h$:
\begin{equation}
    (I-S_h)\wb_j = (1-\beta_h(\lambda_j;\omega))\wb_j, \label{eq:waveholtz_eigvectors}
\end{equation} 
where
\begin{subequations}
\begin{align}
    &\beta_h(\lambda_j;\omega) = \frac{2\Dt}{T}\sum_{j=0}^{N_t}\eta_n\mu^n_j,\quad  \eta_n=\begin{cases}
            \half,\quad n=0\;\text{or}\; n=N_t,\\
            1,\quad\text{otherwise}, 
           \end{cases}\\
    &\mu_j^{n+1}=2\mu_j^n-\mu_j^{n-1}-\frac{\widetilde{\omega}^2}{\omega^2}\Dt^2 \mu_j^n\lambda_{j}^2,\quad 0\leq n\leq N_t-1,\\
    &\mu_j^0 = 1, \quad \mu_j^{-1}=\mu^0+\frac{\widetilde{\omega}^2}{\omega^2}\frac{\Dt^2}{2}\lambda_{j}^2.
\end{align}
\end{subequations}





%%%%%%%%%%%%%%%%%%% 
\section{Deflated conjugate gradient (DCG) method\label{sec:dcg}} 
With energy conserving boundary conditions, the WaveHoltz method for Helmholtz equation or time-harmonic Maxwell's equations results in an SPD linear system, allowing CG method to solve it. However, energy conserving boundary conditions lead to trapped wave structures, and the number of iterations for convergence needed by CG scales as $O(\omega^{d})$ in the worst case, where $d$ is the dimension of the problem. For 3D high frequency problem, many iterations may be required, resulting in a high computational cost, especially when solutions corresponding to many right-hand sides are desired.

To accelerate the convergence of the WaveHoltz method for such cases, we apply the deflated conjugate gradient (DCG) method \cite{saad2000deflated} by adding (approximated) eigenvectors associated with the smallest eigenvalues to the Krylov subspace.
 
In this section, we will first review the DCG algorithm and its convergence theory \cite{saad2000deflated} in Sec. \ref{sec:dcg_algorithm}, and then discuss how to choose the deflation space in Sec. \ref{sec:deflation} and Sec. \ref{sec:deflation-band}.  
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{DCG algorithm  and its convergence theory \label{sec:dcg_algorithm}}
%Assume $A$ is a SPD linear system. %Particularly, we denote $A$ as $A_h$ if it is corresponding to a discrete operator derived from a finite difference approximation of a partial differential equation (PDE) with mesh size $h$.


Consider an SPD linear system $A\xb=\bbb\in\mathbb{R}^N$. Given an initial guess $\xb_0$, in the $k$-th iteration, the CG method seeks the solution $\xb_k$ in the Krylov subspace 
\begin{equation}
    \xb_0+\mathcal{K}(\rb_0,\whiA,k)=\xb_0+\{\rb_0,\whiA\rb_0,\dots,\whiA^{k-1} \rb_0\},\quad \rb_0=\bbb-\whiA\xb_0,
\end{equation}
corresponding to the optimal error with respect to the $||\cdot||_A$ norm,  $||\yb||_A=\sqrt{\yb^T\whiA\yb}$. In other words,
\begin{align*}
\xb_k = \min_{\hat{\xb} \in \xb_0+\mathcal{K}(\rb_0,\whiA,k)}||\xb-\hat{\xb}||_A.
\end{align*}
The DCG method augments the Krylov subspace  with a deflation space, which is the column space of a deflation matrix $W\in\mathbb{R}^{N\times K}$. The DCG method initializes $\xb_0$ in the deflation space such that $$W^TA(\xb_0-\bbb)=W^T\rb_0=0$$ and performs a CG search in the subspace $A$-orthogonal to the deflation space. 
This strategy results in the DCG algorithm \cite{saad2000deflated}, which is presented in Algorithm \ref{alg:DCG}.

As discussed in \cite{saad2000deflated}, the DCG method can be seen as a preconditioned CG method with the preconditioner $PP^T$, where $P$ is the projector onto the $A$-orthogonal complement of the deflation space determined by $W$:
\begin{equation}
    P = I-W(W^TA W)^{-1}W^TA.
\end{equation}
Utilizing this point of view, the convergence speed of the DCG method is analyzed in \cite{saad2000deflated}. 
\begin{thm}\label{thm:dcg}
(Theorem 4.3 of \cite{saad2000deflated})
Let $\kappa_{P^TAP}$ be the condition number of $P^TAP$. The approximated solution of $A\xb=\bbb$ generated by the $j$-th iteration of the DCG algorithm in Algorithm \ref{alg:DCG} satisfies
\begin{equation}
    ||\xb-\xb_j||_A\leq2\left(\frac{\sqrt{\kappa_{P^TAP}}-1}{\sqrt{\kappa_{P^TAP}}+1}\right)^j|| \xb-\xb_0||_A, \quad ||\yb||_A=\sqrt{\yb^TA\yb}.
\end{equation} 
\end{thm}


%If eigenvectors corresponding to smallest eigenvalues of $\whiA$ are inside or well approximated by vectors in the deflation space $W$, the convergence of CG will be accelerated.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{algorithm}
\caption{DCG($\whiA,\bbb,W$): deflated conjugate gradient to solve $\whiA\xb=\bbb$ with the deflation matrix $W$.}\label{alg:DCG}
\begin{algorithmic}[1]
\State Input: $\whiA$, $\bbb$ and $W$.
\State $\xb_{-1}=0$
\State $\rb_{-1} = \bbb-\whiA \xb_{-1}$
\State $\xb_0 =  \xb_{-1} + W (\matW^T \whiA \matW)^{-1} ( \matW^T \rb_{-1} )$
\State $ \rb_0 = \bbb - \whiA \xb_0 $
\State $\etab_0 = \matW^T \whiA \rb_0$
\State $ {\bm \mu_0} = (\matW^T \whiA \matW)^{-1} \etab_0$
\State $ \pb_0 = \rb_0 - \matW {\bm \mu_0}$
\State $ r_2 = \rb^T \rb$
\State $ r_0 = r_2$
\State $k\ge 0$
\While{$r_2/r_0 > {\rm (TOL)}^2$ }
 \State  $\qb_k  = \whiA \pb_k$
 \State  $\alpha_k \gets r_2/ (\pb_k^T \qb_k)$
 \State  $\xb_{k+1} = \xb_k + \alpha_k \pb_k$
 \State  $ \rb_{k+1} = \rb - \alpha_k \qb$
 \State  $ \hat{r}_2 \gets r_2$
 \State  $ r_2 \gets \rb_{k+1}^T \rb_{k+1}$
  \State  $ \beta_{k+1} \gets  r_2/\hat{r}_2$
 \State $\etab_{k+1} = \matW^T \whiA \rb_{k+1}$
 \State $ {\bm \mu_{k+1}}= (\matW^T \whiA \matW)^{-1} \etab_{k+1}$
  \State  $ \pb_{k+1} = \beta_{k+1} \pb_k+\rb_{k+1} - \matW \mu_{k+1}$
  \State $k \gets k+1$
\EndWhile
\end{algorithmic}
\end{algorithm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{algorithm}
\caption{Eig-DCG($\whiA,\bbb,W$): eigenvector deflated conjugate gradient to solve $\whiA\xb=\bbb$.}\label{alg:eig-DCG}
\begin{algorithmic}[1]
\State Input: $\whiA$, $\bbb$ and $W$.
\State $\xb_{-1}=0$
\State $\rb_{-1} = \bbb-\whiA \xb_{-1}$
\State $\xb_0 =  \xb_{-1} + W (\matW^T \whiA \matW)^{-1} ( \matW^T \rb_{-1} )$
\State $ \rb_0 = \bbb - \whiA \xb_0 $
\State $\etab_0 = \matW^T \whiA \rb_0$
\State $ {\bm \mu_0} = (\matW^T \whiA \matW)^{-1} \etab_0$
\State $ \pb_0 = \rb_0 - \matW {\bm \mu_0}$
\State $ r_2 = \rb^T \rb$
\State $ r_0 = r_2$
\State $k\ge 0$
\While{$r_2/r_0 > {\rm (TOL)}^2$ }
 \State  $\qb_k  = \whiA \pb_k$
 \State  $\alpha_k \gets r_2/ (\pb_k^T \qb_k)$
 \State  $\xb_{k+1} = \xb_k + \alpha_k \pb_k$
 \State  $ \rb_{k+1} = \rb - \alpha_k \qb$
 \State  $ \hat{r}_2 \gets r_2$
 \State  $ r_2 \gets \rb_{k+1}^T \rb_{k+1}$
  \State  $ \beta_{k+1} \gets  r_2/\hat{r}_2$
  \State  $ \pb_{k+1} = \beta_{k+1} \pb_k+\rb_{k+1}$
  \State $k \gets k+1$
\EndWhile
\end{algorithmic}
\end{algorithm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{rem}
The main modifications to the CG algorithm made by the deflation method are as follows.
The line $3$ of Algorithm \ref{alg:DCG} constructs  an initial guess $\xb_0\in W$ such that  
\begin{align*}
W^T\rb_0 &= W^T(\bbb-\whiA\xb)=W^T\bbb - W^T\whiA\left(\xb_{-1}+AW(W^TAW)^{-1}W^T\rb_{-1}\right)\notag\\
         &=W^T\bbb - W^T\whiA\xb_{-1}+W^TAW(W^TAW)^{-1}W^T\rb_{-1}= W^T\rb_{-1}-W^T\rb_{-1}=0.
\end{align*}
Line $5,6,20$ and $21$ of Algorithm \ref{alg:DCG} enforce the search direction $\pb_{k}$ to be $A$-orthogonal to the deflation space $W$.
\end{rem}







\subsection{Eigenvector and prolonged eigenvector deflation matrix \label{sec:deflation}}
When eigenvectors are used as the deflation matrix, after initialization through the projection onto the deflation space which is a span of eigenvectors, the Krylov vectors generated by the CG algorithm is always $A$-orthogonal to each other \cite{saad2000deflated}. In other words, when eigenvectors are chosen as the deflation matrix, line 20-22 in Alg. \ref{alg:DCG} enforcing $A$-orthogonality after each iteration is not necessary. Dropping these unnecessary lines result in the simplified eigenvector deflated DCG (eig-DCG) algorithm in Alg. \ref{alg:eig-DCG}.


However, the computational cost of directly computing eigenvectors sometimes could be unaffordable. Alternatively, we can approximate eigenvectors through prolongation from coarser meshes. Let $A_h$ represent a linear system originating from a spatial discretization using mesh size $h$. We can use prolonged eigenvectors obtained  through linear interpolation of eigenvectors from coarser meshes (e.g., eigenvectors $A_{2h},A_{4h}$). On one hand, these prolonged eigenvectors can be obtained with less computational cost. On the other hand, using prolonged eigenvectors breaks the $A$-orthogonality required by the simplified Algorithm in Alg. \ref{alg:eig-DCG}. As a result, we need to use the original DCG method in Alg. \ref{alg:DCG} which enforces $A$-orthogonality in every iteration, otherwise DCG may lose its robustness \cite{saad2000deflated}. 

The condition number of the eigenvector-deflated system $P^TAP$ is discussed in Sec. 5 of \cite{saad2000deflated}, and we summarize it as a theorem here.
\begin{thm}(Sec. 5 of \cite{saad2000deflated})\label{lem:kappa}
Let the eigenvalues of $A$ be $0< \tilde{\lambda}_1\dots\leq\tilde{\lambda}_N$. If the columns of the deflation matrix 
$$W=\left(\wb_1,\wb_2,\dots,\wb_K\right)$$ are  eigenvectors corresponding to $\tilde{\lambda}_1,\dots,\tilde{\lambda}_K$, then the condition number of  $P^TAP$
is $\kappa_{P^TAP}=\frac{\tilde{\lambda}_N}{\tilde{\lambda}_{K+1}}$.
\end{thm}
The eigenvector deflation essentially reduces the condition number of the linear system from $\frac{\tilde{\lambda}_N}{\tilde{\lambda}_1}$ to $\frac{\tilde{\lambda}_N}{\tilde{\lambda}_{K+1}}$. When eigenvectors of the system $A_h$ are well approximated on a coarse mesh, using prolonged eigenvectors as the deflation matrix leads to a deflated system whose condition number is close to $\tilde{\lambda}_N/\tilde{\lambda}_{K+1}$.
A key difference between the eigenvector and prolonged eigenvector deflation is as follows. When columns of $W$ are eigenvectors of $A_h$, one can easily verify that $W^TA_hW$ is a diagonal matrix whose $k$-th diagonal element is $\tilde{\lambda}_k$. Thus, the computational cost of applying $(W^TA_hW)^{-1}$ is $O(K)$.
However, when prolonged eigenvectors are utilized, $W^TA_hW$ is not diagonal, potentially increasing the computational cost of applying $(W^TAW)^{-1}$ to $O(K^2)$.


\begin{rem}
As demonstrated in Appx. \ref{sec:A-orthogonality}, using exact eigenvector deflation eliminates the need to perform line $5,6,20$ and $21$ of Alg \ref{alg:DCG} to enforce $A$-orthogonality. However, in practice, we still execute these lines due to numerical considerations. Eigenvectors of $A$ are usually numerically computed. Without executing these lines of Alg. \ref{alg:DCG}, accumulations of numerical errors over iterations may lead to the loss of $A$-orthogonality. This loss further causes slower convergence.
\end{rem}

\begin{rem}
As pointed out in \cite{kruvzik2018implementace}, besides (approximated) eigenvectors, there are alternative choices for the deflation matrix. For example, it can also be chosen as a prolongation matrix from a geometric or an algebraic multigrid method  \cite{dwarka2020scalable}, subdomain aggregation \cite{nicolaides1987deflation} and discrete Wavelet compression \cite{kruzik2017wavelet}. 
\end{rem}

\begin{rem}
In an abstract formulation, authors of \cite{tang2010comparison} systematically analyze and compare the deflation method and the two-grid method \cite{mandel1993balancing}. They prove that, with careful design, a prolongation based deflation method can achieve almost the same convergence property as a two-grid method.
\end{rem}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Same deflation for a narrow frequency band\label{sec:deflation-band}}
As discussed in Sec. \ref{sec:waveholtz-eig}, the discrete WaveHoltz operator shares identical eigenvectors with the discrete Laplacian operator for any frequency $\omega$. The eigenvectors corresponding to the smallest eigenvalues of the WaveHoltz operators for frequencies in a sufficiently narrow frequency bands are almost identical. Therefore, a shared deflation matrix may be utilized for various frequencies in a narrow band.






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Convergence speed of deflated WaveHoltz method\label{sec:waveholtz_deflation}}%\pzc{To-do: \cite{kahl2017deflated} analyzed how error of eigenvector computations influence convergence, we can probably use their theories to analyze the mulitilevel deflation as well.}

To accelerate the convergence of the WaveHoltz method for energy conserving problems with trapped wave structures, we apply the DCG algorithm with eigenvectors or prolonged eigenvectors as the deflation matrix.
Here, we formally analyze the relation between the number of  eigenvectors in the deflation space and the convergence speed. 
For simplicity, we consider a homogeneous velocity field with $c(\xb)=1$. We first present the analysis results in Sec. \ref{sec:analysis-result}, followed by details of the analysis  in Sec. \ref{sec:analysis-procedure}. 


\subsection{Relation between the number of eigenvectors and computational costs\label{sec:analysis-result}}
Assume a homogeneous velocity field $c(\xb)=1$, which allows us to utilize the Weyl's principle \cite{weyl1912asymptotische} to formally estimate the relation between the dimension of the eigenvector deflation space and the number of iterations needed for convergence of DCG. In this section, we present our main results.

\textbf{Relation between number of eigenvectors and number of iterations for convergence.} Assume $W$ comprising eigenvectors corresponding to the $K$ smallest eigenvalues of the discrete WaveHoltz operator $A=I-S_h$. With  sufficiently high frequency $\omega$,  sufficiently small mesh size $h$ and time step size $\Dt$, the DCG algorithm solving $A\ub=(I-S_h)\ub=\bbb$ converges with $$N^{\textrm{DCG}}_{\textrm{iter}}\approx\frac{C_{\textrm{iter}}}{K}$$  iterations, where $C_{\textrm{iter}}$ represents a constant.

\textbf{Computational cost of the DCG in Alg. \ref{alg:DCG} and Eig-DCG in Alg. \ref{alg:eig-DCG} with the eigenvector deflation.}  When eigenvector deflation is applied, the deflation matrix $W\in\mathbb{R}^{N_{\textrm{DOF}}\times K}$ is a dense matrix, and $W^TAW\in\mathbb{R}^{K\times K}$ is a diagonal matrix leading to $O(K)$ computational cost of applying $(W^TAW)^{-1}$. Additionally, the matrix $W^TA\in\mathbb{R}^{N_{\textrm{DOF}}\times K}$ is dense and can be pre-computed. 
Utilizing these facts, computational cost of each step in the DCG algorithm is  estimated and summarized in Tab. \ref{tab:dcg-cost}.
\begin{table}[htbp]
  \centering
 \medskip
    \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|}
    \hline
	& Vector Operations  & Apply A  & Apply $W^TA$  & Apply $(W^TAW)^{-1}$ & Apply $W$  \\ \hline
 Line in Alg. \ref{alg:DCG} & $14-19, 22$ & $13$ & $20$ & $21$ & $22$ \\ \hline
 Cost &	$O(N_{\textrm{DOF}})$ & $N_tO(N_{\textrm{DOF}})$ & $KO(N_{\textrm{DOF}})$ & $O(K)$ & $KO(N_{\textrm{DOF}})$ \\
 	\hline
 \end{tabular}
      \caption{Computational cost of each steps in the DCG method Alg. \ref{alg:DCG} with the eigenvector deflation.\label{tab:dcg-cost}}
\end{table}

DCG converges with approximately $C_{\textrm{iter}}/K$ iterations. 
Consequently, the total cost of solving the WaveHoltz system $A\xb=(I-S_h)\xb=\bbb$ with DCG can be estimated as follows:
\begin{align}
\textrm{Cost}_{\textrm{DCG}} &\approx N^{\textrm{DCG}}_{\textrm{iter}}\times
\Big( \textrm{Vector Operations (line 14-19, 22)} + \textrm{Apply A (line 13)}\notag\\
&\quad\quad+\textrm{Apply $W^TA$ (line 20)} + \textrm{Solve $W^TAW$ (line 21)}+\textrm{Apply $W$ (line 22)}\Big)\notag\\
&= \frac{C_{\textrm{iter}}}{K}\times
\big(  O(N_\textrm{DOF})+N_t O(N_\textrm{DOF})+K O(\textrm{DOF})+O(K)\big)\notag\\
&=C_{\textrm{iter}}O(N_\textrm{DOF})\left(\frac{C_tN_t+C^{\textrm{DCG}}_{\textrm{vec}}}{K}+C_W+C_{W^TA}\right).\label{eq:cost19}
\end{align}
where $C_t, C^{\textrm{DCG}}_{\textrm{vec}},C_W$ and $C_{W^TA}$ 
 are constants. As a result, we would expect a sub-linear acceleration as we increase the number of eigenvectors $K$. 

Similarly, the cost of Eig-DCG with $K$-eigenvectors as the deflation amtrix can be estimated as:
\begin{align}
\textrm{Cost}_{\textrm{Eig-DCG}} &\approx N^{\textrm{Eig-DCG}}_{\textrm{iter}}\times
\Big( \textrm{Vector Operations (line 14-20)} + \textrm{Apply A (line 13)}\Big)\notag\\
&= \frac{C_{\textrm{iter}}}{K}\times
\big(  O(N_\textrm{DOF})+N_t O(N_\textrm{DOF})\big)\notag\\
&=C_{\textrm{iter}}O(N_\textrm{DOF})\left(\frac{C_tN_t+C^{\textrm{Eig-DCG}}_{\textrm{vec}}}{K}\right).\label{eq:cost19}
\end{align}
where $C_t, C^{\textrm{DCG}}_{\textrm{vec}},C_W$ and $C_{W^TA}$ 
 are constants. 
 

Without deflation, the computational cost of solving the WaveHoltz system with CG is approximately
\begin{align}
\textrm{Cost}_{\textrm{CG}} &\approx N^{\textrm{CG}}_{\textrm{iter}}\times
\left( \textrm{Vector Operations} + \textrm{Apply A }\right)\notag\\
&= N^{\textrm{CG}}_{\textrm{iter}} O(N_{\textrm{DOF}})(C_tN_t+C^{\textrm{CG}}_{\textrm{vec}}).
\end{align}
Therefore, the relative computational cost of the DCG method (Alg. \ref{alg:DCG}) and Eig-DCG method (Alg. \ref{alg:DCG}) with respect to the CG method are approximately
\begin{subequations}
\begin{align}
\textrm{Relative Cost of DCG}&=\frac{\textrm{Cost}_{\textrm{DCG}}}{\textrm{Cost}_{\textrm{CG}}} \approx 
    \frac{C_{\textrm{iter}}}{N_{\textrm{iter}}^{\textrm{CG}}}\left(\frac{\frac{1}{K}\left(C_tN_t+C^{\textrm{DCG}}_{\textrm{vec}}\right)+\left(C_W+C_{W^TA}\right)}{C_tN_t+C^{\textrm{CG}}_{\textrm{vec}}}\right),\\
  \textrm{Relative Cost of Eig-DCG}&=  \frac{\textrm{Cost}_{\textrm{DCG}}}{\textrm{Cost}_{\textrm{CG}}} \approx 
    \frac{C_{\textrm{iter}}}{N_{\textrm{iter}}^{\textrm{CG}}}\left(\frac{\frac{1}{K}\left(C_tN_t+C^{\textrm{Eig-DCG}}_{\textrm{vec}}\right)}{C_tN_t+C^{\textrm{CG}}_{\textrm{vec}}}\right).
\end{align}
\end{subequations}
In comparison with CG, DCG has overheads for applying $W$, $W^TA$ and $(W^TAW)^{-1}$ in each iteration, but it converges with fewer total iterations. Overall, with a proper chosen $K$, DCG achieves acceleration over CG. 



When prolonged eigenvectors are leveraged, the matrix $W^TAW$ is not diagonal anymore, potentially increasing the cost of applying $(W^TAW)^{-1}$ to $O(K^2)$. If eigenvectors on the fine mesh are well approximated by the prolonged eigenvectors from the coarse mesh, the estimated computational cost of solving the WaveHoltz system with DCG becomes
\begin{equation}
C_{\textrm{iter}}O(N_\textrm{DOF})\left(\frac{C_tN_t+C^{\textrm{DCG}}_{\textrm{vec}}}{K}+C'_W+C'_{W^TA}\right)+C'_{W^TAW} O(K)\label{eq:prolong_cost}
\end{equation}
where
$C'_W,C'_{W^TA},C'_{W^TAW}$ are constants. In practice, the number of eigenvectors in the deflation space, $K$, is much smaller than the total number of degrees of freedom $N_{\textrm{DOF}}$, and the $O(K)$ term in the computational cost \eqref{eq:prolong_cost} is almost negligible. We still expect a sub-linear acceleration, as we increase the number of eigenvectors $K$. 

%Since the cost of  applying the WaveHoltz operator is dominant, enlarging the number of prolonged eigenvectors $K$ initially results in computational saving. However, there may be no computational saving or even more computational costs when $K$ becomes too large.     

In our numerical tests, we observe that using a moderate number of eigenvectors or prolonged eigenvectors as the deflation matrix, we are able to gain almost linear acceleration over CG.%computational saving compared to CG. 

% \input tex/convergence_analysis.tex

\section{Numerical experiments\label{sec:numerical}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
To demonstrate the effectiveness of the proposed deflated  WaveHoltz method, we test it with a series of numerical examples. All the code is implemented in the {\tt Julia} programming language.

For problems with known analytical forms of eigenvalues and eigenvectors, we directly use their analytical form. For problems without known analytical forms, we use the Lanczos algorithm implemented in the {\tt KrylovKit.jl} package \cite{krylovkit} to compute the smallest eigenvectors of the WaveHoltz operators. In the Lanczos algorithm, the dimension of the Krylov space is set as $N_{K}=\max(2K,4\textrm{-ceil}(\omega))$, where $K$ is the desired number of eigenvectors, and $\omega$ is the frequency of the underlying problem. 

We define the relative number of iterations for convergence of DCG compared to CG
as
\begin{equation}
\textrm{Iter}_{\textrm{rel}}=\textrm{Iter}_{\textrm{DCG}}/\textrm{Iter}_{\textrm{CG}},
\end{equation}
where $\textrm{Iter}_{\textrm{CG}}$ and $\textrm{Iter}_{\textrm{DCG}}$ are number of iterations for convergence needed by CG and DCG respectively. Similarly, we can define relative computational of DCG compared to CG.


All the 2D tests are performed on an iMac machine with the Apple M1 chip, while all the 3D tests are conducted on the High Performance Community Computing Cluster (HPC3) of the Hong Kong University of Science and Technology (HKUST).

\clearpage
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{2D homogeneous problem\label{sec:2d-h}}
\deaa{Our first experiment for a case where the eigenvectors are known and thus can be easily found. A purpose of this experiment is to experimentally assess the various constants in cost estimate (\ref{eq:cost19})} 



We first consider a 2D homogeneous problem in the computational domain $[0,1]^2$ with the velocity field $c^2(x,y)=1$. A point source is located at $(x,y)=(0.1,0.1)$. For frequencies $\omega=25$ and $50$, we use a uniform mesh with $N=16\omega+1$ grid points in each direction. The relative tolerances in the stopping criteria for CG and DCG are set to $10^{-9}$.

\textbf{Prolonged eigenvectors as the deflation matrix.} The eigenvectors and eigenvalues for the discrete Laplacian operator are known analytically for this homogeneous problem. Therefore, following Sec. \ref{sec:waveholtz-eig}, we analytically compute the eigenvalues and eigenvectors of the discrete WaveHoltz operator. We compare the performance of using eigenvectors and prolonged eigenvectors as the deflation matrix. As presented in Fig. \ref{fig:2d_coarse_deflation},  using eigenvectors and approximated eigenvectors prolonged from $1$ to $3$-level coarsened meshes as the deflation matrix has similar performance. As the number of eigenvectors $K$ increases, the number of iterations for conevergence needed by DCG initially scales as approximately $O(K^{-0.85})$, and eventually bottom out. Computational time of DCG scales approximately $O(K^{-0.82})$. Compared to CG, DCG achieves at most approximately  $8$ times acceleration for $\omega=25$ and approximately  $25$ times acceleration for $\omega=50$.


%\textbf{Rectangle domain with different aspect ratios.} We consider a homogeneous rectangular domain $[0,1]\times[0,r]$ with frequency $\omega=150$ and PEC boundary conditions, where $0<r\leq 1$ is the aspect ratio. We use a uniform mesh with $601$ grid points along $x$-direction and $\lceil600r\rceil+1$ grid points alogn $y$-direction. Results are summarized in Fig. \ref{fig:2d_rectangle}.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[htb] 
\begin{center}
\includegraphics[width=0.4\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/iter_2d_h1.eps}\hspace{0.2cm}
\includegraphics[width=0.4\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/iter_2d_h2.eps}
\includegraphics[width=0.4\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/time_2d_h1.eps}\hspace{0.2cm}
\includegraphics[width=0.4\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/time_2d_h2.eps}
\caption{Relative and absolute number of iterations for convergence and computational time of DCG compared to CG for the 2D homogeneous problem in Sec. \ref{sec:2d-h}. Top: relative number of iterations for convergence. Bottom: relative computational time. \label{fig:2d_coarse_deflation}}
\end{center}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{figure}[htb]
%\begin{center}
%\includegraphics[width=0.4\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/iter_2d_h_rectangle.eps}
%\includegraphics[width=0.4\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/iter_2d_h2.eps}
%\caption{Relative number of iterations and computational time compared to CG for the 2D homogeneous problem in Sec. \ref{sec:2d-h}. \label{fig:2d_rectangle}}
%\end{center}
%\end{figure}

\clearpage

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{2D inhomogeneous problem\label{sec:2d-ih}}
We consider a 2D problem in the computational domain $[-1,1]^2$ with the velocity field 
\begin{equation}
    c^2(x,y) = 1.0-0.9\left( e^{-\left(\frac{x^2+(y-0.4)^2-0.4^2}{0.2^2} \right)^4}+e^{-\left(\frac{x^2+(y+0.4)^2-0.3^2}{0.2^2} \right)^4}\right).
\end{equation}
We consider frequencies $\omega=20,40,60$ and the source term
\begin{equation}
    f(x,y) = \frac{16\omega^2}{\pi}e^{-16\omega^2(x^2+y^2)}.
\end{equation}
We use a mesh with $N=8\omega$+1 grid points in each direction. The relative tolerances in the stopping criteria of CG and DCG are set as $10^{-10}$.
The tolerance of the residual for Schur vectors in the Lanczos algorithm to generate eigenvectors is $10^{-12}$.
The configuration of the velocity field and numerical solutions for frequencies $\omega=20,60$ are displayed in Fig. \ref{fig:reference-2d-ih}.

\textbf{Performance with different dimensions of the deflation space.} In Fig. \ref{fig:convergence_2d_ih}, we present the performance of DCG with different dimensions of the deflation space. The relative number of iterations  for convergence and relative computational time compared to the CG method approximately scale  as $O(K^{-0.9})$. With $50$ to $200$ eigenvectors, DCG achieves approximately $2.23$ to $15.39$ times acceleration compared to CG. As shown in the right picture of Fig. \ref{fig:convergence_2d_ih}, the computational time of obtaining eigenvectors corresponding to smallest eigenvalues takes approximately $3.25$ to $4.93$ times of CG.  %Accounting for the computational time of obtaining eigenvectors, we gain computational saving if solutions for more than $5$ to $8$ different right-hand sides are desired.

\textbf{Same deflation matrix for a  frequency band.} We utilize a uniform grid with $321$ grid points in each direction. Eigenvectors corresponding to the smallest $200$ eigenvalues of the WaveHoltz operator for the frequency $\omega=40$ serve as the deflation matrix for $\omega\in[37.5,42.5]$. The relative number of iterations for convergence and computational time of DCG compared to CG are displayed in Fig. \ref{fig:2d_windowed_deflation}. We observe that, for the frequency band $[37.5,42.5]$, DCG consistently converges with fewer iterations and smaller computational time than CG. Moreover, the closer the frequency to $\omega=40$, the greater the acceleration is achieved. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[htb]
\begin{center}
\includegraphics[width=0.32\textwidth,trim={1.5cm 0.15cm 2.5cm 0.25cm},clip]{figures/c_square_2d_ih.eps}
\includegraphics[width=0.32\textwidth,trim={1.5cm 0.15cm 2.5cm 0.25cm},clip]{figures/sol_2d_ih_20.eps}
%\includegraphics[width=0.40\textwidth,trim={1.5cm 0.15cm 2.5cm 0.25cm},clip]{figures/sol_2d_ih_40.eps}
\includegraphics[width=0.32\textwidth,trim={1.5cm 0.15cm 2.5cm 0.25cm},clip]{figures/sol_2d_ih_60.eps}
\caption{Configuration of the velocity field and  numerical solutions for the inhomogeneous 2D problem in Sec. \ref{sec:2d-ih}. \label{fig:reference-2d-ih}}
\end{center}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[htb]
\begin{center}
\includegraphics[width=0.32\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/iter_2d_ih.eps}
\includegraphics[width=0.32\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/time_2d_ih.eps}
\includegraphics[width=0.32\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/eig_time_2d_ih.eps}
\caption{Results for the 2D inhomogeneous 
 problem in Sec. \ref{sec:2d-ih}. Left:  relative and absolute number of iterations with respect to the CG method. Middle: relative computational time with respect to the CG method. Right: relative  eigenvector computational time with respect to the CG method.\label{fig:convergence_2d_ih}}
\end{center}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[htb]
\begin{center}
\includegraphics[width=0.4\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/iter_window_40.eps}
\includegraphics[width=0.4\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/iter_window_40_zoomed_in.eps}
\caption{Relative number of iterations and computational time of DCG compared to CG for the 2D inhomogeneous problem in Sec. \ref{sec:2d-ih}. \label{fig:2d_windowed_deflation}}
\end{center}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{3D homogeneous cube \label{sec:convergence_test_3d}}
We consider a 3D homogeneous problem with $c(x,y,z)=1$ and a point source term $\delta(x-0.1,y-0.1,z-0.1)$ in the computational domain $[0,1]^3$. We consider three different frequencies $\omega=20,\;25,\;30$. We partition the computation domain with a uniform mesh having $131$ grid points for $\omega = 20$, $181$ grid points for $\omega=25$ and $231$ grid points for $\omega=30$ in each direction. These number of grid points per direction is chosen based on the in the principle determining points per wave length to reach at least $2\%$ relative error. \pzc{cite Bill's paper here}. We set the relative tolerance in the stopping criteria of the CG and DCG solver as $10^{-9}$.

\textbf{Performance with different dimensions of the deflation space.} For this homogeneous medium, the eigenvalues of the the discrete WaveHoltz operator can be analytically computed. Based on this fact, we estimate the condition number of the deflated operator by $\frac{1.5}{\hat{\lambda}_{K+1}}$, where $\hat{\lambda}_{K+1}$ is the $K+1$-th smallest eigenvalue of the discrete WaveHoltz operator. The estimated condition number is displayed in the bottom left plot of Fig. \ref{fig:convergence_test_3d}. We observe that the estimated condition number approximately scales as $O(K^{-2})$  for all frequencies, where $K$ is the number of eigenvectors in the deflation space. This observation matches our analysis.

In the top and bottom right plots of Fig. \ref{fig:convergence_test_3d}, we present the number of iterations for convergence and relative computational time with respect to the CG method. For all frequencies, the number of iterations for convergence scales roughly as $O(K^{-0.9})$ before bottoming out. The relative computational time of DCG with respect to CG scales roughly as $O(K^{-0.9})$. In comparison with CG, when $K=300$, DCG achieves at most more than $10.46$ times acceleration for $\omega=20$,  $8.40$ times acceleration for $\omega=25$ and $10.01$ times acceleration for $\omega=30$. 

\textbf{Prolonged eigenvectors as the deflation matrix.} In Fig. \ref{fig:convergence_test_3d_window}, we compare the number of iterations for convergence  and computational time using prolonged eigenvectors and analytical eigenvectors. We observe that, for frequencies $\omega=20,25,30$, employing prolonged eigenvectors from the $1$-level or $2$-level coarsened mesh, DCG converges with number of iterations comparable to using fine level eigenvectors. However, using prolonged eigenvectors requires enforcing $A$-orthogonality in each iteration. As a result, the speed-up gained by using prolonged eigenvectors is less compared to using the fine level eigenvectors. 


In summary, prolonged eigenvectors as the deflation matrix performs well when the fine level eigenvectors are well approximated on the coarse mesh, otherwise it may suffer from significant efficiency decline.

\begin{figure}[htb]
\begin{center}
\includegraphics[width=0.32\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/iter_3d_20.eps}
\hspace{0.1cm}
\includegraphics[width=0.32\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/iter_3d_25.eps}
\hspace{0.1cm}
\includegraphics[width=0.32\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/iter_3d_30.eps}
\includegraphics[width=0.32\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/cond_3d.eps}
\includegraphics[width=0.32\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/time_3d.eps}
\caption{Results for the 3D  homogeneous cube in Sec. \ref{sec:convergence_test_3d}. Top: relative and absolute number of iterations. Bottom left: estimated conditional number of $W^TAW$. Bottom right: relative computational time with respect to the CG method.   \label{fig:convergence_test_3d}}
\end{center}
 \end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \begin{figure}[htb]
\begin{center}
\includegraphics[width=0.32\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/iter_3d_ml_20.eps}
\includegraphics[width=0.32\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/iter_3d_ml_25.eps}
\includegraphics[width=0.32\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/iter_3d_ml_30.eps}
\includegraphics[width=0.32\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/time_3d_ml_20.eps}
\includegraphics[width=0.32\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/time_3d_ml_25.eps}
\includegraphics[width=0.32\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/time_3d_ml_30.eps}
\caption{Performance of DCG for 3D  homogeneous cube with deflation matrices comprising prolonged eigenvectors  in Sec. \ref{sec:convergence_test_3d}.  Top: relative and absolute number of iterations for convergence. Bottom: relative computational time compared to CG. \label{fig:convergence_test_3d_window}}
\end{center}
 \end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{3D homogeneous ball\label{sec:3d-ball}}
We consider a 3D homogeneous problem   ball
$\{(x,y,z):\sqrt{x^2+y^2+z^2}\leq0.5\}$ 
with $c^2(\xb)=1$ and homogeneous boundary conditions. The source term is defined as
\begin{equation}
    f(x,y,z) = \frac{16\omega^2}{\pi}e^{-16\omega^2( (x-x_c)^2+(y-y_c)^2+(z-z_c)^2 )},
\end{equation}
where $\omega=25$ is the frequency of the underlying problem. The relative tolerances in the stopping criteria of CG and DCG are $10^{-9}$.

To handle the curvilinear geometry, we utilize the second order embedded  boundary (EB) finite difference method in \cite{peng2023universal}. This EB method use interior boundary points leads to a SPD discrete Laplacian operator, so CG solver can still be applied. Moreover, it also avoids small cell stiffness, so a standard CFL condition can still be used in the time-domain simulation of the wave equation.
In the EB method, we set computational domain as $[-0.55,0.55]^3$  and partition it by a uniform cartesian mesh with $220$ grid points in each direction. 

To construct the deflation matrix, we use Lanczos method to compute $100$ eigenvectors  and obtain $123$ converged eigenvectors. The tolerance of the residual for Schur vectors in the Lanczos algorithm is set as $10^{-10}$. The deflation matrix consists of all converged eigenvectors.

\textbf{Different source terms.} To test the performance of the proposed DCG methods for different source terms, we uniformly  pick $10$ different random center points for the source term $(x_c,y_c,z_c)$ inside the ball $\{\sqrt{x^2+y^2+z^2}\leq0.25\}$.

Results are summarized in Tab. \ref{tab:3d-ball}. We observe that, on average, the DCG algorithm converges with approximately $18.90\%$ number of iterations and leads to approximately $3.60$ times acceleration compared to CG. 
The computational time of constructing the deflation matrix is approximately $11.105$ times of the average time for one CG solve. As a result, we gain computational saving if the Helmholtz equation is solved for more than $16$ different source terms.   

\textbf{Same deflation for a narrow frequency band.} We use the deflation matrix constructed for $\omega=25$ to solve problems with $\omega=24.5,24.6,\dots,30.5$ and the source term corresponding to $(x_c,y_c,z_c)=(0.1,0.1,0.1)$. As displayed in Fig. \ref{fig:3d_ball_windowed_deflation}, we observe that, for all frequencies, DCG converges with less number of iterations than CG and achieves approximately $4.00$ to $5.21$ times acceleration compared to CG. %Surprisingly, though the deflation matrix consists of eigenvectors for $\omega=40$, we achieve the largest acceleration at $\omega=40.3$. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[htbp]
  \centering
 \medskip
    \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|}
    \hline
   $\textrm{Iter}_\textrm{CG}$ & $\textrm{Iter}_\textrm{DCG}$ & ${T}_{\textrm{DCG}}/{{T}_{\textrm{CG}}}$ & ${T_{\textrm{Eig}}}/{{T}_{\textrm{CG}}}$ \\ \hline
  $129.8$ & $20.1$ &  $0.278$ & 11.105 \\ \hline
 \end{tabular}
      \caption{Multiple source terms test for the 3D homogeneous ball in Sec. \ref{sec:3d-ball}. $K$: dimension of the deflation space. $\textrm{Iter}_\textrm{(D)CG}$: average number of iterations for (D)CG. $T_{\textrm{D}CG}$: average computational time for the (D)CG. $T_{Eig}$: computational time of obtaining eigenvectors needed by the deflation.  \label{tab:3d-ball}}
\end{table}

\begin{figure}[htb]
\begin{center}
\includegraphics[width=0.40\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/ball_25_various_frequencies.eps}
\caption{The same deflation for various frequencies for the homogeneous ball in Sec. \ref{sec:3d-ball}. Relative number of iterations and computational time of DCG compared to CG are displayed. \label{fig:3d_ball_windowed_deflation}}
\end{center}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{3D inhomogeneous problem\label{sec:3d-ih}}
We consider a 3D inhomoeneous problem on the computational domain $[-0.5,0.5]^3$ with the velocity field 
\begin{equation}
    c^2(x,y,z) = 1.0-0.9e^{-\left( \frac{x^2+y^2+z^2-0.25^2}{0.25^2}\right)^4 }
\end{equation}
and the frequency $\omega=20$.
We consider the source term \begin{equation}
    f(x,y,z) = \frac{16\omega^2}{\pi}e^{-16\omega^2( (x-x_c)^2+(y-y_c)^2+(z-z_c)^2 )},
\end{equation}
where $\omega$ is the frequency of the underlying problem.
We use a uniform grid with $181$ grid points in each direction. The relative tolearnces for the stopping criteria of CG and DCG are chosen as $10^{-9}$.

To construct a deflation matrix, we use Lanczos method to compute $80$ smallest eigenvectors of the WaveHoltz operator on the original mesh and $1$-level coarsend mesh. The tolerance of the residual for Schur vectors is $10^{-11}$. With no coarsening and $1$-level coarsening, the Lanczos algorithm converges with $63$ and $61$ iterations and results in $84$ and $93$ converged eigenvectors, respectively. When eigenvectors are computed on the coarse mesh, we interpolate it to the original mesh with  linear interpolation.



\textbf{Different source terms.} To test the performance of the proposed DCG method for different source terms, we uniformly  pick $10$ different random center points $(x_c,y_c,z_c)$ for the source term  inside the ball $\{\sqrt{x^2+y^2+z^2}\leq0.25\}$.

Results are summarized in Tab. \ref{tab:3d-ih}. On average, deflation matrices comprising eigenvectors and prolonged eigenvectors lead to approximately $27.5\%$ and $29.5\%$ number of iterations for convergence and $3.61$ and $2.79$ times acceleration compared to CG, respectively. 
The average computational time to obtain eigenvectors and prolonged eigenvectors are approximately $7.070$ and $0.595$ times of the average time for one CG solve. Accounting for the time of constructing the deflation matrix, we gain computational saving when solving more than $10$ source terms for the eigenvector deflation and $2$ source terms for the prolonged eigenvector deflation.  

\textbf{Performance with different dimensions of the deflation space.} With $(x_c,y_c,z_c)=(-0.4,0.45,0.4)$, we test the performance of DCG with different dimensions of the deflation space $K$. The corresponding numerical solution is presented in Fig. \ref{fig:3d_ih_solution} 
As shown in Fig. \ref{fig:3d_ih}, DCG method converges with less number of iterations and computational time compared to CG. The number of iterations and computational time for convergence approximately scale as $O(K^{-0.6})$. 

\textbf{Same deflation for a narrow frequency band.} We use the converged $84$ eigenvectors and $93$ prolonged eigenvectors for $\omega=20$ as the deflation matrix for frequencies in the band $[19.4,20.6]$. As displayed in Tab. \ref{fig:3d_ih}, both eigenvector and prolonged eigenvector deflation is faster than CG. For all tested frequencies except for $\omega=20.6$, using the fine level eigenvectors as the deflation matrix achieves more acceleration than using prolonged eigenvectors. %when the frequency $\omega$ is close to $20$, this deflation matrix results in less number of iterations for convergence and smaller computational time.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[htbp]
  \centering
 \medskip
    \begin{tabular}
    {|l|c|c|c|c|c|c|c|c|c|c|c|}
    \hline
Eigenvector computation & $K$ & $\textrm{Iter}_\textrm{CG}$ & $\textrm{Iter}_\textrm{DCG}$ &  $\textrm{Iter}_\textrm{Eig}$ & ${T}_{\textrm{DCG}}/{{T}_{\textrm{CG}}}$ & ${T_{\textrm{Eig}}}/{{T}_{\textrm{CG}}}$ \\ \hline
 No coarsening & $84$ &  $511.1$ & $140.6$ & $63$ & $0.277$ & $7.070$ \\ \hline
 $1$-level coarsening & $93$ & $511.1$ & $151$ & $61$ & $0.358$ & $0.696$ \\ \hline
 \end{tabular}
      \caption{Multiple source terms test for the 3D inhomogeneous problem in Sec. \ref{sec:3d-ih}. $\textrm{Iter}_\textrm{(D)CG}$: average number of iterations for (D)CG. $T_{\textrm{D}CG}$: average computational time for the (D)CG. $T_{Eig}$: computational time of obtaining eigenvectors needed by the deflation.  \label{tab:3d-ih}}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[htbp]
  \centering
 \medskip
    \begin{tabular}
    {|l|c|c|c|c|c|c|c|c|c|c|c|}
    \hline
 $\omega$ & $19.4$ & $19.6$ & $19.8$ & $20.0$ & $20.2$ & $20.4$ & $20.6$\\ \hline
 {$\textrm{Iter}_\textrm{DCG}/\textrm{Iter}_\textrm{CG}$, no coarsening} &  $0.458$&    $0.303$&    $0.289$&    $0.301$&    $0.335$&    $0.485$& $0.917$ \\ \hline
 {$\textrm{Iter}_\textrm{DCG}/\textrm{Iter}_\textrm{CG}$}, $1$-level coarsening &  $0.861$&    $0.473$ &    $0.350$&    $0.321$ &    $0.248$ &    $0.301$    & $0.335$ \\ \hline
{${T}_{\textrm{DCG}}/{{T}_{\textrm{CG}}}$, no coarsening} &  $0.459$&    $0.300$   & $0.271$   & $0.301$    &$0.329$    & $0.488$    & $0.952$ \\ \hline
 {${T}_{\textrm{DCG}}/{{T}_{\textrm{CG}}}$, 1-level coarsening} &    $0.985$&    $0.607$&    $0.401$&    $0.423$&    $0.328$&    $0.377$&    $0.349$\\\hline 
 \end{tabular}
      \caption{Same deflation for frequencieis in a narrow band for the 3D inhomogeneous problem in Sec. \ref{sec:3d-ih}. $\textrm{Iter}_\textrm{(D)CG}$: average number of iterations for (D)CG. $T_{\textrm{(D)CG}}$: average computational time for the (D)CG.  \label{tab:3d-ih-window}}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[htb]
\begin{center}
\includegraphics[width=0.32\textwidth,trim={0.3cm 0.3cm 0.3cm 0.4cm},clip]{figures/sliced_solution_x.eps}
\includegraphics[width=0.32\textwidth,trim={0.3cm 0.05cm 0.3cm 0.4cm},clip]{figures/sliced_solution_y.eps}
\includegraphics[width=0.32\textwidth,trim={0.3cm 0.05cm 0.3cm 0.4cm},clip]{figures/sliced_solution_z.eps}
\caption{Slices of the numerical solution for 3D inhomogeneous problem in Sec. \ref{sec:3d-ih} with the source term corresponding to $(x_c,y_c,z_c)=(-0.4,0.45,0.4)$.  \label{fig:3d_ih_solution}}
\end{center}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%
 \begin{figure}[htb]
\begin{center}
\includegraphics[width=0.45\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/iter_3d_ih.eps}
\hspace{0.1cm}
\includegraphics[width=0.45\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/time_3d_ih.eps}
%\includegraphics[width=0.32\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/cube_20_various_frequencies.eps}
\caption{Results for 3D inhomogeneous problem in Sec. \ref{sec:3d-ih} with the source term corresponding to $(x_c,y_c,z_c)=(-0.4,0.45,0.4)$. Left: relative and absolute number of iterations for convergence for $\omega=20$. Right: relative computational time for $\omega=20$. \label{fig:3d_ih}}
\end{center}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Conclusions \label{sec:conclusion}}
In this paper, we propose a deflated WaveHoltz method to solve Helmholtz problem with multiple right hand sides and energy conserving boundary conditions which yield trapped wave structures. 

We formally show that using eigenvectors as the deflation matrix, the proposed deflated WaveHoltz method converges with a number of iterations approximately proportional to the  reciprocal  of number of eigenvectors, leading to a sub-linear saving of computational time. 

Our numerical experiments demonstrate the effectiveness of the proposed method. The WaveHoltz method is effectively accelerated by leveraging a deflation matrix consisting of eigenvectors or approximated eigenvectors prolonged from a coarse mesh, which effectively resolves the wave structure. Additionally, we also show that the same deflation matrix can be applied for problems with various frequencies in a narrow band. 

In the future, we plan to investigate using a deflation matrix based on reduced order models  for parametric problems \cite{cortes2018pod,panagiotopoulos2023accelerated}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\appendix
\section{$A$-orthogonality with exact eigenvector deflation\label{sec:A-orthogonality}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Here, we show that, when $W$ comprises exact eigenvectors of $\whiA_h$, there is no need to  impose $A$-orthogonality in DCG, as $A$-orthogonality is auntomatically guaranteed.

Expand $\rb_0$ as a linear combintation of eigenvectors $\rb_0=\sum_{j=1}^N r_j\wb_j$.
Since $W^T\rb_0=0$ we have $r_j=0$ with $j=1,\dots,K$. As a result 
\begin{equation*}
W^TA \rb_0 = \sum_{j={K+1}}^N W^T \lambda_j r_j\wb_j =0.
\end{equation*}
This guarantees ${\bm \mu_0}=0$ and $W^T \pb_0=0$. With mathematical induction one can show that ${\bm \mu_k}=0$ and $W^T\pb_{k}=W^T\rb_{k}=0$ for any $k$.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \bibliographystyle{plain}
% \bibliography{ref}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\clearpage
%%%%%%%%%%%%%%%%%
%\begin{comment}
%%%%%%%%%%%%%%%%%
\subsubsection{Accuracy needed for $(W^TAW)^{-1}$}
We need to apply $(W^TAW)^{-1}$ when we construct $\xb_0$ or impose $A$-orthogonality with respect to the deflation space to the search directions $\pb_k$. Here we will discuss how we implement $(W^TAW)^{-1}$ operation in practice.

When $W$ is formed eigenvectors of $A$, one can prove that $W^TAW$ is a diagonal matrix whose diagonal elements are the corresponding eigenvalues, and it is simple and computationally cheap to invert such a $W^TAW$.
When the size of $W^TAW$, $K$ is much smaller than $N$, we can directly factorize it to compute $W^TAW)^{-1}$. 
For a larger $W^TAW$, we can use a Krylov subspace iterative solver to invert it. The required accuracy for such solvers is numerically investigated in \cite{nabben2006comparison}, analyzed and further relaxed in \cite{kahl2017deflated}. The analysis in \cite{kahl2017deflated} suggests that given the sopping criterion for the DCG algorithm
$||\rb_k||\leq \varepsilon \bbb$, 
the required accuracy for the inner loop solving the linear system determined by $W^TAW$ is
\begin{equation}
    ||\rb_k^{\textrm{inner}}||\leq c\frac{\varepsilon}{||\rb_k||}||\bbb^{\textrm{inner}}|||,\quad 0\leq c<1.
\end{equation}
As the iteration continues, the residual in the DCG algorithm $||\rb_k||$ becomes smaller and the required accuracy for the inner loop solving $W^TAW$ can be adaptively enlarged.



\subsection{Eigenvalues for different geometries} (\textcolor{blue}: we should remove this Section)
The geometry of $\Omega$ affects the distribution and values of the eigenvalues of the $S$ operator. Here, we present the eigenvalues for a few different geometries.




\subsubsection{The Unit Square in $d$-dimensions}
The eigenvalues and eigenvectors of the three point discretization $[-1, 2, -1]$ of the Laplacian on $[0,1]$ with a grid size $h=1/(n+1)$ with Dirichlet boundary conditions are
\begin{eqnarray}
    \lambda_k &= 2 \left(1-\cos \left(\frac{k \pi}{n+1}\right) \right),\ \ k = 1\ldots,n \\
    w_k[i] &= \sqrt{\frac{2}{n+1}} \sin\left(i\frac{k\pi}{n+1}\right),\ \  i = 1\ldots,n,\, k = 1\ldots,n. 
\end{eqnarray}


\begin{figure}[htb]
\begin{center}
\includegraphics[width=0.46\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/beta_eig_contour_2d}
\includegraphics[width=0.5\textwidth]{figures/beta_eig_contour_3d}
\caption{Number of eigenvectors needed to reach $\beta_\omega(\lambda)<\beta$. Left: 2D. Right: 3D. \label{fig:beta_omega_contour}}
\end{center}
\end{figure}


\begin{figure}[htb]
\begin{center}
\includegraphics[width=0.5\textwidth]{figures/omega_ap_contour_2d}
\caption{Number of eigenvectors needed to reach $\beta_\omega(\lambda)<0.95$. \label{fig:beta_omega_contour}}
\end{center}
\end{figure}

\subsection{Multilevel DCG}
Constructing eigenvector deflation matrix may be costly especially when a refined grid is used. To mitigate this computational cost, we can design a multilevel DCG method which first converts $\whiA\xb=\bbb$ to a problem on a coarse grid  and then performs the eigenvector deflation on the coarse grid where the eigenvectors can be more efficiently computed.  

Multilevel DCG method can be designed following \cite{kruzik2017wavelet,kruvzik2018implementace}. Given a hierarchy of deflation matrix $W_l\in\mathbb{R}^{K_{l-1}\times K_l}$ with $l=1,\dots,L$ and $K_0=N$. Then the deflation matrix and the corresponding Galerkin matrix for the multilevel method are
\begin{equation*}
W = W_1W_2\dots W_L \quad\text{and}\quad W_L^T\dots W_2^T W_1^TAW_1W_2\dots W_L.
\end{equation*}
When solving $A\xb=\bbb$ we apply the DCG method with deflation matrix $W_1$, namely DCG($A,\bbb,W_1$). Inside DCG($A,\bbb,W_1$) we invert $W_1^TAW_1$ with a second DCG solver DCG($W_1^TAW_1,\cdot,W_2)$. We nest the DCG solve until we reach the last level $L$ and invert $W_L^TAW_L$ with a direct or Krylov solver.

Particularly we will apply the following prolongation based deflation (PED) when inverting the WaveHoltz linear system. For $l=1,\dots,L-1$, we choose $W_l$ as a prolongation from a coarse grid with $h_l=2^lh$ to a fine grid with $h_{l-1}=2^{l-1}h$ and choose $W_L$ as eigenvectors of the Galerkin matrix $W_{L-1}^T\dots W_1^T A W_1\dots W_{L-1}^T$ on the most coarse level. The eigenvectors will be only computed on the most coarse grid and there is no need to impose the $A$-orthogonality in the DCG solve for $W_{L-1}^T\dots W_1^T A W_1\dots W_{L-1}^T$. 


\begin{rem}
The multilevel DCG described above may be combined with the aforementioned idea of approximating eigenvectors based on information provided by successive solves of multiple right hand side \cite{saad2000deflated,stathopoulos2010computing}, and this combination is left for future investigation.    
\end{rem}

\subsection{Prolongation based eigenvector deflation for the WaveHoltz matrix $\whiA_h$}
Here we define a prolongation eigenvector deflation based a the linear prolongation, and we will find the eigenvectors for the most coarse Galerkin matrix $W_L^TW_{L-1}^T\dots W_1^T\whiA_h W_1W_2\dots W_L$. 

For simplicity we consider $1D$ Helmholtz problem $c(x)\equiv1$.
We first introduce the following grid. Assume $N$ be an even integer. Let $\Omega_h$ be a fine grid: $0=x_0\leq x_1 = h\leq \ldots\leq x_N=1$. Let $\Omega_{2h}$ be the coarse grid:
$0=x^c_0\leq x^c_1 = 2h\leq \ldots\leq x^c_{N/2}=1$. 
The fine grid  $\Omega_h$ and coarse grid $\Omega_{2h}$ with $N=8$ are illustrated in Fig. \ref{fig:fine-coarse-grid}. 
 Let $L_h$ denote the matrix corresponding to the $[-1,2,-1]$ central difference discretization  of $\Delta$ with the mesh size $h=\frac{1}{N}$.

We define the linear prolongation operator $I_{2h}^h$ which maps a grid function $\vb^{2h}$ on the coarse grid $\Omega_{2h}$ to a grid function  on the fine grid $\Omega_h$:
\begin{subequations}
    \begin{align}
    &I_{2h}^h\vb^{2h}_{2j} = \vb^{2h}_j,\;0\leq j\leq\frac{N}{2},\\
    &I_{2h}^h\vb^{2h}_{2j+1} =\half\left( \vb^{2h}_{j}+\vb^{2h}_{j+1}\right),\;0\leq j\leq\frac{N}{2}-1.
    \end{align}
\end{subequations}
The full weighting restriction operator mapping a grid function $\vb^h$ on $\Omega_h$ to a grid function $\Omega_{2h}$ is defined as:
\begin{equation}
(I_{h}^{2h}\vb^h)_{j}=\frac{1}{4}(\vb^h_{j-1}+2\vb^h_{j}+\vb^h_{j+1}), \; 1\leq j\leq \frac{N}{2}-1.
\end{equation}
The full weighting restriction $I_{h}^{2h}$ and the linear prolongation $I_{2h}^h$ satisfy the variational relation: 
\begin{equation}
    I_{h}^{2h} = \frac{1}{2} (I_{2h}^h)^T.\label{eq:variational_property}
\end{equation}
Since in the DCG algorithm $W_l^T$ only appears in $(W^TAW)^{-1}W^T$ terms one can actually replace $W_l^T$ with the restriction operator $I_{2^{l-1}h}^{2^lh}$ when implementing the algorithm.

In the $L$ level prolongation based eigenvector deflation we choose deflation matrices as
\begin{equation}
W_l = \begin{cases}
       I_{2^lh}^{2^{l-1}h}, \quad &1\leq l\leq L-1,\\ 
       \textrm{first $K$ eigenvectors of }W_{L-1}^T\dots W_1^T A W_1\dots W_{L-1}, \quad &l= L. 
       \end{cases}
\end{equation}
With $\whiA_h$ equal to the WaveHoltz operator $I-S_h$, we will show that the eigenvectors for $W_{L-1}^T\dots W_1^T \whiA_h W_1\dots W_{L-1}$ are the eigenvectors of the discrete Laplacian operator on the most coarse grid, $L_{2^Lh}$. 

\subsubsection{Eigenvectors of $W_{L-1}^T\dots W_1^T \whiA_h W_1\dots W_{L-1}$}
We start with proving eigenvectors of $W_1^T\whiA_h W_1$ are the eigenvectors of the discrete Laplacian operator $L_{2h}$. With the variational property \eqref{eq:variational_property}, it is enough to find eigenvectors for $I^{2h}_{h}\whiA I_{2h}^h$. 

The proof is based on the properties of the full weighting restriction and the linear prolongation \cite{briggs2000multigrid}. Let $\wb^h_k$ be an eigenvector of the discrete Laplacian operator $L_{h}$.
\begin{lem}\label{lem:restriction_and_prolong_effect}
Let $k'=N-k$. For $1\leq k < \frac{N}{2}$, following relations are satisfied:
\begin{subequations}
\label{eq:restri_prolong_equality}
\begin{align}
    I_{2h}^{h} \wb^{2h}_k &= c_k^{2h}\wb_k^h-s_k^{2h}\wb_{k'}^h,\label{eq:full_weight} \\
    I_{h}^{2h}\wb^h_k &= c_k^{2h}\wb_k^{2h},\label{eq:prolong_k}\\
    I_{h}^{2h}\wb^h_{k'} &= - s_k^{2h}\wb_k^{2h},\label{eq:prolong_kp}
\end{align}
\end{subequations}
where $c_k^{2h}=\cos^2(\frac{k\pi}{2N})$ and $s_k^{2h}=\sin^2(\frac{k\pi}{2N})$.
\end{lem}

\begin{thm}
Let $1\leq k< \frac{N}{2}$  and $L_{2h}\wb^{2h}_{k}=\sigma_k^2\wb^{2h}_{k}$. Then $\wb^{2h}_k$ is also an eigenvector of $I_{h}^{2h} \whiA_h I_{2h}^h$ with $\whiA_h$ being the WaveHoltz operator on $\Omega_h$ and 
\begin{equation}
I_{h}^{2h} \whiA_h I_{2h}^h\wb^{2h}_k =\left(\; 
(c_k^{2h})^2(1-\beta_h(\sigma_k))+(s_k^{2h})^2(1-\beta_h(\sigma_{k'}))\;\right)\wb_k^{2h}.\label{eq:projected_waveholtz_eig}
\end{equation}
with $k'=N-k$.
\end{thm}
\begin{proof}
Recall that eigenvectors of $L_h$ is also an eigenvector of $\whiA_h$ and satisfies \eqref{eq:waveholtz_eigvectors}. 
Utilizing equation \eqref{eq:full_weight} and \eqref{eq:waveholtz_eigvectors} we get
\begin{align}
\whiA_h I_{2h}^h\wb^{2h}_k &= \whiA_hc_k^{2h}\wb_k^h-\whiA_hs_k^{2h}\wb_{k'}^h\notag\\
&= (\;1-\beta(\sigma_k^h)\;)c_k^{2h}\wb_k^h-(\;1-\beta(\sigma_{k'}^h)\;)s_k^{2h}\wb_{k'}^h.
\end{align}
Then using \eqref{eq:prolong_k} and \eqref{eq:prolong_kp} we obtain
\begin{align}
I_{h}^{2h}\whiA_h I_{2h}^h\wb_{2h}^k &= (\;1-\beta(\sigma_k^h)\;)c_k^{2h}I_{h}^{2h}\wb_k^h-(\;1-\beta(\sigma_{k'}^h)\;)s_k^{2h}I_{h}^{2h}\wb_{k'}^h\notag\\
&=  (\;1-\beta(\sigma_k^h)\;)(c_k^{2h})^2\wb_k^{2h}+
(\;1-\beta(\sigma_{k'}^h)\;)(s_k^{2h})^2\wb_k^{2h}\notag\\
&=\left(\; 
(c_k^{2h})^2(1-\beta_h(\sigma_k))+(s_k^{2h})^2(1-\beta_h(\sigma_{k'}))\;\right)\wb_{k}^{2h}.
\end{align}
\end{proof}

Now we move to the multilevel case. The computation is similar but more involved.
\begin{thm}\label{thm:multilevel_eig}
Let $1\leq k<\frac{N}{2^{l}}$. Then the $k$-th eigenvector of the discrete Laplacian operator $L_{2^{l}h}$, $\wb_{k}^{2^lh}$, is an eigenvector of 
$I_{2^{l-1}h}^{2^lh}\dots I_{h}^{2h} \whiA_h I_{2h}^h\dots I_{2^lh}^{2^{l-1}h}$.
\end{thm}
\begin{proof}
Repeatedly using \eqref{eq:restri_prolong_equality}, we get
\begin{align*}
   I_{2^{l-1}h}^{2^lh}\dots I_{h}^{2h} \whiA_h I_{2h}^h\dots I_{2^lh}^{2^{l-1}h}w_{k}^{2^lh} &=
   I_{2^{l-1}h}^{2^lh}\dots I_{h}^{2h} \whiA_h I_{2h}^h\dots I_{2^{l-1}h}^{2^{l-2}h}
   \left(C_k^{(l)}\wb_{k}^{2^{l-1}h}+C_{\frac{N}{2^{l-1}}-k}^{(l)}\wb^{2^{l-1}h}_{\frac{N}{2^{l-1}}-k}\right)\notag\\
   &=I_{2^{l-1}h}^{2^lh}\dots I_{h}^{2h} \whiA_h
  \left( \sum_{j=1}^{2^{l-1}} C_{\frac{(j-1)N}{2^{l-1}}+k}^{(1)}\wb_{\frac{(j-1)N}{2^{l-1}}+k}^h
   +\sum_{j=1}^{2^{l-1}} C_{\frac{jN}{2^{l-1}}-k}^{(1)}\wb_{\frac{jN}{2^{l-1}}-k}^h\right)\notag\\
   &=I_{2^{l-1}h}^{2^lh}\dots I_{h}^{2h}\left( \sum_{j=1}^{2^{l-1}} \widetilde{C}_{\frac{(j-1)N}{2^{l-1}}+k}^{(1)}\wb_{\frac{(j-1)N}{2^{l-1}}+k}^h
   +\sum_{j=1}^{2^{l-1}} \widetilde{C}_{\frac{jN}{2^{l-1}}-k}^{(1)}\wb_{\frac{jN}{2^{l-1}}-k}^h\right)\notag\\
   &=I_{2^{l-1}h}^{2^lh}\dots I_{2h}^{4h}\left( \sum_{j=1}^{2^{l-2}} \hat{C}_{\frac{(j-1)N}{2^{l-1}}+k}^{(2)}\wb_{\frac{(j-1)N}{2^{l-1}}+k}^{2h}
   +\sum_{j=1}^{2^{l-2}} \hat{C}_{\frac{jN}{2^{l-1}}-k}^{(2)}\wb_{\frac{jN}{2^{l-1}}-k}^{2h}\right)\notag\\
   &= \hat{C}^{(l)}\wb_{k}^{2^lh},
\end{align*}
where all the $\hat{C}$, $\widetilde{C}$ and $C$ are generic constants. 
\end{proof}

A direct result of the variational property \eqref{eq:variational_property} and Theorem \ref{thm:multilevel_eig} is that eigenvectors of $W_{L-1}^T\dots W_1^T A_h W_1\dots W_{L-1}$ with $W_l=I_{2^{l+1}h}^{2^lh}$ are the eigenvectors of the discrete Laplacian operator $L_{2^{L}h}$. 

\subsubsection{Loss of Galerkin condition}
We also want to point out that the WaveHoltz operator $\whiA_h$ does not satisfy the Galerkin condition, in other words 
\begin{equation*}
    \whiA_{2h}\neq I_{h}^{2h}\whiA_hI_{2h}^h.
\end{equation*}
With the time stepping in \eqref{eq:modified_time_stepping} and the quadrature in \eqref{eq:quadrature} one can show that $\whiA_{h}\wb = P_{N_t}(L_h)\wb$ where 
$P_{N_t}(x)=\xi_0+\xi_1x+\dots+\xi_{N_t}x^{N_t}$ is a polynomial with $\xi_{N_t}\neq 0$.
If CFL conditions for the coarse grid $\Omega_{2h}$ and the fine grid $\Omega_h$ are the same, the total number of time steps will be different and $A_{2h}$ will be a polynomial of $L_{2h}$ but with adifferent degree. We can also use the same total number of time steps on the coarse level to get a modified coarse level WaveHoltz operator $\widetilde{\whiA}_{2h}=P_{N_t}(L_2h)$. Based on the Galerkin condition $L_{2h}=I_{h}^{2h}L_hI_{2h}^h$ we have
\begin{equation}
(L_{2h})^{n_t} = (I_{h}^{2h}L_hI_{2h}^h)^{n_t}= I_{h}^{2h}L_h (I_{2h}^hI_{h}^{2h})L_h\dots L_h(I_{2h}^hI_{h}^{2h})L_h I_{h}^{2h} \neq I_h^{2h} (L_h)^{n_t} I_{2h}^h,\quad \textrm{if} n_t\geq 1.
\end{equation}
 As a result $\widetilde{\whiA}_{2h}\neq I_{h}^{2h}\whiA_hI_{2h}^h$.
Without the Galerkin condition 
$\left(I_{h}^{2h}\whiA_h I_{2h}^h\right)^{-1}$ can not be inverted by directly applying the WaveHoltz solver on the coarse grid.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}
\begin{center}
\setlength{\unitlength}{0.8cm}
\begin{picture}(8,3) 
% Grid
\thicklines
\put(0,1){\line(1,0){8}}
\put(0,2){\line(1,0){8}}
% intervals on refined mesh
\put(0,2){\line(0,1){0.25}}
\put(1,2){\line(0,1){0.25}}
\put(2,2){\line(0,1){0.25}}
\put(3,2){\line(0,1){0.25}}
\put(4,2){\line(0,1){0.25}}
\put(5,2){\line(0,1){0.25}}
\put(6,2){\line(0,1){0.25}}
\put(7,2){\line(0,1){0.25}}
\put(8,2){\line(0,1){0.25}}
% intervalus on coarse mesh
\put(0,1){\line(0,1){0.25}}
\put(2,1){\line(0,1){0.25}}
\put(4,1){\line(0,1){0.25}}
\put(6,1){\line(0,1){0.25}}
\put(8,1){\line(0,1){0.25}}
% index for grid points on refined mesh
\put(-0.1,2.3){$0$}
\put(0.9,2.3){$1$} 
\put(1.9,2.3){$2$} 
\put(2.9,2.3){$3$} 
\put(3.9,2.3){$4$} 
\put(4.9,2.3){$5$} 
\put(5.9,2.3){$6$} 
\put(6.9,2.3){$7$} 
\put(7.9,2.3){$8$} 
% index for grid points on coarse mesh
\put(-0.1,1.3){$0$}
\put(1.9,1.3){$1$} 
\put(3.9,1.3){$2$} 
\put(5.9,1.3){$3$} 
\put(7.9,1.3){$4$} 
% text
\put(-1,2){$\Omega_h$:}
\put(-1,1){$\Omega_{2h}$:}
\end{picture}
\end{center}
\caption{The fine grid $\omega_h$ and the coarse grid $\omega_{2h}$ with $N=8$.\label{fig:fine-coarse-grid}}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Numerical verification}
To verify the theory in Sec. \ref{sec:iter_vs_eig}, we
consider two tests.

In the first test we consider the problem
\begin{align}
\omega^2 u +\Delta u = \omega^2\delta(\bx-\bx_c), \quad\bx\in[0,1]^d,\bx_c=(0.5,\dots,0.5)^T, d=2,3.
\end{align}
We consider $\omega=40,80$ in 2D with and $\omega=20,40$ in 3D, In each direction we use $N=2^{\lceil\log_2(\lceil 4\omega\rceil)\rceil}-1$ in 2D and $N=2^{\lceil\log_2(\lceil 2\omega\rceil)\rceil}-1$ grid points in 3D. In the deflation step we not only use eigenvectors from the original grid but also use the eigenvectors interpolated from one level and two level coarsen grids.

In Fig. \ref{fig:iter_vs_eig} we plot the number of iterations of the DCG method to reach the relative tolerance $10^{-7}$ as a function of the number of eigenvectors in the deflation space.
According to our theory if the number of eigenvalues $K$ scales as $O(\omega^s)$, the number of iterations for the convergence $N_{\textrm{iter}}$ scales as $O(\omega^{d-s})$. Under the $\log$-scale we have
\begin{equation}
    \log_{10}(K)\propto\log_{10}(\omega) s \quad\text{and}\quad
    \log_{10}(N_{\textrm{iter}})\propto \log_{10}(\omega)(d-s)=\log_{10}(\omega)d - \log_{10}(K),
\end{equation}
so $log_{10}(K)$-$\log_{10}(N_{\textrm{iter}})$ picture is a straight line with slope $-1$. 
In Fig. \ref{fig:iter_vs_deflation_dim} $N_{\textrm{iter}}$-$K$ can indeed be qualitatively captured by straight lines with slope $-1$ under the $\log$-scale with both exact eigenvectors and eigenvectors interpolated from one or two level coarsened grid. 

In the second test 

 

\begin{figure}[htb]
\begin{center}
\includegraphics[width=0.46\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/2d_eig_vs_iter_eig_orig_40.eps}
\includegraphics[width=0.46\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/2d_eig_vs_iter_eig_orig_80.eps}
\includegraphics[width=0.46\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/3d_eig_vs_iter_eig_orig_20.eps}
\includegraphics[width=0.46\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/3d_eig_vs_iter_eig_orig_40.eps}
\caption{Number of iterations as a function of number of eigenvectors in the deflation space to reach relative error tolerance $10^{-7}$. \label{fig:iter_vs_eig}}
\end{center}
\end{figure}







\subsection{Complexity}
In this section we express the complexity with respect to estimated floating point operations and storage requirements. Throughout we assume that the discretization is done with a fixed number of points per wavelength. We give the complexity estimates both in terms of the frequency $\omega$ and the system size $N$. As will be seen some of the estimates are dimension dependent.   

\begin{table}[htbp]
  \centering
 \medskip
    \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|}
    \hline
 	Apply $A$ & $W^TA r$ & $(W^TAW)^{-1}$ & $O(N)$ operations & Total cost & Memory \\ \hline
 	$N\times N_t$ & $k_\textrm{eig}\times N$ & $k_\textrm{eig}^2$ \textrm{or} $k_\textrm{eig}$ & $N$ & $k_\textrm{eig}\times N$ &
 	 $k_\textrm{eig}\times N$ \\ \hline
 	$\omega^d\times N_t$ & $\omega^{2d}$ & $\omega^{2d}$ or $\omega^d$ & $\omega^d$ &
 	$\omega^{2d}$ & $\omega^{2d}$\\ 
 	\hline
 	 $N\times N_t$ & $N^2$ & $N^{2}$ or $N$ & $N$ & $N^2$ & $N^2$\\
 	\hline
 \end{tabular}
      \caption{}
\end{table}

\begin{table}[htbp]
  \centering
 \medskip
    \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|}
    \hline
 	Apply $A$ & $W^TA r$ & $(W^TAW)^{-1}$ & $O(N)$ operations & Total cost & Memory \\ \hline
 	$N\times N_t$ & $k_\textrm{eig}\times N$ & $k_\textrm{eig}^2$ \textrm{or} $k_\textrm{eig}$ & $N$ & $k_\textrm{eig}\times N$ &
 	 $k_\textrm{eig}\times N$ \\ \hline
 	$\omega^d\times N_t$ & $\omega^{d+s}$ & $\omega^{2s}$ or $\omega^{s}$ & $\omega^d$ &
 	$N_\textrm{iter}\omega^{d+s}$ & $\omega^{d+s}$\\ 
 	\hline
 	 $N\times N_t$ & $N^{1+s/d}$ & $N^{2s/d}$ or $N^{s/d}$ & $N$ & $N_\textrm{iter}\times N^{1+s/d}$ & $N^{1+s/d}$\\
 	\hline\hline
 	 	 $N\times N_t$ & $N$ & $1$  & $N$ & $N^2$ & $N$\\
 	\hline
 	 	 	 $N\times N_t$ & $N^{1+(d-1)/d}$ & $N^{2(d-1)/d}$ or $N^{(d-1)/d}$ & $N$ & $ N^2$ & $N^{1+(d-1)/d}$\\
 	 	 	 \hline
 \end{tabular}
      \caption{}
\end{table}


\begin{table}[htbp]
\scriptsize
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|}
    \hline
 	& Apply $A$ & $W^TA r$ & $(W^TAW)^{-1}$ & Form $AW$ & Form $W$ & Total cost & Memory    \\ 
 	 	\hline
 	DCG & $NN_t$ & $N^{2}$ & $N^2$ or $N$ & $N_tN^2$ & $N_\textrm{arpack}$ & $N_\textrm{RHS}( N_\textrm{iter}N+ N^{2})+N_t N^2+N_\textrm{arpack}$ & $N^2$
 	 \\ \hline
 	DCG & $N N_t$ & $N^{1+s/d}$ & $N^{2s/d}$ or $N^{s/d}$ & $N_tN^{1+s/d}$ & $N_\textrm{arpack}$ & $N_\textrm{RHS}( N^{1-s/d}N+ N^{1+s/d}) +N_t N^{1+s/d}+N_\textrm{arpack}$& $N^{1+s/d}$
 	 \\ \hline
 	 DCG & $\omega^d N_t$ & $\omega^{d+s}$ & $\omega^{2s}$ or $\omega^s$ & $N_t\omega^{d+s}$ & $N_\textrm{arpack}$ & $N_\textrm{RHS}( \omega^{2d-s}+ \omega^{d+s}) +N_t \omega^{d+s}+N_\textrm{arpack}$& $\omega^{d+s}$
 	 \\ \hline
   CG & $N N_t$ & NA & NA & NA & NA & $N_\textrm{RHS}N^2$ & $N$ \\ \hline
   CG & $N N_t$ & NA & NA & NA & NA & $N_\textrm{RHS}\omega^{2d}$ & $N$ \\ \hline
 \end{tabular}
      \caption{}
 \end{center}
\end{table}
\normalsize


\begin{figure}[htb]
\begin{center}
\includegraphics[width=0.48\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/neigs_vs_cputime_40_2d}
\includegraphics[width=0.48\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/neigs_vs_cputime_30_3d}
\includegraphics[width=0.48\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/neigs_vs_iter_40_2d}
\includegraphics[width=0.48\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/neigs_vs_iter_30_3d}
\caption{CPU time and number of iterations for the KrylovKit (Krylov-Schur algorithm) to compute eigenvectors. Left: 2D. Right: 3D. \label{fig:eig_efficiency}}
\end{center}
\end{figure}


\subsection{Rate of convergence with and without deflation}


\begin{figure}[htb]
\begin{center}
\includegraphics[width=0.32\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/2d_iter_vs_defdim}
\includegraphics[width=0.32\textwidth]{figures/3d_iter_vs_defdim}
\includegraphics[width=0.32\textwidth]{figures/3d_iter_vs_defdim_2}
\caption{Number of iterations for convergence for different dimensions of the deflation space. \label{fig:iter_vs_deflation_dim}}
\end{center}
\end{figure}


\subsection{Compression of matrices}
\subsubsection{Compression of $W$}
\subsubsection{Compression of $W^T \whiA$}

\clearpage


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Experiments in One Dimension}
The eigenvalues and eigenvectors of the three point discretization $[-1, 2, -1]$ of the Laplacian on the unit square with a grid size $h=1/(n+1)$ with Dirichlet boundary conditions are
\begin{eqnarray}
    \lambda_k &= 2 \left(1-\cos \left(\frac{k \pi}{n+1}\right) \right),\ \ k = 1\ldots,n \\
    v_k[i] &= \sqrt{\frac{2}{n+1}} \sin\left(i\frac{k\pi}{n+1}\right),\ \  i = 1\ldots,n,\, k = 1\ldots,n. 
\end{eqnarray}

To test how well the deflation works with eigenvectors computed on a coarse grid and then interpolated to a fine grid we consider the grids with $n=2^l-1$ interior points. In this experiment we only consider the case when the course and the fine level are one level apart. 

In Fig. \ref{fig:conv_linear} and Fig. \ref{fig:conv_spline} we display the relative reduction in the Euclidean norm of each of the eigenvectors after one WaveHoltz iteration using $\omega = 30$. We also display the the square root of the WaveHoltz filter function 
\begin{equation}
\beta(\lambda;\omega) = \frac{\omega (3 \lambda^2+\omega^2) \sin \left(2 \pi \frac{\lambda}{\omega} \right)}{ (4 \pi (\lambda^3 - \lambda \omega^2)},
\end{equation}
and the relative reduction in the Euclidean norm of the error in the interpolated eigenvector with the part along the coarse eigenvector removed (deflated). To be precise, let $\mathcal{I}$ be the interpolation (prolongation) operator and $v^{\rm f}_k$ and $ v^{\rm c}_k$ be the $k$th eigenvectors on the fine and coarse grids. Then for each $\lambda_k$ on the coarse grid we display $ \| \Pi \delta_{\rm D} \| / \| \delta_{\rm D} \|$ where
\[
\delta_{\rm D} = v^{\rm f}_k -  \mathcal{I} v^{\rm c}_k. 
\]  

The two different figures display results using linear interpolation and spline interpolation.

As can be seen in both cases the WaveHoltz iteration is highly efficient in reducing the size of the error contribution orthogonal to the deflation subspace (in this case a single vector...).

It is also clear that the reduction is improved with increasing resolution but also on coarse meshes it is fairly good.

\begin{figure}[htb]
\begin{center}
\includegraphics[width=1.0\textwidth,trim={8.0cm 2.5cm 6.0cm 2.3cm},clip]{figures/conv_in_norm1D_linear}
\caption{Relative reduction in norm using deflation with interpolated eigenvectors. This figure is for linear interpolation. \label{fig:conv_linear}}
\end{center}
 \end{figure}

\begin{figure}[htb]
\begin{center}
\includegraphics[width=1.0\textwidth,trim={8.0cm 2.5cm 6.0cm 2.3cm},clip]{figures/conv_in_norm1D_spline}
\caption{Relative reduction in norm using deflation with interpolated eigenvectors. This figure is for spline interpolation. \label{fig:conv_spline}}
\end{center}
 \end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\clearpage
\subsection{Experiments in Two Dimensions}
\subsubsection{The unit square}
% This is computations using the file test2D_square.m
The eigenvalues and eigenvectors of the five point discretization of the Laplacian on the unit square with a grid size $h=1/(n+1)$ with Dirichlet boundary conditions are found by tensor products from the one dimensional case. 
%\begin{eqnarray}
%    \lambda_k &= 2 \left(1-\cos \left(\frac{k \pi}{n+1}\right) \right),\ \ k = 1\ldots,n \\
 %   v_k[i] &= \sqrt{\frac{2}{n+1}} \sin\left(i\frac{k\pi}{n+1}\right),\ \  i = 1\ldots,n,\, k = 1\ldots,n. 
%\end{eqnarray}

Let $n$ be odd, then we can prolongate these onto a grid with $n_{\rm f} = (n-1)/2+1$ points by injection and linear interpolation (i.e. averaging). 

In Fig. \ref{fig:unit_square1} we display the number of iterations needed to reach a relative tolerance of $10^{-12}$ for $\omega = 10,11,\ldots,70$ using $n = \lceil 4 \omega \rceil -1$ and with the number of eigenvalues in the deflation space being $\lceil 0.005N \rceil $. The figure to the right also includes the number of iterations needed for the standard CG algorithm.

We note that the computations only computed the eigenvectors by prolonging those from a coarser grid, the matrix $\matW^T \whiA$ was formed using the prolonged eigenvectors. We next consider the case when also $\matW^T \whiA$ is computed on a coarse grid.

\begin{figure}[htb]
\begin{center}
\includegraphics[width=0.45\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/unit_square_iter2}
\includegraphics[width=0.45\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/unit_square_iter1}
\caption{Number of iterations needed to reach tolerance $10^{-12}$ for deflation using eigenvalues/eigenvectors computed on the grid (DCG) and using prolongated eigenvectors computed on a grid coarsened by a factor of 2 (DCG-prolonged). To the right results for CG is included for reference.  \label{fig:unit_square1}}
\end{center}
 \end{figure}


\subsection{Experiments in Three Dimensions}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\clearpage

\subsection{Experiments on the $d$-dimensional unit cube}
In one dimension the eigenvalues and eigenvectors of the three-point center difference discretization $[-1,2,-1]$ of the Laplacian operator with a grid size $h=1/(n+1)$ with Dirichlet boundary conditions are
\begin{subequations}
    \begin{align}
        &\lambda_k = 2\left(1-\cos(\frac{k\pi}{n+1})\right),\;k=1,\dots,n,\\
        &\vb_k^n[i] =\sqrt{\frac{2}{n+1}}\sin\left(i\frac{k\pi}{n+1}\right),\;i=1,\dots,n,\;k=1,\dots,n. 
    \end{align}
\end{subequations}
Let the matrix corresponding to this discretization be $L^{\textrm{(1d)}}_n$. Then $5$-point and $7$-point central difference of the  Laplacian operator for the unit square in 2D and unit cube in 3D can be written as
\begin{equation}
L^{\textrm{(2d)}}_n=L^{\textrm{(1d)}}_n\otimes I_{n}+I_{n}\otimes L^{\textrm{(1d)}}_n \quad\text{and}\quad
L^{\textrm{(3d)}}_n=(L^{\textrm{(1d)}}_n\otimes I_{n})\otimes I_{n}+
(I_{n}\otimes L^{\textrm{(1d)}}_n )\otimes I_{n}+
I_{n}\otimes (I_{n}\otimes L^{\textrm{(1d)}}_n )
\end{equation}
respectively. 

To test the deflation with eigenvectors computed on a coarse mesh and then prolonged to a fine grid, we consider $n=2^l-1$ interior points along one direction.

Besides the original DCG algorithm, we also consider two modified version of it. We call the first modified version DCG-D. We invert the diagonal part of $W^TAW$, namely $\textrm{diag}(W^TAW)$, instead of $W^TAW$. With $A$ being SPD and $W$ being eigenvectors of $A$ $W^TAW$ is diagonal, however, when $W$ is constructed with prolonged eigenvectors $W^TAW$ is not exactly diagonal. In the second modified version of DCG we drop  $ {\bm \mu} \gets (\matW^T \whiA \matW)^{-1} (\matW^T \whiA \rb)$ in the inner loop of Algorithm \ref{alg:DCG}, and we call it DCG-OI.  

We investigate the relation between number of iterations for the relative residual below $10^{-7}$ and the dimension of deflation space. We consider a problem with point source on the center of the computational domain $[0,1]^d$ with $d=1,2,3$.  In 1D the number of grid points is $n=2^{\lceil\log_2(\lceil16\omega\rceil)\rceil}-1$. In 2D we use 
$n=2^{\lceil\log_2(\lceil4\omega\rceil)\rceil}-1$ grid points along one direction.

\textcolor{blue}{Comment on the observations.}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[htb]
\begin{center}
\includegraphics[width=0.32\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/regular_geometry/1d_iter_eig1_orig.eps}
\includegraphics[width=0.32\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/regular_geometry/1d_iter_eig1_diag.eps}
\includegraphics[width=0.32\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/regular_geometry/1d_iter_eig1_no.eps}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\includegraphics[width=0.32\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/regular_geometry/1d_iter_eig75_orig.eps}
\includegraphics[width=0.32\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/regular_geometry/1d_iter_eig75_diag.eps}
\includegraphics[width=0.32\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/regular_geometry/1d_iter_eig75_no.eps}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\includegraphics[width=0.32\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/regular_geometry/1d_iter_eig5_orig.eps}
\includegraphics[width=0.32\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/regular_geometry/1d_iter_eig5_diag.eps}
\includegraphics[width=0.32\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/regular_geometry/1d_iter_eig5_no.eps}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\includegraphics[width=0.32\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/regular_geometry/1d_iter_eig25_orig.eps}
\includegraphics[width=0.32\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/regular_geometry/1d_iter_eig25_diag.eps}
\includegraphics[width=0.32\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/regular_geometry/1d_iter_eig25_no.eps}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\caption{Number of iterations as a function of frequency on 1D unit interval.\label{fig:iter_vs_omega_1d}}
\end{center}
 \end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[htb]
\begin{center}
\includegraphics[width=0.32\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/regular_geometry/2d_iter_eig2_orig.eps}
\includegraphics[width=0.32\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/regular_geometry/2d_iter_eig2_diag.eps}
\includegraphics[width=0.32\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/regular_geometry/2d_iter_eig2_no.eps}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\includegraphics[width=0.32\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/regular_geometry/2d_iter_eig15_orig.eps}
\includegraphics[width=0.32\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/regular_geometry/2d_iter_eig15_diag.eps}
\includegraphics[width=0.32\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/regular_geometry/2d_iter_eig15_no.eps}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\includegraphics[width=0.32\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/regular_geometry/2d_iter_eig1_orig.eps}
\includegraphics[width=0.32\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/regular_geometry/2d_iter_eig1_diag.eps}
\includegraphics[width=0.32\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/regular_geometry/2d_iter_eig1_no.eps}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\includegraphics[width=0.32\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/regular_geometry/2d_iter_eig05_orig.eps}
\includegraphics[width=0.32\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/regular_geometry/2d_iter_eig05_diag.eps}
\includegraphics[width=0.32\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/regular_geometry/2d_iter_eig05_no.eps}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\caption{Number of iterations as a function of frequency on 2D unit square.\label{fig:iter_vs_omega_1d}}
\end{center}
 \end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newpage

Line 17: 
\begin{align}
W^TAW=D+B=D+U\Sigma U^T
=UDU^T+U\Sigma U^T
= U(D+\Sigma)U^T\\
 U(D+\Sigma)^{-1}U^T\\
D^{-1}W^TAW=D^{-1}(D+U\Sigma U^T)
= I + D^{-1} U\Sigma U^T
\end{align}
Von-Neumann series converges fast.
%\end{comment}




==> tex/symm3D.tex <==
%!TEX root = ../deflation.tex

\section{Numerical experiments for symmetric discretizations\label{sec:numerical}}

\input tex/symm2D


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{3D homogeneous cube \label{sec:convergence_test_3d}}
We consider a 3D homogeneous problem with $c(x,y,z)=1$ and a point source term $\delta(x-0.1,y-0.1,z-0.1)$ in the computational domain $[0,1]^3$. We consider three different frequencies $\omega=20,\;25,\;30$. We partition the computation domain with a uniform mesh having $131$ grid points for $\omega = 20$, $181$ grid points for $\omega=25$ and $231$ grid points for $\omega=30$ in each direction. These number of grid points per direction is chosen based on the in the principle determining points per wave length to reach at least $2\%$ relative error. \pzc{cite Bill's paper here}. We set the relative tolerance in the stopping criteria of the CG and DCG solver as $10^{-9}$.

\textbf{Performance with different dimensions of the deflation space.} For this homogeneous medium, the eigenvalues of the the discrete WaveHoltz operator can be analytically computed. Based on this fact, we estimate the condition number of the deflated operator by $\frac{1.5}{\hat{\lambda}_{\Na+1}}$, where $\hat{\lambda}_{\Na+1}$ is the $\Na+1$-th smallest eigenvalue of the discrete WaveHoltz operator. The estimated condition number is displayed in the bottom left plot of Fig. \ref{fig:convergence_test_3d}. We observe that the estimated condition number approximately scales as $O(\Na^{-2})$  for all frequencies, where $\Na$ is the number of eigenvectors in the deflation space. This observation matches our analysis.

In the top and bottom right plots of Fig. \ref{fig:convergence_test_3d}, we present the number of iterations for convergence and relative computational time with respect to the CG method. For all frequencies, the number of iterations for convergence scales roughly as $O(\Na^{-0.9})$ before bottoming out. The relative computational time of DCG with respect to CG scales roughly as $O(\Na^{-0.9})$. In comparison with CG, when $\Na=300$, DCG achieves at most more than $10.46$ times acceleration for $\omega=20$,  $8.40$ times acceleration for $\omega=25$ and $10.01$ times acceleration for $\omega=30$. 

\textbf{Prolonged eigenvectors as the deflation matrix.} In Fig. \ref{fig:convergence_test_3d_window}, we compare the number of iterations for convergence  and computational time using prolonged eigenvectors and analytical eigenvectors. We observe that, for frequencies $\omega=20,25,30$, employing prolonged eigenvectors from the $1$-level or $2$-level coarsened mesh, DCG converges with number of iterations comparable to using fine level eigenvectors. However, using prolonged eigenvectors requires enforcing $A$-orthogonality in each iteration. As a result, the speed-up gained by using prolonged eigenvectors is less compared to using the fine level eigenvectors. 


In summary, prolonged eigenvectors as the deflation matrix performs well when the fine level eigenvectors are well approximated on the coarse mesh, otherwise it may suffer from significant efficiency decline.

\begin{figure}[htb]
\begin{center}
\includegraphics[width=0.32\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/iter_3d_20.eps}
\hspace{0.1cm}
\includegraphics[width=0.32\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/iter_3d_25.eps}
\hspace{0.1cm}
\includegraphics[width=0.32\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/iter_3d_30.eps}
\includegraphics[width=0.32\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/cond_3d.eps}
\includegraphics[width=0.32\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/time_3d.eps}
\caption{Results for the 3D  homogeneous cube in Sec. \ref{sec:convergence_test_3d}. Top: relative and absolute number of iterations. Bottom left: estimated conditional number of $W^TAW$. Bottom right: relative computational time with respect to the CG method.   \label{fig:convergence_test_3d}}
\end{center}
 \end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \begin{figure}[htb]
\begin{center}
\includegraphics[width=0.32\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/iter_3d_ml_20.eps}
\includegraphics[width=0.32\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/iter_3d_ml_25.eps}
\includegraphics[width=0.32\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/iter_3d_ml_30.eps}
\includegraphics[width=0.32\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/time_3d_ml_20.eps}
\includegraphics[width=0.32\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/time_3d_ml_25.eps}
\includegraphics[width=0.32\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/time_3d_ml_30.eps}
\caption{Performance of DCG for 3D  homogeneous cube with deflation matrices comprising prolonged eigenvectors  in Sec. \ref{sec:convergence_test_3d}.  Top: relative and absolute number of iterations for convergence. Bottom: relative computational time compared to CG. \label{fig:convergence_test_3d_window}}
\end{center}
 \end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{3D homogeneous ball\label{sec:3d-ball}}
We consider a 3D homogeneous problem   ball
$\{(x,y,z):\sqrt{x^2+y^2+z^2}\leq0.5\}$ 
with $c^2(\xb)=1$ and homogeneous boundary conditions. The source term is defined as
\begin{equation}
    f(x,y,z) = \frac{16\omega^2}{\pi}e^{-16\omega^2( (x-x_c)^2+(y-y_c)^2+(z-z_c)^2 )},
\end{equation}
where $\omega=25$ is the frequency of the underlying problem. The relative tolerances in the stopping criteria of CG and DCG are $10^{-9}$.

To handle the curvilinear geometry, we utilize the second order embedded  boundary (EB) finite difference method in \cite{peng2023universal}. This EB method use interior boundary points leads to a SPD discrete Laplacian operator, so CG solver can still be applied. Moreover, it also avoids small cell stiffness, so a standard CFL condition can still be used in the time-domain simulation of the wave equation.
In the EB method, we set computational domain as $[-0.55,0.55]^3$  and partition it by a uniform cartesian mesh with $220$ grid points in each direction. 

To construct the deflation matrix, we use Lanczos method to compute $100$ eigenvectors  and obtain $123$ converged eigenvectors. The tolerance of the residual for Schur vectors in the Lanczos algorithm is set as $10^{-10}$. The deflation matrix consists of all converged eigenvectors.

\textbf{Different source terms.} To test the performance of the proposed DCG methods for different source terms, we uniformly  pick $10$ different random center points for the source term $(x_c,y_c,z_c)$ inside the ball $\{\sqrt{x^2+y^2+z^2}\leq0.25\}$.

Results are summarized in Tab. \ref{tab:3d-ball}. We observe that, on average, the DCG algorithm converges with approximately $18.90\%$ number of iterations and leads to approximately $3.60$ times acceleration compared to CG. 
The computational time of constructing the deflation matrix is approximately $11.105$ times of the average time for one CG solve. As a result, we gain computational saving if the Helmholtz equation is solved for more than $16$ different source terms.   

\textbf{Same deflation for a narrow frequency band.} We use the deflation matrix constructed for $\omega=25$ to solve problems with $\omega=24.5,24.6,\dots,30.5$ and the source term corresponding to $(x_c,y_c,z_c)=(0.1,0.1,0.1)$. As displayed in Fig. \ref{fig:3d_ball_windowed_deflation}, we observe that, for all frequencies, DCG converges with less number of iterations than CG and achieves approximately $4.00$ to $5.21$ times acceleration compared to CG. %Surprisingly, though the deflation matrix consists of eigenvectors for $\omega=40$, we achieve the largest acceleration at $\omega=40.3$. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[htbp]
  \centering
 \medskip
    \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|}
    \hline
   $\textrm{Iter}_\textrm{CG}$ & $\textrm{Iter}_\textrm{DCG}$ & ${T}_{\textrm{DCG}}/{{T}_{\textrm{CG}}}$ & ${T_{\textrm{Eig}}}/{{T}_{\textrm{CG}}}$ \\ \hline
  $129.8$ & $20.1$ &  $0.278$ & 11.105 \\ \hline
 \end{tabular}
      \caption{Multiple source terms test for the 3D homogeneous ball in Sec. \ref{sec:3d-ball}. $\Na$: dimension of the deflation space. $\textrm{Iter}_\textrm{(D)CG}$: average number of iterations for (D)CG. $T_{\textrm{D}CG}$: average computational time for the (D)CG. $T_{Eig}$: computational time of obtaining eigenvectors needed by the deflation.  \label{tab:3d-ball}}
\end{table}

\begin{figure}[htb]
\begin{center}
\includegraphics[width=0.40\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/ball_25_various_frequencies.eps}
\caption{The same deflation for various frequencies for the homogeneous ball in Sec. \ref{sec:3d-ball}. Relative number of iterations and computational time of DCG compared to CG are displayed. \label{fig:3d_ball_windowed_deflation}}
\end{center}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{3D inhomogeneous problem\label{sec:3d-ih}}
We consider a 3D inhomoeneous problem on the computational domain $[-0.5,0.5]^3$ with the velocity field 
\begin{equation}
    c^2(x,y,z) = 1.0-0.9e^{-\left( \frac{x^2+y^2+z^2-0.25^2}{0.25^2}\right)^4 }
\end{equation}
and the frequency $\omega=20$.
We consider the source term \begin{equation}
    f(x,y,z) = \frac{16\omega^2}{\pi}e^{-16\omega^2( (x-x_c)^2+(y-y_c)^2+(z-z_c)^2 )},
\end{equation}
where $\omega$ is the frequency of the underlying problem.
We use a uniform grid with $181$ grid points in each direction. The relative tolearnces for the stopping criteria of CG and DCG are chosen as $10^{-9}$.

To construct a deflation matrix, we use Lanczos method to compute $80$ smallest eigenvectors of the WaveHoltz operator on the original mesh and $1$-level coarsend mesh. The tolerance of the residual for Schur vectors is $10^{-11}$. With no coarsening and $1$-level coarsening, the Lanczos algorithm converges with $63$ and $61$ iterations and results in $84$ and $93$ converged eigenvectors, respectively. When eigenvectors are computed on the coarse mesh, we interpolate it to the original mesh with  linear interpolation.



\textbf{Different source terms.} To test the performance of the proposed DCG method for different source terms, we uniformly  pick $10$ different random center points $(x_c,y_c,z_c)$ for the source term  inside the ball $\{\sqrt{x^2+y^2+z^2}\leq0.25\}$.

Results are summarized in Tab. \ref{tab:3d-ih}. On average, deflation matrices comprising eigenvectors and prolonged eigenvectors lead to approximately $27.5\%$ and $29.5\%$ number of iterations for convergence and $3.61$ and $2.79$ times acceleration compared to CG, respectively. 
The average computational time to obtain eigenvectors and prolonged eigenvectors are approximately $7.070$ and $0.595$ times of the average time for one CG solve. Accounting for the time of constructing the deflation matrix, we gain computational saving when solving more than $10$ source terms for the eigenvector deflation and $2$ source terms for the prolonged eigenvector deflation.  

\textbf{Performance with different dimensions of the deflation space.} With $(x_c,y_c,z_c)=(-0.4,0.45,0.4)$, we test the performance of DCG with different dimensions of the deflation space $\Na$. The corresponding numerical solution is presented in Fig. \ref{fig:3d_ih_solution} 
As shown in Fig. \ref{fig:3d_ih}, DCG method converges with less number of iterations and computational time compared to CG. The number of iterations and computational time for convergence approximately scale as $O(\Na^{-0.6})$. 

\textbf{Same deflation for a narrow frequency band.} We use the converged $84$ eigenvectors and $93$ prolonged eigenvectors for $\omega=20$ as the deflation matrix for frequencies in the band $[19.4,20.6]$. As displayed in Tab. \ref{fig:3d_ih}, both eigenvector and prolonged eigenvector deflation is faster than CG. For all tested frequencies except for $\omega=20.6$, using the fine level eigenvectors as the deflation matrix achieves more acceleration than using prolonged eigenvectors. %when the frequency $\omega$ is close to $20$, this deflation matrix results in less number of iterations for convergence and smaller computational time.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[htbp]
  \centering
 \medskip
    \begin{tabular}
    {|l|c|c|c|c|c|c|c|c|c|c|c|}
    \hline
Eigenvector computation & $\Na$ & $\textrm{Iter}_\textrm{CG}$ & $\textrm{Iter}_\textrm{DCG}$ &  $\textrm{Iter}_\textrm{Eig}$ & ${T}_{\textrm{DCG}}/{{T}_{\textrm{CG}}}$ & ${T_{\textrm{Eig}}}/{{T}_{\textrm{CG}}}$ \\ \hline
 No coarsening & $84$ &  $511.1$ & $140.6$ & $63$ & $0.277$ & $7.070$ \\ \hline
 $1$-level coarsening & $93$ & $511.1$ & $151$ & $61$ & $0.358$ & $0.696$ \\ \hline
 \end{tabular}
      \caption{Multiple source terms test for the 3D inhomogeneous problem in Sec. \ref{sec:3d-ih}. $\textrm{Iter}_\textrm{(D)CG}$: average number of iterations for (D)CG. $T_{\textrm{D}CG}$: average computational time for the (D)CG. $T_{Eig}$: computational time of obtaining eigenvectors needed by the deflation.  \label{tab:3d-ih}}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[htbp]
  \centering
 \medskip
    \begin{tabular}
    {|l|c|c|c|c|c|c|c|c|c|c|c|}
    \hline
 $\omega$ & $19.4$ & $19.6$ & $19.8$ & $20.0$ & $20.2$ & $20.4$ & $20.6$\\ \hline
 {$\textrm{Iter}_\textrm{DCG}/\textrm{Iter}_\textrm{CG}$, no coarsening} &  $0.458$&    $0.303$&    $0.289$&    $0.301$&    $0.335$&    $0.485$& $0.917$ \\ \hline
 {$\textrm{Iter}_\textrm{DCG}/\textrm{Iter}_\textrm{CG}$}, $1$-level coarsening &  $0.861$&    $0.473$ &    $0.350$&    $0.321$ &    $0.248$ &    $0.301$    & $0.335$ \\ \hline
{${T}_{\textrm{DCG}}/{{T}_{\textrm{CG}}}$, no coarsening} &  $0.459$&    $0.300$   & $0.271$   & $0.301$    &$0.329$    & $0.488$    & $0.952$ \\ \hline
 {${T}_{\textrm{DCG}}/{{T}_{\textrm{CG}}}$, 1-level coarsening} &    $0.985$&    $0.607$&    $0.401$&    $0.423$&    $0.328$&    $0.377$&    $0.349$\\\hline 
 \end{tabular}
      \caption{Same deflation for frequencieis in a narrow band for the 3D inhomogeneous problem in Sec. \ref{sec:3d-ih}. $\textrm{Iter}_\textrm{(D)CG}$: average number of iterations for (D)CG. $T_{\textrm{(D)CG}}$: average computational time for the (D)CG.  \label{tab:3d-ih-window}}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[htb]
\begin{center}
\includegraphics[width=0.32\textwidth,trim={0.3cm 0.3cm 0.3cm 0.4cm},clip]{figures/sliced_solution_x.eps}
\includegraphics[width=0.32\textwidth,trim={0.3cm 0.05cm 0.3cm 0.4cm},clip]{figures/sliced_solution_y.eps}
\includegraphics[width=0.32\textwidth,trim={0.3cm 0.05cm 0.3cm 0.4cm},clip]{figures/sliced_solution_z.eps}
\caption{Slices of the numerical solution for 3D inhomogeneous problem in Sec. \ref{sec:3d-ih} with the source term corresponding to $(x_c,y_c,z_c)=(-0.4,0.45,0.4)$.  \label{fig:3d_ih_solution}}
\end{center}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%
 \begin{figure}[htb]
\begin{center}
\includegraphics[width=0.45\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/iter_3d_ih.eps}
\hspace{0.1cm}
\includegraphics[width=0.45\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/time_3d_ih.eps}
%\includegraphics[width=0.32\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/cube_20_various_frequencies.eps}
\caption{Results for 3D inhomogeneous problem in Sec. \ref{sec:3d-ih} with the source term corresponding to $(x_c,y_c,z_c)=(-0.4,0.45,0.4)$. Left: relative and absolute number of iterations for convergence for $\omega=20$. Right: relative computational time for $\omega=20$. \label{fig:3d_ih}}
\end{center}
\end{figure}
